Abundances of 30 elements in 23 metal-poor stars

We report the abundances of 30 elements in 23 metal-poor ([Fe/H] <-1.7) giants. These are based on 7774 equivalent widths and spectral synthesis of 229 additional lines. Hyperfine splitting is taken into account when appropriate. Our choice of model atmospheres has the most influence on the accuracy of our abundances. We consider the effect of different model atmospheres on our results. In addition to the random errors in Teff, log g, and microturbulent velocity, there are several sources of systematic error. These include using Teff determined from FeI lines rather than colors, ignoring NLTE effects on the FeI/FeII ionization balance, using models with solar [alpha/Fe] ratios and using Kurucz models with overshooting. Of these, only the use of models with solar [alpha/Fe] ratios had a negligible effect. However, while the absolute abundances can change by > 0.10 dex, the relative abundances, especially between closely allied atoms such as the rare earth group, often show only small (<0.03 dex) changes. We found that some strong lines of FeI, MnI and CrI consistently gave lower abundances by ~0.2 dex, a number larger than the quoted errors in the gf values. After considering a model with depth-dependent microturbulent velocity and a model with hotter temperatures in the upper layers, we conclude that the latter did a better job of resolving the problem and agreeing with observational evidence for the structure of stars. The error analysis includes the effects of correlation of Teff, log g, and microturbulent velocity errors, which is crucial for certain element ratios, such as [Mg/Fe]. The abundances presented here are being analyzed and discussed in a separate series of papers.

==> tab2a.tex <==
\begin{deluxetable}{lccccccccccccccc}
\tabletypesize{\scriptsize}
\tablenum{2A}
\tablewidth{0pt}
\tablecaption{Equivalent Widths (m\AA)}
\tablehead{
\colhead{$\lambda$ (\AA)}  & \colhead{log $gf$} & \colhead{EP} 
& \multicolumn{2}{r}{63791} & \multicolumn{2}{r}{108577} & 
\multicolumn{2}{r}{122563}
& \multicolumn{2}{r}{128279} 
& \multicolumn{2}{r}{186478} & \multicolumn{2}{r}{218857}
& \colhead{Source} \\
\colhead{} & \colhead{}  & \colhead{eV} &
\multicolumn{2}{l}{29574} &\multicolumn{2}{l}{88609} & \multicolumn{2}{l}{115444} &
\multicolumn{2}{l}{126587} & \multicolumn{2}{l}{165195}  & \multicolumn{2}{l}{216143} & \colhead{} 
}
\startdata
\multicolumn{16}{c}{ NaI} \\
 5889.97 &  0.11 &  0.00 &  \nodata & 241.5 & 179.0 & 191.6 & 175.1 & 206.5 & 158.9 & 147.7 &  \nodata & 191.1 & 225.9 & 180.7 & 1      \\
 5895.94 & $-$0.19 &  0.00 &  \nodata & 219.0 & 147.5 & 165.0 & 149.6 & 160.4 & 139.7 & 131.1 &  \nodata & 188.8 & 196.3 & 165.5 & 1      \\
\multicolumn{16}{c}{ {MgI}} \\
 3829.36 & 0.13 &  2.71 &  \nodata &  \nodata & 170.2 &  \nodata & 150.5 &  \nodata & 154.6 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 2      \\
 3832.31 &  0.27 &  2.71 &  \nodata &  \nodata & 197.8 &  \nodata & 177.0 &  \nodata & 174.8 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 2      \\
 3838.30 &  0.46 &  2.72 &  \nodata &  \nodata & 221.0 &  \nodata & 205.2 &  \nodata & 200.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 2      \\
 4167.28 & $-$0.77 &  4.34 & 120.3 & 128.4 &  40.8 &  61.5 &  36.0 &  49.1 &  37.6 &  62.1 &  \nodata &  68.3 &  91.9 &  83.7 & 3      \\
 4703.00 & $-$0.52 &  4.34 & 145.9 & 132.4 &  60.6 &  87.3 &  51.7 &  70.6 &  51.1 &  77.7 & 114.4 &  84.9 & 109.4 &  92.4 & 4      \\
 5172.70 & $-$0.39 &  2.71 & \nodata & 407.8 & 202.4 & 211.7 & 173.8 & 208.5 & 169.7 & 218.0 & 294.9 & 221.3 & 261.4 &  \nodata & 4      \\
 5183.62 & $-$0.17 &  2.72 & \nodata & 466.1 & 214.1 & 236.4 & 192.2 & 237.6 & 183.0 & 245.1 & 341.0 & 247.7 & 309.6 &  \nodata & 4      \\
 5528.42 & $-$0.50 &  4.34 & 169.2 & 141.5 &  64.2 &  89.6 &  55.7 &  77.7 &  51.1 &  77.8 & 129.7 &  92.4 & 114.4 &  93.7 & 4      \\
\multicolumn{16}{c}{ {AlI}} \\
 3961.53 & $-$0.34 &  0.01 & 234.9 &  \nodata & 134.1 & 133.4 & 109.8 & 139.4 & 104.1 & 108.8 & 165.1 & 145.1 & 174.6 & 108.5 & 1      \\
\multicolumn{16}{c}{ {SiI}} \\
 4102.94 & $-$3.14 &  1.91 & 132.8 & 107.2 &  74.6 &  96.4 &  54.6 &  78.9 &  54.0 &  60.1 & 109.6 &  84.8 &  96.8 &  61.9 & 5      \\
 5648.62 & $-$2.15 & 4.93 & \nodata & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & 4.0 & \nodata & \nodata & 6 \\
 5708.41 & $-$1.47 &  4.95 &  \nodata &  34.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  11.1 &  16.3 &   9.0 & 5      \\
 5772.15 & $-$1.75 &  5.08 &  20.7 &  13.9 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   5.1 &   4.9 & 5      \\
 6155.14 & $-$0.84 &  5.62 &  21.1 &  21.9 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   9.9 &   5.9 &   9.9 &  \nodata & 6      \\
\multicolumn{16}{c}{ {CaI}} \\
 4318.65 & $-$0.21 &  1.90 & 136.1 & 108.4 &  44.1 &  65.5 &  37.4 &  52.2 &  39.4 &  55.6 &  94.1 &  66.8 &  84.4 &  71.5 & 1      \\
 4425.44 & $-$0.36 &  1.88 & 124.6 & 106.0 &  40.4 &  58.8 &  31.7 &  46.6 &  33.9 &  53.9 &  81.2 &  59.3 &  72.6 &  70.8 & 1      \\
 4455.89 & $-$0.51 &  1.90 & 110.9 &  96.4 &  29.3 &  52.2 &  24.2 &  37.0 &  26.6 &  46.2 &  79.8 &  52.7 &  72.2 &  62.3 & 1      \\
 4526.94 & $-$0.55 &  2.71 &  43.0 &  44.4 &   5.3 &  10.8 &   3.4 &   6.5 &   4.9 &  12.3 &  18.6 &  10.8 &  19.3 &  16.9 & 7      \\
 4578.55 & $-$0.70 &  2.52 &  56.8 &  51.8 &   4.7 &  13.7 &   4.0 &   7.0 &   4.3 &  12.2 &  23.1 &  13.5 &  24.7 &  19.5 & 7      \\
 5261.71 & $-$0.58 &  2.52 &  68.3 &  64.4 &  \nodata &  \nodata &  \nodata &  11.4 &  \nodata &  18.8 &  32.8 &  20.2 &  31.5 &  27.0 & 7      \\
 5265.56 & $-$0.11 &  2.52 &  \nodata &  \nodata &  19.9 &  46.7 &  17.8 &  \nodata &  17.8 &  49.2 &  \nodata &  \nodata &  \nodata &  \nodata & 7      \\
 5349.47 & $-$0.31 &  2.71 &  68.8 &  65.3 &   8.6 &  23.2 &  \nodata &  12.7 &   8.5 &  13.3 &  35.5 &  21.0 &  31.1 &  28.1 & 7      \\
 5512.98 & $-$0.45 &  2.93 &  41.8 &  44.1 &  \nodata &  11.0 &  \nodata &  \nodata &  \nodata &  \nodata &  21.0 &  12.0 &  18.2 &  17.3 & 7      \\
 5581.97 & $-$0.56 &  2.52 &  69.2 &  62.8 &  11.1 &  17.3 &  \nodata &  13.3 &  \nodata &  17.4 &  37.0 &  22.0 &  33.8 &  30.0 & 7      \\
 5588.76 &  0.36 &  2.52 & 126.6 & 106.4 &  38.4 &  64.1 &  31.8 &  48.0 &  31.6 &  59.8 &  90.0 &  69.2 &  81.0 &  70.3 & 7      \\
 5590.12 & $-$0.57 &  2.52 &  66.7 &  62.8 &  \nodata &  \nodata &  \nodata &  14.2 &  \nodata &  16.3 &  34.1 &  18.9 &  32.8 &  27.8 & 7      \\
 5594.47 &  0.10 &  2.52 & 126.2 & 105.0 &  29.1 &  51.9 &  24.3 &  36.5 &  23.6 &  40.7 &  78.7 &  53.5 &  72.1 &  60.5 & 7      \\
 5601.28 & $-$0.52 &  2.52 &  68.9 &  65.9 &   8.8 &  21.5 &  \nodata &  13.6 &   6.4 &  17.2 &  36.1 &  20.8 &  31.7 &  28.5 & 7      \\
 6102.73 & $-$0.79 &  1.88 & 125.9 &  98.4 &  29.2 &  45.5 &  19.4 &  35.8 &  26.6 &  40.5 &  85.5 &  52.3 &  74.8 &  58.5 & 1      \\
 6122.23 & $-$0.32 &  1.89 & 169.4 & 130.7 &  59.3 &  79.4 &  44.7 &  68.2 &  48.1 &  66.3 & 127.4 &  85.1 & 108.2 &  86.6 & 1      \\
 6161.29 & $-$1.27 &  2.52 &  35.9 &  26.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  12.6 &   5.7 &  10.6 &  \nodata & 7      \\
 6162.18 & $-$0.09 &  1.90 & 182.8 & 140.4 &  68.8 &  93.6 &  57.0 &  81.6 &  59.9 &  79.1 & 136.4 &  97.1 & 120.5 &  99.6 & 1      \\
 6166.44 & $-$1.14 &  2.52 &  41.4 &  35.8 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  16.1 &   8.1 &  13.3 &  10.2 & 7      \\
 6169.56 & $-$0.48 &  2.52 &  85.9 &  71.2 &  \nodata &  19.5 &  \nodata &  15.0 &  \nodata &  22.7 &  44.7 &  25.7 &  39.4 &  34.2 & 7      \\
 6439.07 &  0.39 &  2.52 & 150.4 & 123.8 &  51.6 &  77.1 &  41.3 &  61.5 &  43.0 &  60.7 & 119.8 &  75.8 &  95.4 &  80.6 & 7      \\
 6455.60 & $-$1.29 &  2.52 &  27.5 &  25.5 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  11.2 &  \nodata &   9.9 &  \nodata & 7      \\
 6471.66 & $-$0.69 &  2.52 &  91.3 &  68.3 &  10.9 &  17.8 &  \nodata &  \nodata &  \nodata &  \nodata &  35.6 &  \nodata &  30.2 &  36.1 & 7      \\
 6493.78 & $-$0.11 &  2.52 & 116.1 &  94.2 &  29.3 &  46.3 &  \nodata &  26.2 &  \nodata &  37.6 &  74.5 &  49.9 &  69.5 &  51.0 & 7      \\
 6499.65 & $-$0.82 &  2.52 &  60.7 &  59.0 &   7.0 &  15.8 &  \nodata &   9.4 &  \nodata &  20.1 &  30.2 &  17.1 &  24.5 &  \nodata & 7      \\
 6717.69 & $-$0.52 &  2.71 &  77.0 &  64.2 &  \nodata &  18.6 &  \nodata &   9.4 &  \nodata &  17.9 &  39.2 &  21.0 &  32.2 &  27.9 & 7      \\
\multicolumn{16}{c}{{ScII}} \\
 4246.84 &  0.24 &  0.31 & 213.4 & 162.9 & 123.9 & 138.7 & 107.2 & 131.3 & 103.3 &  95.4 & 174.3 & 134.8 &  \nodata & 107.2 & 8      \\
 4294.78 & $-$1.39 &  0.61 &  \nodata &  \nodata &  30.2 &  38.6 &  20.5 &  43.6 &  21.0 &  22.1 &  \nodata &  53.9 &  \nodata &  \nodata & 8      \\
 4320.75 & $-$0.25 &  0.61 &  \nodata & 118.7 &  81.9 & 107.9 &  76.3 &  94.1 &  59.9 &  63.0 & 135.3 &  97.3 & 130.5 &  75.2 & 8      \\
 4354.61 & $-$1.58 &  0.61 &  \nodata &  \nodata &  22.4 &  27.8 &  \nodata &  31.2 &  \nodata &  14.7 &  67.4 &  \nodata &  \nodata &  \nodata & 8      \\
 4415.56 & $-$0.67 &  0.60 & 137.8 & 105.6 &  61.8 &  76.4 &  49.8 &  74.0 &  43.5 &  47.8 & 106.6 &  78.1 &  97.4 &  64.0 & 8      \\
 4431.44 & $-$1.97 &  0.61 &  57.5 &  39.7 &   8.9 &  14.0 &   6.0 &  \nodata &  \nodata &  \nodata &  37.2 &  15.4 &  \nodata &  12.4 & 8      \\
 4400.40 & $-$0.54 &  0.61 &  \nodata &  \nodata &  70.5 &  81.7 &  54.5 &  \nodata &  48.8 &  51.7 &  \nodata &  79.7 &  \nodata &  \nodata & 8      \\
 4420.67 & $-$2.27 &  0.62 &  \nodata &  \nodata &   5.4 &  \nodata &  \nodata &   7.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 8      \\
 4670.41 & $-$0.58 &  1.36 &  \nodata &  70.9 &  23.6 &  39.0 &  16.1 &  34.2 &  12.3 &  14.6 &  70.0 &  37.7 &  62.6 &  27.3 & 8      \\
 5239.82\tablenotemark{a} & $-$0.76 &  1.45 &  77.8 &  52.1 &  12.6 &  23.4 &  11.5 &  19.5 &  \nodata &  \nodata &  48.8 &  25.6 &  39.7 &  17.9 & 8      \\
 5318.36 & $-$2.02 &  1.36 &  16.1 &  10.2 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   8.4 &  \nodata &   6.3 &  \nodata & 8      \\
 5526.82 &  0.02 &  1.77 & 101.0 &  76.6 &  29.8 &  46.5 &  17.5 &  39.8 &  19.6 &  20.0 &  74.3 &  45.4 &  62.5 &  36.9 & 8      \\
 5640.99 & $-$1.13 &  1.50 &  55.5 &  37.9 &   9.3 &  13.9 &  \nodata &  15.5 &  \nodata &  \nodata &  32.9 &  15.6 &  26.3 &  10.0 & 8      \\
 5657.88 & $-$0.60 &  1.51 &  90.5 &  66.2 &  17.3 &  37.0 &  13.4 &  34.6 &   8.4 &  16.2 &  66.5 &  \nodata &  54.9 &  28.5 & 8      \\
 6604.60 & $-$1.31 &  1.36 &  53.5 &  31.6 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  26.8 &  14.9 &  \nodata &  10.5 & 8      \\
\multicolumn{16}{c}{{TiI}} \\
 3653.50 & 0.28 & 0.05 & \nodata & \nodata & 57.7 & 68.6 & 52.5 &
66.4 & 49.4 & 57.8 & \nodata & 69.4 & \nodata  & \nodata & 9 \\
 3729.81 & $-$0.29 & 0.00 & \nodata & \nodata & 49.3 & 59.6 & 42.3 &
58.4 & 35.9 & 42.2 & \nodata & \nodata & 71.4  & \nodata & 9 \\
 3741.06 & $-$0.15 & 0.02 & \nodata & \nodata & 47.5 & 59.3 & 42.5 &
55.4 & 39.4 & 46.4 & \nodata & \nodata & 62.9  & \nodata & 9 \\
 3752.86 & 0.04 &  0.05 &  \nodata &  \nodata &  56.3 &  \nodata &  49.6 &  66.0 &  45.3 &  52.1 &  \nodata &  70.7 &  \nodata  & \nodata & 9      \\
 3924.53 & $-$0.88 &  0.02 &  \nodata &  77.4 &  22.6 &  31.1 &  18.3 &  27.2 &  15.6 &  22.3 &  60.9 &  40.2 &  \nodata &  \nodata & 9      \\
 3929.88 & $-$1.01 &  0.00 &  \nodata &  \nodata &  \nodata &  \nodata &  13.0 &  \nodata &   8.3 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 9      \\
 3962.85 & $-$1.11 &  0.00 &  \nodata &  \nodata &  12.1 &  22.9 &  11.1 &  17.7 &  \nodata &  12.9 &  \nodata &  27.5 &  \nodata &  \nodata & 9      \\
 3964.27 & $-$1.11 &  0.02 &  \nodata &  \nodata &   9.9 &  17.4 &  13.2 &  \nodata &   8.6 &  \nodata &  \nodata &  30.8 &  \nodata &  \nodata & 9      \\
 4112.71 & $-$1.70 &  0.05 &  67.8 &  41.1 &   6.3 &  \nodata &  \nodata &   6.8 &  \nodata &  \nodata &  \nodata &   9.3 &  28.8 &  \nodata & 9      \\
 4287.41 & $-$0.38 &  0.84 &  84.3 &  67.1 &   8.5 &  17.4 &   8.0 &  14.8 &  \nodata &  \nodata &  39.3 &  24.4 &  \nodata &  \nodata & 9      \\
 4453.32 & 0.01 &  1.50 &  71.1 &  46.7 &   4.9 &  10.5 &   3.9 &   7.3 &  \nodata &   8.4 &  28.3 &  11.5 &  24.0 &  \nodata & 9      \\
 4512.73 & $-$0.42 &  0.84 &  84.7 &  62.8 &   9.5 &  15.9 &   8.5 &  13.4 &   7.3 &  11.8 &  47.7 &  21.1 &  38.1 &  22.7 & 9      \\
 4518.02 & $-$0.26 &  0.83 &  97.6 &  69.3 &  12.9 &  23.1 &  11.5 &  17.5 &   9.8 &  15.6 &  59.8 &  26.1 &  46.1 &  26.5 & 9      \\
 4533.24 &  0.54 &  0.85 & 132.8 &  97.6 &  42.8 &  56.7 &  36.7 &  50.2 &  33.6 &  44.9 &  91.8 &  62.3 &  80.6 &  60.6 & 9      \\
 4534.78 &  0.34 &  0.84 & 124.2 &  88.7 &  33.6 &  47.3 &  29.7 &  40.4 &  27.3 &  37.6 &  86.2 &  52.3 &  70.1 &  53.2 & 9      \\
 4548.76 & $-$0.29 &  0.83 &  97.3 &  65.8 &  12.4 &  20.7 &   9.9 &  16.9 &   8.2 &  14.7 &  51.6 &  25.0 &  42.8 &  26.0 & 9      \\
 4555.49 & $-$0.43 &  0.85 &  85.8 &  59.5 &   8.8 &  15.1 &   6.6 &  13.0 &   5.7 &  10.3 &  43.9 &  19.5 &  38.4 &  20.0 & 9      \\
 4617.27 &  0.45 &  1.75 &  58.3 &  45.3 &   5.3 &  12.4 &   5.4 &   8.4 &   4.8 &   9.1 &  29.0 &  12.8 &  23.5 &  17.3 & 9      \\
 4623.10 &  0.17 &  1.74 &  45.9 &  33.8 &  \nodata &   7.1 &   3.2 &   5.1 &  \nodata &   4.7 &  18.0 &   7.2 &  14.8 &  \nodata & 9      \\
 4645.19 & $-$0.50 &  1.89 &  \nodata &  16.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 9      \\
 4656.47 & $-$1.29 &  0.00 & 109.5 &  70.5 &  14.2 &  18.4 &  11.5 &  19.0 &   8.0 &  13.6 &  73.5 &  29.2 &  51.4 &  25.0 & 9      \\
 4681.91 & $-$1.01 &  0.05 & 125.0 &  81.9 &  22.3 &  27.1 &  16.8 &  27.7 &  13.2 &  20.0 &  83.3 &  39.2 &  60.0 &  33.3 & 9      \\
 4820.42 & $-$0.38 &  1.50 &  64.3 &  34.5 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  14.2 &  21.1 &  \nodata & 9      \\
 4840.87 & $-$0.45 &  0.90 &  80.6 &  \nodata &  11.2 &  15.1 &  \nodata &  11.5 &  \nodata &  \nodata &  42.8 &  15.7 &  33.1 &  20.4 & 9      \\
 4913.62 &  0.22 &  1.87 &  37.5 &  34.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  16.7 &  \nodata &  12.0 &   6.5 & 9      \\
 4981.73 &  0.56 &  0.85 & 153.4 & 106.5 &  49.8 &  66.2 &  42.9 &  61.7 &  40.3 &  52.2 & 112.4 &  70.8 &  92.3 &  70.6 & 9      \\
 4999.50 &  0.31 &  0.83 & 152.8 & 102.3 &  38.7 &  55.2 &  34.6 &  46.3 &  32.6 &  39.3 & 104.1 &  59.8 &  85.9 &  57.5 & 9      \\
 5016.16 & $-$0.51 &  0.85 &  88.8 &  60.0 &  11.5 &  \nodata &  \nodata &  10.3 &  \nodata &  \nodata &  50.3 &  18.0 &  35.0 &  19.7 & 9      \\
 5020.03 & $-$0.35 &  0.84 & 101.6 &  71.4 &  11.7 &  20.1 &  11.8 &  16.5 &  12.2 &  17.8 &  61.3 &  27.2 &  47.7 &  27.9 & 9      \\
 5022.87 & $-$0.37 &  0.83 & 103.0 &  68.7 &  \nodata &  19.1 &  12.4 &  16.0 &   8.7 &  \nodata &  59.9 &  26.1 &  45.7 &  26.4 & 9      \\
 5024.84 & $-$0.54 &  0.82 &  95.0 &  61.0 &  \nodata &  17.3 &   9.4 &  13.0 &  \nodata &  \nodata &  52.5 &  20.8 &  39.4 &  21.0 & 9      \\
 5036.47 &  0.19 &  1.44 &  89.5 &  56.2 &  \nodata &  \nodata &  \nodata &  13.1 &  \nodata &  \nodata &  43.1 &  17.7 &  33.0 &  17.4 & 9      \\
 5038.40 &  0.07 &  1.43 &  79.3 &  58.1 &  \nodata &  \nodata &  \nodata &  10.5 &  \nodata &  \nodata &  41.4 &  14.7 &  31.0 &  19.7 & 9      \\
 5039.96 & $-$1.07 &  0.21 & 131.2 &  80.7 &  23.9 &  28.8 &  17.1 &  29.0 &  14.1 &  21.7 &  88.0 &  43.9 &  69.9 &  38.1 & 9      \\
 5064.65 & $-$0.93 &  0.05 & 139.6 &  88.3 &  29.6 &  33.5 &  20.2 &  36.7 &  \nodata &  24.5 &  96.2 &  48.1 &  75.1 &  43.9 & 9      \\
 5071.47 & $-$1.00 &  1.46 &  16.0 &  10.8 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   3.5 &  \nodata & 9      \\
 5113.44 & $-$0.72 &  1.44 &  32.5 &  14.5 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   9.7 &   3.9 &   4.5 &  \nodata & 9      \\
 5147.48 & $-$1.95 &  0.00 &  83.6 &  41.6 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  35.9 &   7.7 &  22.2 &  \nodata & 9      \\
 5173.74 & $-$1.06 &  0.00 & 146.4 &  89.9 &  26.0 &  29.5 &  18.1 &  29.5 &  \nodata &  19.6 &  95.0 &  45.4 &  73.1 &  37.8 & 9      \\
 5192.97 & $-$0.95 &  0.02 & 166.3 &  94.0 &  31.8 &  33.4 &  20.8 &  35.7 &  18.5 &  35.8 & 108.4 &  51.2 &  83.5 &  46.9 & 9      \\
 5210.39 & $-$0.82 &  0.05 & 152.8 &  95.2 &  34.5 &  40.4 &  25.3 &  42.4 &  20.7 &  34.6 & 106.3 &  55.7 &  81.2 &  50.2 & 9      \\
 5219.70 & $-$2.23 &  0.02 &  60.3 &  25.3 &  \nodata &  \nodata &  \nodata &   6.7 &  \nodata &  \nodata &  23.2 &   5.8 &  13.6 &  \nodata & 9      \\
 5224.30 &  0.13 &  2.13 &  30.4 &  18.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   9.9 &  \nodata & 10     \\
 5426.26 & $-$2.95 &  0.02 &  18.8 &   7.2 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   7.0 &  \nodata &   4.3 &  \nodata & 9      \\
 5866.45 & $-$0.78 &  1.07 &  63.0 &  36.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  24.8 &   7.1 &  15.9 &   7.8 & 9      \\
 5978.54 & $-$0.44 &  1.89 &  18.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   1.1 &   6.1 &  \nodata & 9      \\
 6258.10 & $-$0.29 &  1.44 &  57.8 &  36.8 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  24.6 &   6.7 &  17.4 &  11.5 & 9      \\
 6261.10 & $-$0.42 &  1.43 &  54.8 &  31.7 &  \nodata &  \nodata &  \nodata &   6.1 &  \nodata &  \nodata &  19.0 &   7.2 &  14.0 &  10.8 & 9      \\
 6556.06 & $-$1.01 &  1.46 &  \nodata &  13.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   5.8 &  \nodata &   3.0 &  \nodata & 9      \\
\multicolumn{16}{c}{{TiII}} \\
 4056.19 & $-$3.30 &  0.61 &  78.0 &  56.0 &  17.6 &  24.7 &  12.0 &  21.2 &   6.9 &   9.0 &  47.6 &  27.7 &  45.7 &  \nodata & 11     \\
 4394.06 & $-$1.77 &  1.22 & 127.6 & 101.6 &  54.5 &  71.4 &  46.2 &  63.9 &  40.5 &  42.2 &  97.6 &  74.7 &  91.1 &  56.0 & 11     \\
 4395.04 & $-$0.51 &  1.08 &  \nodata &  \nodata & 137.1 & 138.8 & 111.1 &  \nodata &  \nodata &  98.7 &  \nodata &  \nodata & 172.1 & 112.9 & 11     \\
 4395.84 & $-$1.97 &  1.24 &  98.6 &  \nodata &  40.5 &  57.8 &  32.1 &  46.3 &  28.6&  30.3 &  84.1 &  54.9 &  73.8 &  47.2 & 11     \\
 4398.29 & $-$2.78 &  1.22 &  68.0 &  \nodata &  10.2 &  19.0 &   5.8 &  10.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 11     \\
 4409.52 & $-$2.57 &  1.23 &  \nodata &  59.8 &  17.1 &  28.9 &  14.3 &  21.4 &  \nodata &   9.3 &  \nodata &  29.5 &  \nodata &  \nodata & 11     \\
 4443.80 & $-$0.70 &  1.08 & 200.4 & 147.6 & 116.3 & 128.8 & 102.4 & 115.9 &  96.2 &  90.8 & 159.9 & 119.1 & 143.6 & 108.1 & 11     \\
 4444.56 & $-$2.21 &  1.12 & 137.3 &  85.8 &  38.4 &  53.6 &  30.4 &  44.4 &  23.0 &  25.3 &  88.8 &  54.1 &  78.3 &  44.9 & 11     \\
 4450.48 & $-$1.51 &  1.08 &  \nodata & 122.1 &  81.0 &  94.6 &  68.6 &  84.6 &  62.2 &  59.0 & 123.0 &  92.8 &  \nodata &  83.4 & 11     \\
 4468.49 & $-$0.60 &  1.13 & 216.9 & 148.3 & 118.6 & 135.7 & 104.4 & 117.0 &  
96.1 &  93.1 & 171.5 & 123.9 & 147.6 & 113.1 & 11     \\
 4493.52 & $-$2.83 &  1.08 &  76.5 &  54.3 &  14.0 &  23.4 &  10.2 &  17.1 &   8.1 &   7.6 &  49.4 &  24.9 &  40.5 &  17.7 & 11     \\
 4501.27 & $-$0.76 &  1.12 & 202.5 &  \nodata & 116.0 & 131.6 &  99.9 & 118.2 &  94.3 &  85.6 & 160.6 & 120.5 & 145.1 & 106.8 & 11     \\
 4583.41 & $-$2.87 &  1.16 &  67.8 &  47.4 &  13.2 &  19.2 &   9.3 &  15.8 &   6.5 &   7.2 &  41.3 &  21.0 &  40.4 &  19.7 & 11     \\
 4609.27 & $-$3.43 &  1.18 &  \nodata &  23.3 &  \nodata &   7.7 &  \nodata &   5.3 &  \nodata &  \nodata &  \nodata &   7.4 &  15.6 &  \nodata & 11     \\
 4636.32 & $-$3.23 &  1.16 &  49.2 &  28.2 &   6.7 &  11.2 &   5.0 &   8.1 &   2.7 &   3.3 &  29.3 &  12.1 &  20.2 &  \nodata & 11     \\
 4657.20 & $-$2.32 &  1.24 &  95.1 &  71.6 &  29.0 &  41.6 &  22.4 &  33.9 &  17.7 &  17.6 &  73.1 &  46.2 &  62.8 &  35.0 & 11     \\
 4708.66 & $-$2.37 &  1.24 &  86.6 &  69.4 &  25.9 &  40.2 &  20.9 &  31.9 &  15.7 &  16.4 &  66.5 &  39.6 &  57.5 &  30.0 & 11     \\
 4719.52 & $-$3.28 & 1.24 & \nodata & 21.4 & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 11 \\ 
 4764.53 & $-$2.77 &  1.24 &  70.3 &  49.7 &  \nodata &  \nodata &  \nodata &  17.9 &  \nodata &  \nodata &  44.6 &  22.9 &  40.7 &  20.4 & 11     \\
 4798.53 & $-$2.67 &  1.08 &  \nodata &  65.7 &  25.9 &  34.1 &  16.7 &  29.7 &  16.5 &  \nodata &  64.4 &  38.6 &  58.2 &  33.1 & 11     \\
 5005.17 & $-$2.73 &  1.57 &  41.8 &  28.5 &  \nodata &   9.3 &  \nodata &  \nodata &  \nodata &  \nodata &  25.4 &  15.6 &  20.2 &   8.8 & 11     \\
 5336.79 & $-$1.63 &  1.58 & 117.4 &  86.3 &  43.1 &  63.4 &  32.8 &  53.6 &  26.6 &  31.0 &  91.8 &  61.6 &  80.8 &  54.2 & 11     \\
\multicolumn{16}{c}{{VI}} \\
 3864.86\tablenotemark{b} & $-$0.44 &  0.02 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   6.2 &  \nodata &  \nodata &  \nodata &   7.3 &  \nodata &  \nodata & 12     \\
 4111.78\tablenotemark{b} &  0.41 &  0.30 &  \nodata &  73.6 &  11.3 &  18.0 &   8.1 &  19.0 &   8.0 &  14.5 &  49.0 &  23.4 &  48.2 &  \nodata & 12     \\
 4379.23\tablenotemark{b} &  0.55 &  0.30 & 121.9 &  95.6 &  19.5 &  29.0 &  13.8 &  29.5 &  12.4 &  23.4 &  84.6 &  36.5 &  66.4 &  35.6 & 13     \\
 4389.98\tablenotemark{b} &  0.27 &  0.28 & 102.7 &  68.7 &  11.3 &  15.9 &  \nodata &  20.3 &  \nodata &  \nodata &  55.9 &  27.2 &  49.8 &  \nodata & 13     \\
 4459.75 & $-$0.50 &  0.29 &  49.9 &  29.0 &  \nodata &   3.4 &  \nodata &  \nodata &  \nodata &  \nodata &  21.1 &   4.3 &  13.5 &  \nodata & 12     \\
 4577.18\tablenotemark{b} & $-$1.05 &  0.00 &  41.8 &  20.5 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  11.7 &   3.6 &   8.4 &  \nodata & 12     \\
\multicolumn{16}{c}{{VII}} \\
 3517.30\tablenotemark{b} & $-$0.21 & 1.13  &  \nodata &  \nodata &  54.9 &  \nodata & 45.5 
&  67.6 &  39.0 &  45.3 &  \nodata &   65.5 &  \nodata &  \nodata & 
14 \\
 3545.19\tablenotemark{b}  & $-$0.26 & 1.10 &  \nodata &  \nodata &  49.3 & \nodata & 41.1 
&  60.0 &  36.9 &  43.9 &  \nodata &   64.7 &  \nodata &  \nodata & 
14 \\ 
 3592.02\tablenotemark{b} & $-$0.26 & 1.10 &  \nodata &  \nodata &  54.2 & \nodata & 42.2 
&  62.3 &  37.5 &  41.3 &  \nodata &   64.6 &  \nodata &  \nodata & 
14 \\
 3732.75\tablenotemark{b} & $-$0.35 & 1.56 &  \nodata &  \nodata &  34.5 & \nodata &  29.3 
&  35.4 &  26.9 & 30.9 &  \nodata &   \nodata &  \nodata &  \nodata & 
14  \\
 3884.84\tablenotemark{b} & $-$1.41 &  1.79 &  \nodata &  \nodata &  \nodata &   8.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   5.5 &  \nodata &  \nodata & 14     \\
 3951.96\tablenotemark{b} & $-$0.78 &  1.48 &  \nodata &  69.8 &  23.0 &  47.8 &  17.9 &  35.4 &  13.6 &  21.0 &  \nodata&  41.6 &  66.5 &  \nodata & 14     \\
 4036.78\tablenotemark{b} & $-$1.59 &  1.48 &  \nodata &  38.4 &  \nodata &  14.4 &  \nodata &  11.3 &  \nodata &   7.5 &  31.3 &  13.9 &  26.4 &  \nodata & 14     \\
\multicolumn{16}{c}{{CrI}} \\
 4254.35\tablenotemark{a} & $-$0.11 &  0.00 & 234.5 & 155.9 & 108.7 & 116.5 &  \nodata & 115.4 &  87.4 &  97.2 & 163.5 & 115.3 & 155.0 & 118.2 & 15     \\
 4351.06 & $-$1.45 &  0.97 &  \nodata &  \nodata &   8.5 &  \nodata &   4.0 &  12.7 &   7.3 &  13.4 &  \nodata &  \nodata &  \nodata &  \nodata & 15     \\
 4545.96 & $-$1.38 &  0.94 &  93.7 &  64.8 &   9.8 &  18.9 &   6.3 &  14.5 &   6.1 &  14.2 &  51.0 &  20.8 &  48.0 &  31.0 & 15     \\
 4591.40 & $-$1.76 &  0.97 &  73.4 &  48.4 &  \nodata &   8.5 &  \nodata &   7.2 &  \nodata &   6.3 &  28.4 &   9.9 &  30.9 &  18.9 & 15     \\
 4600.76 & $-$1.26 &  1.00 &  98.5 &  63.5 &  10.2 &  20.8 &   6.9 &  15.2 &   5.1 &  13.9 &  53.0 &  25.4 &  51.5 &  30.0 & 15,16  \\
 4616.13 & $-$1.20 &  0.98 & 100.1 &  69.9 &  13.2 &  24.1 &   8.2 &  17.8 &   8.1 &  17.0 &  58.2 &  27.1 &  57.1 &  38.7 & 15,16  \\
 4626.18 & $-$1.32 &  0.97 &  93.6 &  65.4 &   9.8 &  19.2 &   6.7 &  14.5 &   6.1 &  14.0 &  52.1 &  21.4 &  49.0 &  27.6 & 15,16  \\
 4646.17 & $-$0.72 &  1.03 & 116.3 &  84.8 &  26.1 &  40.3 &  19.1 &  35.1 &  16.7 &  31.6 &  75.9 &  42.3 &  73.0 &  54.3 & 15,16  \\
 4651.29 & $-$1.46 &  0.98 &  87.6 &  58.9 &   6.9 &  14.9 &   5.2 &  11.6 &  \nodata &  10.2 &  46.2 &  17.5 &  40.3 &  22.4 & 15,16  \\
 5247.57 & $-$1.64 &  0.96 &  95.3 &  57.5 &   7.9 &   9.7 &   5.8 &   7.9 &  \nodata &   7.0 &  45.6 &  15.9 &  40.3 &  \nodata & 15,16  \\
 5296.70 & $-$1.40 &  0.98 & 104.8 &  69.7 &  11.5 &  \nodata &  11.3 &  16.8 &  \nodata &  \nodata &  57.2 &  23.0 &  52.5 &  30.0 & 15,16  \\
 5300.75 & $-$2.13 &  0.98 &  58.0 &  31.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  21.5 &  \nodata &  17.7 &   8.7 & 15,16  \\
 5345.81 & $-$0.98 &  1.00 & 131.2 &  90.5 &  21.0 &  37.6 &  15.9 &  33.9 &  11.8 &  20.9 &  84.1 &  41.5 &  76.7 &  47.5 & 15,16  \\
 5348.33 & $-$1.29 &  1.00 & 109.9 &  71.8 &  11.9 &  22.0 &  \nodata &  19.0 &  \nodata &  \nodata &  62.1 &  25.8 &  58.1 &  34.4 & 15,16  \\
 5409.80 & $-$0.72 &  1.03 & 149.0 & 102.8 &  33.2 &  48.7 &  21.7 &  43.7 &  16.5 &  34.4 &  96.1 &  53.3 &  90.3 &  60.5 & 15,16  \\
 4652.17 & $-$1.03 &  1.00 & 105.0 &  76.2 &  16.8 &  29.3 &  11.9 &  23.3 &   9.7 &  22.0 &  71.4 &  31.4 &  62.3 &  42.5 & 16     \\
\multicolumn{16}{c}{{CrII}} \\
 4558.66 & $-$0.66 &  4.07 &  \nodata &  61.4 &  13.4 &  38.9 &  10.2 &  19.4 &   8.6 &  18.8 &  41.4 &  25.7 &  50.3 &  36.3 & 12     \\
 4634.10 & $-$1.24 &  4.07 &  38.7 &  30.8 &   2.9 &  15.3 &  \nodata &   5.4 &  \nodata &   6.7 &  \nodata &   8.4 &  23.5 &  18.0 & 12     \\
\multicolumn{16}{c}{{MnI}} \\
 3823.51 &  0.06 &  2.14 &  \nodata &  \nodata &  12.4 &  26.2 &   6.7 &  18.8 &   8.5 &  20.8 &  \nodata &  21.4 &  \nodata &  \nodata & 17     \\
 4030.76\tablenotemark{a} & $-$0.47 &  0.00 &  \nodata & 183.0 & 117.3 & 137.6 &  93.6 & 134.6 &  90.7 & 108.9 & 190.9 &  \nodata & 175.0 & 129.2 & 17     \\
 4033.07\tablenotemark{a} & $-$0.62 &  0.00 & 207.3 & 171.3 & 108.8 & 123.4 &  84.0 & 125.0 &  78.4 &  95.9 & 177.8 & 121.1 & 171.6 & 118.7 & 17     \\
 4034.49\tablenotemark{a} & $-$0.81 &  0.00 & 186.5 & 170.1 &  96.3 & 106.7 &  73.3 & 113.2 &  75.5 &  91.1 & 155.5 & 118.0 & 168.5 & 123.3 & 17     \\
 4055.55 & $-$0.07 &  2.14 & 102.8 &  68.9 &   7.3 &  29.4 &   7.6 &  18.7 &  \nodata &  17.4 &  45.2 &  24.3 &  64.3 &  32.6 & 17     \\
 4082.94 & $-$0.35 &  2.18 &  \nodata &  45.9 &   6.7 &  11.9 &  \nodata &  12.7 &  \nodata &   9.8 &  26.4 &  11.2 &  25.6 &  \nodata & 17     \\
 4709.72 & $-$0.34 &  2.89 &  38.7 &  17.8 &  \nodata &   5.0 &  \nodata &  \nodata &  \nodata &  \nodata &  13.5 &   5.3 &  13.4 &  \nodata & 17     \\
 4754.04 & $-$0.09 &  2.28 &  93.4 &  69.3 &   7.5 &  27.6 &  \nodata &  22.8 &  \nodata &  \nodata &  44.6 &  21.8 &  55.4 &  29.4 & 17     \\
 4761.53 & $-$0.14 &  2.95 &  22.8 &  17.8 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  10.4 &  \nodata & 17     \\
 4783.42 &  0.04 &  2.30 & 101.7 &  76.3 &  17.0 &  26.4 &  \nodata &  21.7 &  \nodata &  \nodata &  55.8 &  27.2 &  62.1 &  36.5 & 17     \\
 5432.55 & $-$3.80 &  0.00 &  50.9 &  13.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  11.7 &  \nodata &  10.0 &  \nodata & 17     \\
 6021.80 &  0.03 &  3.08 &  40.7 &  25.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  13.4 &   4.5 &  16.5 &   7.7 & 17     \\
 4070.28 & $-$0.95 &  2.19 &  \nodata &  21.7 &  \nodata &   5.9 &  \nodata &  \nodata &  \nodata &  \nodata &  18.8 &   3.8 &  14.5 &  \nodata & 18     \\
\multicolumn{16}{c}{{MnII}} \\
 3441.99 & $-$0.27 & 1.78 & \nodata & \nodata & 81.5 & 114.1 & 70.3 & 
96.8 & 72.6 & 80.8 & \nodata & 91.6 & \nodata & \nodata & 19 \\
 3460.32 & $-$0.54 & 1.81 & \nodata & \nodata & 77.0 & \nodata & 60.0 & 
\nodata & 61.8 & 65.7 & \nodata & \nodata & \nodata & \nodata & 19 \\
 3488.68 & $-$0.86 & 1.85 & \nodata & \nodata & 56.7 & \nodata & 53.8 & 
78.5 & 52.7 & 60.2 & \nodata & 74.0 & \nodata & \nodata & 19 \\
 3497.53 & $-$1.33 & 1.85 & \nodata & \nodata & \nodata & 73.2 & 33.4 & 
\nodata & 31.6 & 41.9 & \nodata & 55.0 & \nodata & \nodata & 19 \\
\multicolumn{16}{c}{{FeI}} \\
 3246.48 & $-$1.41 &  2.59 & \nodata & \nodata & \nodata & 20.6 & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata  & \nodata & \nodata & 20 \\
 3406.79 & $-$1.04 &  2.22 & \nodata & \nodata & \nodata & 73.0 & \nodata & 
\nodata & 35.3 & 53.0 & \nodata & \nodata & \nodata & \nodata & 20 \\
 3442.26 & $-$1.35 &  2.28 & \nodata & \nodata & \nodata & 41.6 & 18.7  & 
35.7 & 27.0 & 34.8 & \nodata & 42.8 & \nodata & \nodata  & 22 \\
 3617.78 & $-$0.05 &  3.02 & \nodata & \nodata & 38.9 & 59.0 & 36.0 & 
49.9 & 35.1 & 50.2 & \nodata & 57.4 & \nodata & \nodata  & 20 \\
 3628.81 & $-$2.21 &  2.99 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 20 \\
 3633.83 & $-$1.54 &  2.99 & \nodata & \nodata & \nodata & 12.3 & \nodata & 
9.2 & \nodata & 13.6 & \nodata & 12.3 & \nodata & \nodata   & 20 \\
 3709.25 & $-$0.61 &  0.92 & \nodata & \nodata & 144.1 & \nodata & 119.9 & 
\nodata & 123.6 & 131.6 & \nodata & \nodata & \nodata & \nodata  & 22 \\
 3715.91 & $-$1.53 &  2.28 & \nodata & \nodata & 32.1 & 45.0 & 22.3 & 
42.2 & 21.0 & 33.3 & \nodata & \nodata & \nodata & \nodata &  22 \\
 3760.05 & $-$0.81 &  2.40 &  \nodata &  \nodata &  54.8 &  70.8 &  44.8 &  65.7 &  45.7 &  55.0 &  \nodata &  71.8 &  \nodata &  \nodata & 22     \\
 3767.19 & $-$0.35 &  1.01 &  \nodata &  \nodata & 146.8 & 153.6 & 131.3 &  \nodata & 124.9 & \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 22     \\
 3777.45 & $-$1.74 &  2.56 &  \nodata &  \nodata &  12.3 &  25.3 &   7.9 &  20.0 &   7.4 &  \nodata &  \nodata &  30.1 &  \nodata &  \nodata & 22     \\
 3786.67 & $-$2.16 &  1.01 &  \nodata &  \nodata &  91.3 &  \nodata &  70.1 &  91.5 &  67.2 & \nodata &  \nodata &  95.1 &  \nodata &  \nodata & 20     \\
 3787.88 & $-$0.82 &  1.01 &  \nodata &  \nodata & 129.5 & 132.2 & 111.2 & 149.1 & 109.3 & 113.2 &  \nodata & 137.2 &  \nodata &  \nodata & 22     \\
 3790.10 & $-$1.72 &  0.99 &  \nodata &  \nodata & 105.5 & 106.3 &  85.7 & 105.3 &  81.1 &  78.4 &  \nodata &  \nodata &  \nodata &  \nodata & 22     \\
 3808.73 & $-$1.12 &  2.56 &  \nodata &  \nodata &  34.6 &  53.8 &  30.1 &  46.0 &  26.4 &  43.0 &  \nodata &  56.5 &  \nodata &  \nodata & 22     \\
 3849.97 & $-$0.83 &  1.01 &  \nodata &  \nodata & 142.8 & 141.3 & 113.7 &  \nodata & 109.1 & 117.0 &  \nodata &  \nodata &  \nodata &  \nodata & 22     \\
 3856.37 & $-$1.25 &  0.05 &  \nodata &  \nodata & 168.8 & 165.5 & 140.8 &  \nodata & 141.3 & 142.0 &  \nodata &  \nodata &  \nodata &  \nodata & 22     \\
 3886.28 & $-$1.04 &  0.05 &  \nodata &  \nodata & 184.3 & 176.4 & 161.1 & 191.4 & 151.5 & 171.5 &  \nodata &  \nodata &  \nodata &  \nodata & 22     \\
 3887.05 & $-$1.10 &  0.92 &  \nodata &  \nodata & 131.6 & 129.1 & 111.9 & 131.2 & 103.8 & 102.8 &  \nodata & 137.0 &  \nodata &  \nodata & 22     \\
 3899.71 & $-$1.49 &  0.09 &  \nodata &  \nodata & 159.1 & 155.1 & 136.7 & 167.4 & 126.3 & 127.5 &  \nodata & 159.1 &  \nodata &  \nodata & 22     \\
 3916.74 & $-$0.56 &  3.24 &  80.3 &  62.2 &  16.8 &  40.2 &  16.5 &  29.2 &  15.9 &  33.1 &  \nodata &  33.7 &  \nodata &  \nodata & 20     \\
 3917.18 & $-$2.15 &  0.99 &  \nodata & 126.4 & 102.4 &  93.3 &  79.3 & 104.9 &  72.8 &  72.5 & 149.7 & 100.2 &  \nodata &  \nodata & 21     \\
 3920.26 & $-$1.71 &  0.12 &  \nodata &  \nodata & 151.7 & 146.7 & 130.0 &  \nodata & 121.4 & 115.4 &  \nodata &  \nodata &  \nodata &  \nodata & 22     \\
 3922.91 & $-$1.61 &  0.05 &  \nodata &  \nodata & 169.6 & 163.9 & 142.5 & 172.9 & 127.1 & 130.7 & 245.6 &  \nodata &  \nodata &  \nodata & 22     \\
 3949.96 & $-$1.25 &  2.17 &  \nodata &  93.6 &  56.1 &  69.1 &  42.2 &  68.6 &  43.4 &  53.6 &  96.0 &  70.2 &  94.4 &  \nodata & 21     \\
 4067.28 & $-$1.38 &  2.56 & 127.5 &  86.8 &  29.8 &  46.7 &  20.9 &  39.0 &  18.6 &  33.8 &  85.7 &  50.3 &  81.1 &  \nodata & 22     \\
 4072.51 & $-$1.44 &  3.43 &  28.6 &  35.5 &  \nodata &   8.0 &  \nodata &   4.4 &  \nodata &   5.3 &  \nodata &   6.7 &  18.0 &  \nodata & 20     \\
 4076.64 & $-$0.53 &  3.21 &  \nodata &  \nodata &  \nodata &  55.9 &  23.7 &  43.9 &  23.2 &  42.5 &  \nodata &  \nodata &  \nodata &  \nodata & 21     \\
 4091.55 & $-$2.07 &  2.83 &  \nodata &  29.7 &  \nodata &   5.8 &  \nodata &   5.1 &  \nodata &   5.6 &  \nodata &   8.3 &  20.9 &  \nodata & 20     \\
 4114.45 & $-$1.30 &  2.83 &  96.8 &  69.3 &  17.4 &  33.5 &  12.5 &  27.3 &  11.9 &  25.0 &  60.1 &  33.8 &  61.4 &  41.3 & 21     \\
 4132.91 & $-$1.00 &  2.84 &  \nodata &  88.9 &  28.3 &  48.4 &  21.6 &  39.9 &  19.7 &  37.7 &  89.3 &  48.4 &  72.6 &  49.2 & 21     \\
 4139.93 & $-$3.59 &  0.99 & 103.4 &  71.9 &  22.1 &  28.7 &  13.0 &  31.4 &  10.0 &  17.8 &  78.1 &  37.3 &  68.4 &  30.8 & 22     \\
 4147.68 & $-$2.06 &  1.49 & 138.8 & 102.7 &  70.3 &  72.8 &  51.7 &  77.7 &  50.8 &  54.7 & 118.5 &  82.1 & 105.1 &  67.8 & 22     \\
 4154.50 & $-$0.69 &  2.83 &  \nodata &  \nodata &  36.6 &  59.7 &  28.8 &  \nodata &  30.5 &  47.7 &  85.1 &  \nodata &  \nodata &  76.7 & 21     \\
 4156.81 & $-$0.81 &  2.83 &  \nodata &  \nodata &  40.5 &  64.7 &  31.3 &  52.3 &  31.9 &  49.2 &  \nodata &  62.3 &  \nodata &  68.7 & 21     \\
 4157.79 & $-$0.40 &  3.42 &  91.5 &  86.1 &  25.0 &  42.5 &  20.2 &  34.5 &  21.1 &  36.6 &  68.8 &  43.7 &  73.2 &  42.9 & 21     \\
 4174.92 & $-$2.93 &  0.92 & 142.3 & 102.2 &  67.6 &  64.8 &  44.9 &  75.7 &  41.6 &  47.7 & 125.6 &  80.0 &  \nodata &  \nodata & 22     \\
 4175.64 & $-$0.83 &  2.85 &  99.8 &  86.6 &  35.3 &  60.4 &  31.8 &  47.6 &  29.6 &  47.2 &  82.4 &  60.5 &  81.3 &  52.4 & 21     \\
 4182.39 & $-$1.18 &  3.02 &  77.2 &  73.2 &  11.8 &  26.1 &  10.2 &  20.9 &   7.9 &  21.9 &  48.6 &  28.1 &  55.7 &  32.8 & 21     \\
 4187.04 & $-$0.51 &  2.45 &  \nodata & 124.6 &  79.7 &  92.4 &  61.2 &  \nodata &  64.8 &  75.1 & 116.9 &  90.1 & 113.9 &  89.9 & 22     \\
 4195.34 & $-$0.49 &  3.33 &  \nodata & 105.7 &  29.2 &  47.0 &  26.5 &  42.0 &  \nodata &  41.4 &  \nodata &  \nodata &  81.6 &  60.5 & 21     \\
 4202.03 & $-$0.67 &  1.49 &  \nodata & 171.7 & 130.9 & 126.7 & 103.7 & 128.9 & 103.4 & 101.0 & 174.9 &  \nodata & 164.2 & 116.0 & 22     \\
 4216.19 & $-$3.32 &  0.00 &  \nodata & 127.0 & 109.5 &  97.5 &  84.3 & 111.0 &  82.3 &  75.4 & 160.8 &  \nodata & 138.9 &  85.7 & 22     \\
 4222.22 & $-$0.93 &  2.45 & 134.8 &  98.1 &  63.2 &  72.1 &  46.5 &  70.7 &  46.2 &  59.2 & 101.1 &  76.1 &  98.2 &  77.1 & 22     \\
 4224.18 & $-$0.51 &  3.37 &  \nodata &  79.3 &  \nodata &  42.6 &  18.0 &  31.2 &  16.8 &  34.5 &  56.0 &  42.7 &  \nodata &  51.4 & 21     \\
 4227.44 &  0.27 &  3.33 &  \nodata &  \nodata &  72.0 & 100.3 &  43.8 &  \nodata &  53.8 &  72.3 &  \nodata &  \nodata &  \nodata &  \nodata & 21     \\
 4233.61 & $-$0.56 &  2.48 &  \nodata & 116.0 &  \nodata &  88.3 &  59.0 &  83.1 &  60.0 &  71.8 &  \nodata &  89.3 & 112.9 &  82.1 & 22     \\
 4250.13 & $-$0.37 &  2.47 & 161.3 & 133.5 &  83.5 &  98.8 &  67.8 &  88.6 &  66.8 &  78.1 & 123.4 &  \nodata &  \nodata &  91.6 & 22     \\
 4260.47 &  0.14 &  2.40 &  \nodata &  \nodata & 107.6 & 122.3 &  91.2 & 112.0 &  93.1 & 105.6 &  \nodata & 119.7 &  \nodata & 126.2 & 20     \\
 4271.76 & $-$0.12 &  1.49 &  \nodata &  \nodata & 153.2 & 166.0 & 128.6 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 22     \\
 4282.41 & $-$0.78 &  2.17 & 195.5 & 123.5 &  81.7 &  90.9 &  66.1 &  88.3 &  66.4 &  72.8 &  \nodata &  \nodata &  \nodata &  87.0 & 21     \\
 4337.05 & $-$1.66 &  1.56 & 185.2 & 126.1 &  88.7 &  89.0 &  73.8 &  91.9 &  61.1 &  \nodata & 139.8 &  96.6 & 127.9 &  86.8 & 22     \\
 4347.24 & $-$5.46 &  0.00 &  86.0 &  46.3 &   9.3 &   6.6 &   5.4 &  12.9 &  \nodata &   3.3 &  \nodata &  17.3 &  \nodata &  \nodata & 22     \\
 4375.93 & $-$2.99 &  0.00 & 202.5 & 138.5 & 125.7 & 111.5 &  99.4 & 124.8 &  92.2 &  85.5 & 178.3 & 120.4 & 153.0 &  99.7 & 22     \\
 4383.55 &  0.24 &  1.49 &  \nodata &  \nodata & 177.1 & 189.5 & 150.2 & 187.3 & 147.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 22     \\
 4388.41 & $-$0.68 &  3.60 &  69.6 &  60.6 &  10.9 &  24.3 &   7.9 &  18.3 &   8.7 &  21.7 &  39.8 &  25.4 &  43.8 &  31.5 & 21     \\
 4389.24 & $-$4.54 &  0.05 & 146.2 &  82.8 &  43.5 &  32.3 &  22.6 &  50.0 &  17.2 &  21.7 & 107.1 &  57.1 &  87.6 &  41.9 & 22     \\
 4404.75 & $-$0.10 &  1.56 &  \nodata &  \nodata & 148.6 & 155.7 & 130.4 &  \nodata &  \nodata & 139.1 & 237.9 & 162.4 & 217.1 &  \nodata & 22     \\
 4415.13 & $-$0.62 &  1.61 &  \nodata &  \nodata & 127.8 & 128.1 & 106.9 &  \nodata & 104.1 & 111.8 &  \nodata & 131.7 & 170.3 & 127.5 & 21     \\
 4427.31 & $-$3.00 &  0.05 &  \nodata &  \nodata &  \nodata & 112.1 &  98.7 & 124.6 &  93.9 &  88.8 & 184.7 & 123.6 & 159.2 & 106.3 & 22     \\
 4430.62 & $-$1.62 &  2.22 & 119.3 &  98.0 &  \nodata &  53.3 &  29.4 &  52.3 &  27.1 &  43.7 &  92.7 &  59.4 &  88.4 &  62.3 & 22     \\
 4439.88 & $-$2.96 &  2.28 &  46.0 &  28.4 &   3.1 &   4.4 &  \nodata &   4.2 &  \nodata &   4.0 &  17.7 &   5.9 &  15.8 &  \nodata & 22     \\
 4443.20 & $-$1.04 &  2.86 &  \nodata &  89.4 &  26.7 &  42.3 &  18.2 &  34.6 &  18.1 &  34.0 &  74.5 &  44.6 &  72.7 &  50.0 & 21     \\
 4445.48 & $-$5.40 &  0.09 &  91.3 &  43.5 &   9.8 &   6.0 &   2.3 &  11.5 &  \nodata &   2.9 &  60.1 &  13.5 &  37.8 &  13.4 & 22     \\
 4447.73 & $-$1.34 &  2.22 & 150.5 & 112.9 &  58.4 &  73.4 &  44.1 &  68.5 &  42.6 &  58.1 & 113.1 &  77.4 & 104.4 &  72.5 & 21     \\
 4454.39 & $-$1.30 &  2.83 & 118.6 &  74.9 &  17.6 &  32.4 &  12.8 &  27.5 &  13.3 &  26.4 &  69.1 &  37.9 &  65.3 &  43.6 & 21     \\
 4461.65 & $-$3.17 &  0.09 &  \nodata & 120.9 & 122.0 &  99.4 &  88.6 & 115.5 &  86.9 &  77.7 & 170.4 & 109.7 &  \nodata &  88.5 & 22     \\
 4471.68 & $-$5.95 &  0.11 &  56.4 &  20.6 &  \nodata &  \nodata &  \nodata &   3.1 &  \nodata &  \nodata &  26.2 &   3.9 &  14.2 &  \nodata & 22     \\
 4484.23 & $-$0.86 &  3.60 &  70.3 &  64.4 &  10.5 &  24.5 &   7.2 &  16.8 &   7.7 &  18.7 &  42.3 &  23.3 &  42.0 &  29.0 & 21     \\
 4489.74 & $-$3.93 &  0.12 & 172.9 & 112.9 &  76.6 &  64.5 &  50.3 &  84.9 &  44.6 &  48.7 & 138.1 &  79.5 & 115.0 &  73.7 & 22     \\
 4494.57 & $-$1.10 &  2.20 & 170.9 & 124.6 &  75.5 &  84.7 &  56.9 &  85.1 &  56.0 &  65.3 & 127.2 &  86.8 & 115.0 &  82.8 & 22     \\
 4531.15 & $-$2.11 &  1.49 &  \nodata & 119.9 &  74.8 &  74.7 &  52.9 &  79.4 &  48.5 &  56.8 & 129.0 &  84.7 & 114.4 &  71.5 & 22     \\
 4602.01 & $-$3.11 &  1.61 &  96.5 &  64.2 &  13.7 &  17.7 &   7.4 &  19.4 &   6.7 &  12.5 &  62.3 &  27.4 &  53.8 &  25.5 & 22     \\
 4602.94 & $-$2.18 &  1.49 & 161.2 & 107.2 &  71.5 &  76.7 &  51.7 &  80.8 &  46.3 &  57.0 & 126.4 &  82.7 & 111.0 &  78.6 & 22     \\
 4630.13 & $-$2.59 &  2.28 &  91.8 &  59.7 &   9.3 &  15.0 &   5.7 &  13.1 &   5.2 &  10.3 &  51.3 &  19.9 &  44.4 &  21.1 & 21     \\
 4632.92 & $-$2.90 &  1.61 & 126.3 &  86.1 &  23.8 &  29.1 &  13.9 &  34.0 &  12.4 &  19.3 &  86.3 &  40.6 &  73.1 &  42.5 & 21     \\
 4635.85 & $-$2.36 &  2.84 &  41.5 &  26.3 &   1.5 &   4.6 &   1.6 &   2.9 &  \nodata &   3.4 &  \nodata &   4.8 &  14.0 &  \nodata & 21     \\
 4643.46 & $-$1.15 &  3.64 &  47.1 &  36.5 &  \nodata &   8.1 &  \nodata &   4.8 &   2.3 &   6.8 &  16.1 &   7.5 &  21.2 &  13.6 & 21     \\
 4647.43 & $-$1.35 &  2.94 & 104.4 &  71.3 &  15.9 &  30.6 &  10.4 &  24.2 &   9.3 &  22.4 &  67.6 &  33.1 &  58.3 &  39.1 & 21     \\
 4673.17 & $-$1.06 &  3.65 &  59.9 &  45.0 &  \nodata &   9.5 &  \nodata &   6.7 &  \nodata &   7.3 &  19.6 &   6.9 &  22.8 &  \nodata & 21     \\
 4678.85 & $-$0.83 &  3.59 &  76.2 &  64.9 &  10.1 &  25.9 &   8.3 &  17.6 &   8.5 &  20.7 &  42.7 &  24.8 &  46.6 &  34.6 & 21     \\
 4683.57 & $-$2.32 &  2.83 &  35.6 &  25.3 &  \nodata &   4.3 &  \nodata &  \nodata &  \nodata &  \nodata &  12.1 &   4.2 &  13.6 &  \nodata & 21     \\
 4690.14 & $-$1.64 &  3.68 &  26.8 &  20.0 &  \nodata &   3.9 &  \nodata &  \nodata &  \nodata &  \nodata &  10.8 &   3.0 &  10.1 &   7.8 & 21     \\
 4691.41 & $-$1.52 &  2.98 & 115.4 &  89.4 &  12.3 &  24.5 &   9.0 &  19.7 &   8.3 &  18.5 &  60.4 &  28.0 &  56.7 &  40.5 & 21     \\
 4710.28 & $-$1.61 &  3.00 &  \nodata &  73.4 &   8.3 &  17.6 &   6.8 &  14.4 &   5.1 &  13.7 &  48.1 &  19.8 &  46.8 &  27.0 & 21     \\
 4733.60 & $-$2.95 &  1.49 & 124.8 &  81.1 &  31.1 &  34.0 &  17.5 &  40.2 &  \nodata &  \nodata &  92.7 &  42.6 &  76.0 &  42.7 & 22     \\
 4736.77 & $-$0.75 &  3.20 & 117.0 &  87.4 &  29.5 &  50.3 &  22.5 &  43.6 &  26.5 &  35.2 &  84.2 &  50.0 &  75.4 &  55.3 & 21     \\
 4800.65 & $-$1.03 &  4.12 &  25.3 &  17.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   7.2 &  \nodata & 21     \\
 4859.74 & $-$0.76 &  2.86 & 135.5 &  97.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  92.8 &  67.0 &  \nodata &  \nodata & 21     \\
 4871.32 & $-$0.36 &  2.85 & 157.9 & 117.4 &  64.3 &  81.5 &  51.7 &  81.2 &  57.8 &  62.2 & 124.4 &  90.2 & 109.2 &  85.4 & 21     \\
 4872.14 & $-$0.57 &  2.87 & 158.4 & 113.3 &  52.1 &  72.4 &  49.2 &  67.8 &  41.9 &  54.4 & 107.5 &  74.8 & 103.6 &  82.6 & 21     \\
 4890.75 & $-$0.39 &  2.86 & 159.8 & 120.9 &  61.8 &  83.3 &  53.2 &  81.1 &  48.4 &  68.4 & 118.4 &  85.6 & 112.6 &  84.8 & 21     \\
 4891.49 & $-$0.11 &  2.84 & 163.3 & 130.6 &  75.7 &  95.6 &  64.1 &  92.5 &  66.3 &  73.2 & 127.1 &  96.7 & 120.6 &  99.4 & 21     \\
 4903.31 & $-$0.93 &  2.87 & 129.6 &  94.4 &  37.8 &  52.7 &  26.8 &  50.3 &  26.7 &  42.8 &  93.6 &  60.7 &  85.2 &  61.3 & 21     \\
 4918.99 & $-$0.34 &  2.85 & 156.9 & 122.5 &  64.9 &  77.2 &  54.1 &  85.0 &  54.7 &  71.4 & 117.3 &  87.9 & 110.6 &  88.7 & 21     \\
 4920.50 &  0.07 &  2.82 &  \nodata & 160.4 &  89.1 & 112.0 &  73.2 & 102.5 &  72.7 &  86.5 & 169.5 & 111.8 & 152.3 & 110.6 & 21     \\
 4924.77 & $-$2.25 &  2.28 & 109.8 &  76.4 &  18.6 &  32.2 &   9.7 &  27.8 &  \nodata &  17.8 &  69.8 &  37.4 &  63.4 &  36.9 & 20     \\
 4930.32 & $-$1.20 &  3.96 &  31.5 &  22.3 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   9.2 &  \nodata & 20  \\
 4938.81 & $-$1.08 &  2.86 & 117.2 &  85.1 &  28.2 &  47.1 &  19.2 &  40.0 &  22.5 &  29.3 &  83.2 &  50.8 &  74.9 &  56.3 & 21     \\
 4939.69 & $-$3.30 &  0.86 & 160.1 &  98.8 &  58.3 &  55.6 &  36.0 &  73.4 &  31.2 &  37.0 & 121.3 &  72.7 & 102.1 &  63.8 & 22     \\
 4994.13 & $-$3.04 &  0.92 & 168.2 & 104.8 &  69.8 &  70.1 &  48.1 &  81.5 &  43.5 &  50.4 & 133.0 &  86.9 & 111.9 &  74.7 & 22     \\
 5006.12 & $-$0.66 &  2.83 & 145.1 & 111.8 &  58.8 &  67.4 &  43.1 &  70.7 &  41.3 &  56.2 & 106.8 &  80.8 & 104.8 &  78.2 & 20     \\
 5039.25 & $-$1.57 &  3.35 &  69.6 &  47.6 &  \nodata &  16.0 &  \nodata &  \nodata &  \nodata &  \nodata &  31.0 &   7.7 &  30.3 &  19.0 & 21     \\
 5041.07 & $-$3.09 &  0.95 &  \nodata &  \nodata &  70.6 &  \nodata &  46.5 &  94.8 &  41.5 &  51.8 & 140.8 &  88.6 & 124.0 &  81.8 & 21     \\
 5048.44 & $-$1.03 &  3.94 &  30.8 &  29.3 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  11.0 &  \nodata &  11.0 &  10.3 & 21     \\
 5049.82 & $-$1.34 &  2.28 & 159.2 & 110.2 &  56.8 &  67.6 &  39.7 &  72.9 &  49.7 &  50.7 & 119.3 &  76.9 & 105.3 &  78.5 & 20     \\
 5051.64 & $-$2.76 &  0.92 & 196.1 & 124.7 &  89.8 &  85.1 &  64.9 & 101.5 &  59.5 &  59.7 & 152.7 & 102.1 & 132.8 &  87.4 & 22     \\
 5068.77 & $-$1.04 &  2.93 & 112.5 &  85.9 &  26.0 &  41.8 &  17.0 &  40.1 &  17.7 &  36.2 &  82.3 &  47.5 &  72.1 &  53.2 & 21     \\
 5079.23 & $-$2.03 &  2.20 &  \nodata &  92.3 &  33.8 &  39.7 &  17.8 &  45.3 &  \nodata &  \nodata &  90.3 &  51.6 &  81.4 &  50.8 & 22     \\
 5079.74 & $-$3.18 &  0.99 &  \nodata & 109.7 &  58.4 &  54.5 &  39.2 &  71.3 &  30.0 &  38.3 & 126.5 &  74.6 & 109.0 &  65.7 & 22     \\
 5083.34 & $-$2.92 &  0.96 & 172.6 & 109.1 &  77.4 &  68.9 &  52.5 &  87.2 &  42.3 &  48.8 & 137.8 &  87.9 & 116.1 &  76.3 & 22     \\
 5123.72 & $-$3.03 &  1.01 & 181.1 & 112.4 &  65.4 &  64.9 &  41.2 &  75.6 &  35.6 &  44.3 & 135.2 &  83.4 & 116.1 &  74.3 & 22     \\
 5127.36 & $-$3.27 &  0.92 & 166.0 & 101.1 &  60.7 &  57.5 &  34.2 &  66.4 &  27.2 &  35.5 & 123.9 &  73.3 & 106.9 &  62.3 & 22     \\
 5141.73 & $-$1.96 &  2.42 &  96.5 &  65.5 &  15.6 &  23.6 &  \nodata &  16.9 &   8.1 &  11.8 &  60.0 &  25.2 &  50.5 &  28.3 & 20     \\
 5142.93 & $-$3.08 &  0.96 &  \nodata & 137.0 &  68.6 &  67.6 &  40.3 &  80.6 &  32.3 &  51.0 & 138.4 &  82.3 & 122.7 &  75.2 & 20     \\
 5151.92 & $-$3.28 &  1.01 & 160.8 &  98.8 &  47.3 &  \nodata &  29.1 &  61.2 &  25.2 &  28.0 & 117.5 &  65.7 &  98.9 &  \nodata & 22     \\
 5166.29 & $-$4.16 &  0.00 & 195.1 & 114.9 &  83.9 &  66.9 &  55.0 &  92.6 &  44.9 &  48.3 & 154.7 &  92.1 & 124.7 &  74.7 & 22     \\
 5171.60 & $-$1.75 &  1.49 & 192.2 & 133.3 &  96.9 &  99.6 &  78.7 & 109.8 &  73.2 &  74.6 & 151.9 & 109.6 & 133.7 &  95.6 & 22     \\
 5191.45 & $-$0.55 &  3.03 & 171.5 & 116.7 &  43.6 &  66.0 &  36.1 &  55.1 &  \nodata &  53.8 & 112.3 &  73.2 & 104.9 &  72.9 & 21     \\
 5192.34 & $-$0.42 &  2.99 & 152.9 & 114.9 &  54.0 &  69.0 &  42.4 &  77.3 &  43.4 &  64.2 & 110.9 &  78.4 & 103.7 &  78.0 & 21     \\
 5194.94 & $-$2.05 &  1.56 &  \nodata & 116.1 &  79.3 &  77.5 &  56.7 &  87.2 &  52.9 &  56.4 & 136.8 &  \nodata & 118.3 &  82.9 & 22     \\
 5198.71 & $-$2.09 &  2.22 & 121.4 &  81.6 &  25.3 &  \nodata &  14.9 &  33.5 &  15.1 &  30.0 &  88.4 &  44.6 &  65.7 &  \nodata & 22     \\
 5215.18 & $-$0.87 &  3.27 & 103.3 &  74.3 &  19.0 &  28.2 &  11.8 &  26.6 &  12.9 &  29.0 &  62.0 &  35.8 &  59.0 &  40.8 & 20     \\
 5216.28 & $-$2.11 &  1.61 & 165.6 & 111.9 &  70.8 &  74.8 &  48.8 &  80.4 &  49.4 &  55.7 & 129.4 &  85.5 & 112.3 &  77.3 & 22     \\
 5217.39 & $-$1.07 &  3.21 &  96.6 &  72.0 &  13.8 &  28.8 &   9.5 &  24.2 &  \nodata &  20.9 &  57.8 &  30.1 &  56.8 &  37.9 & 20     \\
 5225.53 & $-$4.75 &  0.11 & 148.6 &  81.8 &  35.0 &  23.2 &  17.5 &  43.8 &  13.8 &  \nodata & 108.3 &  47.8 &  84.5 &  37.5 & 22     \\
 5232.94 & $-$0.10 &  2.94 & 176.1 & 131.2 &  77.1 &  92.4 &  65.8 &  93.3 &  61.8 &  78.0 & 132.6 &  96.9 & 119.4 & 100.1 & 20     \\
 5242.49 & $-$0.97 &  3.62 &  \nodata &  52.7 &  \nodata &  17.2 &  \nodata &  11.8 &  \nodata &  \nodata &  32.5 &  \nodata &  34.6 &  23.5 & 21     \\
 5247.05 & $-$4.91 &  0.09 & 142.2 &  77.8 &  26.2 &  18.9 &  14.9 &  37.3 &  \nodata &  11.3 & 101.8 &  41.0 &  77.7 &  31.7 & 22     \\
 5250.21 & $-$4.90 &  0.12 & 143.1 &  73.9 &  28.4 &  18.7 &  13.3 &  34.7 &   7.6 &  \nodata &  99.8 &  39.6 &  78.1 &  30.1 & 22     \\
 5253.46 & $-$1.57 &  3.28 &  59.7 &  42.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  26.5 &  10.6 &  24.5 &  15.7 & 20     \\
 5263.31 & $-$0.88 &  3.27 & 101.6 &  79.9 &  17.9 &  32.7 &  12.0 &  28.0 &  \nodata &  27.2 &  63.0 &  36.3 &  63.2 &  42.7 & 20     \\
 5266.56 & $-$0.38 &  2.99 & 159.2 & 122.1 &  59.9 &  76.0 &  44.5 &  69.1 &  45.1 &  65.4 & 118.8 &  79.9 & 107.9 &  80.9 & 21     \\
 5269.54 & $-$1.33 &  0.86 & 303.7 & 209.9 & 161.5 & 150.8 & 134.6 & 169.4 & 126.1 & 114.6 & 234.1 & 165.9 & 202.5 & 153.6 & 21     \\
 5281.79 & $-$0.83 &  3.03 & 120.2 &  92.3 &  29.7 &  44.9 &  22.8 &  43.9 &  26.8 &  36.5 &  83.6 &  53.0 &  80.6 &  58.0 & 21     \\
 5283.62 & $-$0.52 &  3.23 & 137.2 &  99.9 &  39.3 &  55.5 &  28.0 &  50.8 &  32.3 &  53.0 &  91.8 &  63.7 &  88.2 &  68.6 & 21     \\
 5288.53 & $-$1.51 &  3.68 &  25.8 &  20.7 &  \nodata &   3.6 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   8.1 &  \nodata & 21     \\
 5302.30 & $-$0.72 &  3.28 & 113.7 &  83.9 &  25.9 &  38.3 &  15.3 &  34.1 &  \nodata &  30.0 &  74.9 &  43.0 &  70.4 &  50.4 & 20     \\
 5307.37 & $-$2.95 &  1.61 & 120.4 &  77.6 &  24.1 &  29.3 &  12.7 &  32.8 &  \nodata &  \nodata &  84.5 &  39.9 &  72.1 &  38.8 & 22     \\
 5332.90 & $-$2.78 &  1.55 & 134.4 &  90.2 &  34.3 &  37.1 &  17.8 &  45.8 &  18.3 &  25.1 &  97.8 &  50.3 &  83.9 &  48.2 & 21     \\
 5339.93 & $-$0.65 &  3.27 & 116.7 &  88.9 &  27.1 &  48.2 &  18.3 &  \nodata &  20.2 &  36.8 &  80.0 &  49.1 &  76.0 &  57.1 & 20     \\
 5341.02 & $-$1.95 &  1.60 &  \nodata & 129.9 &  83.4 &  86.8 &  62.7 & 107.8 &  62.8 &  63.6 &  \nodata & 100.8 & 129.6 &  88.1 & 21     \\
 5365.40 & $-$1.02 &  3.56 &  58.8 &  44.5 &  \nodata &   7.0 &  \nodata &  \nodata &  \nodata &  \nodata &  24.4 &  10.6 &  27.2 &  15.1 & 21     \\
 5367.48 &  0.44 &  4.41 &  84.1 &  69.8 &  15.8 &  34.6 &  13.0 &  24.1 &  \nodata &  22.0 &  54.4 &  30.9 &  51.7 &  40.9 & 20     \\
 5369.96 &  0.54 &  4.35 &  95.2 &  76.5 &  19.2 &  32.8 &  13.2 &  26.6 &  19.2 &  26.9 &  58.2 &  37.3 &  58.2 &  45.8 & 21     \\
 5371.49 & $-$1.64 &  0.95 & 262.3 & 176.6 & 141.4 & 134.4 & 120.3 & 148.6 & 114.7 & 108.4 & 209.2 & 148.1 & 181.4 & 142.9 & 21     \\
 5383.37 &  0.64 &  4.31 & 105.7 &  84.5 &  23.8 &  45.8 &  19.4 &  34.0 &  21.5 &  36.0 &  68.0 &  45.4 &  68.0 &  54.0 & 21     \\
 5393.17 & $-$0.71 &  3.24 & 116.8 &  \nodata &  24.6 &  42.3 &  \nodata &  42.0 &  16.5 &  \nodata &  85.6 &  46.0 &  75.9 &  53.4 & 20     \\
 5397.13 & $-$1.95 &  0.92 & 239.4 & 157.5 & 135.1 & 126.4 & 108.3 & 141.8 & 102.6 & 100.4 & 193.1 & 137.2 & 166.3 & 114.8 & 22     \\
 5404.15 &  0.52 &  4.42 & 115.4 &  93.5 &  27.0 &  47.4 &  21.3 &  33.6 &  21.4 &  43.2 &  76.1 &  48.8 &  71.5 &  58.7 & 21     \\
 5405.78 & $-$1.80 &  0.99 & 240.0 & 159.8 & 132.4 & 127.3 & 111.0 & 140.5 & 102.7 & 100.9 & 190.8 & 138.9 & 166.8 & 117.3 & 22     \\
 5410.91 &  0.40 &  4.45 &  77.9 &  64.8 &  \nodata &  27.7 &   9.1 &  16.8 &   8.8 &  30.6 &  42.6 &  25.5 &  44.9 &  37.2 & 21     \\
 5415.20 &  0.64 &  4.37 &  98.9 &  78.9 &  19.6 &  43.4 &  16.6 &  32.3 &  14.8 &  36.0 &  64.3 &  38.7 &  64.0 &  52.3 & 21     \\
 5429.70 & $-$1.88 &  0.95 & 268.8 & 191.8 & 134.4 & 128.5 & 109.1 & 142.0 & 105.9 &  98.5 & 206.0 & 143.1 & 176.9 & 123.9 & 21     \\
 5434.53 & $-$2.08 &  1.01 & 223.7 & 144.3 & 125.2 & 110.5 &  98.1 & 125.6 &  89.3 &  88.1 & 180.4 & 129.1 & 154.5 & 106.3 & 22     \\
 5497.52 & $-$2.83 &  1.01 & 197.2 & 133.2 &  87.3 &  \nodata &  57.7 &  97.5 &  47.8 &  55.1 & 154.9 &  98.8 & 128.2 &  84.8 & 21     \\
 5501.46 & $-$3.05 &  0.95 & 180.8 & 114.0 &  77.2 &  72.4 &  49.2 &  86.3 &  44.6 &  50.1 & 140.5 &  88.9 & 120.9 &  76.0 & 21     \\
 5506.78 & $-$2.70 &  0.99 & 190.9 & 121.2 &  89.4 &  80.4 &  62.1 &  99.7 &  52.4 &  61.1 & 151.7 &  98.4 & 130.8 &  88.6 & 22     \\
 5567.39 & $-$2.56 &  2.61 &  52.3 &  31.3 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  21.3 &  11.1 &  19.0 &  \nodata & 20     \\
 5569.62 & $-$0.49 &  3.42 & 119.0 &  92.3 &  27.0 &  43.4 &  22.0 &  38.3 &  21.5 &  34.6 &  75.7 &  45.8 &  72.3 &  55.6 & 20     \\
 5572.84 & $-$0.28 &  3.40 & 135.8 & 104.0 &  37.9 &  54.0 &  24.8 &  53.6 &  27.7 &  46.3 &  97.2 &  59.2 &  87.3 &  65.4 & 20     \\
 5586.76 & $-$0.14 &  3.35 & 140.2 & 106.4 &  48.3 &  65.2 &  36.6 &  60.7 &  37.2 &  58.3 & 104.8 &  72.2 &  97.0 &  79.2 & 21     \\
 5658.82 & $-$0.84 &  3.38 & 128.6 &  91.5 &  \nodata &  33.1 &  \nodata &  29.5 &  12.7 &  26.9 &  68.7 &  \nodata &  64.4 &  45.2 & 21     \\
 5701.55 & $-$2.18 &  2.56 &  92.7 &  67.5 &  \nodata &  \nodata &  \nodata &  14.8 &  \nodata &  \nodata &  53.0 &  21.1 &  46.8 &  28.4 & 22     \\
 5753.12 & $-$0.69 &  4.24 &  43.5 &  31.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  13.6 &   5.9 &  16.3 &  11.6 & 21     \\
 5778.46 & $-$3.43 &  2.59 &  15.6 &   6.3 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   2.9 &  \nodata & 20     \\ 
 5916.25 & $-$2.95 &  2.45 &  55.6 &  26.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  23.7 &   5.6 &  18.3 &  14.6 & 22     \\
 6065.49 & $-$1.49 &  2.61 & 140.1 &  96.2 &  33.1 &  39.5 &  23.0 &  45.5 &  25.2 &  39.7 &  98.6 &  54.6 &  84.5 &  60.2 & 22     \\
 6136.61 & $-$1.41 &  2.44 & 162.7 & 107.5 &  52.0 &  62.3 &  36.1 &  65.5 &  36.2 &  52.1 & 115.6 &  73.3 & 106.1 &  75.2 & 21     \\
 6137.70 & $-$1.36 &  2.59 & 150.1 & 102.4 &  42.9 &  57.2 &  26.3 &  57.8 &  26.7 &  44.7 & 105.8 &  64.7 &  98.1 &  68.3 & 22     \\
 6151.62 & $-$3.26 &  2.18 &  57.6 &  28.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  24.2 &   7.0 &  19.5 &   7.2 & 22     \\
 6173.34 & $-$2.84 &  2.22 &  82.9 &  50.5 &  10.0 &  11.1 &  \nodata &  12.1 &  \nodata &  \nodata &  44.8 &  14.8 &  34.1 &  15.5 & 22     \\
 6180.21 & $-$2.59 &  2.73 &  47.0 &  27.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  19.7 &  \nodata &  14.9 &  \nodata & 20     \\
 6200.32 & $-$2.40 &  2.61 &  76.2 &  49.5 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  37.1 &  13.8 &  31.9 &  17.0 & 22     \\
 6219.29 & $-$2.39 &  2.20 & 117.2 &  75.3 &  19.3 &  25.9 &  10.1 &  24.2 &  \nodata &  14.7 &  79.9 &  35.7 &  65.1 &  35.1 & 22     \\
 6229.23 & $-$2.81 &  2.84 &  25.3 &  14.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   9.3 &  \nodata &   8.0 &  \nodata & 20     \\
 6232.64 & $-$1.22 &  3.65 &  56.5 &  41.2 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  22.8 &  \nodata &  22.1 &  15.4 & 20     \\
 6240.65 & $-$3.23 &  2.22 &  53.3 &  27.5 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  21.1 &  10.4 &  17.5 &   6.0 & 20     \\
 6246.32 & $-$0.73 &  3.60 &  89.7 &  67.9 &  11.6 &  22.0 &  \nodata &  18.0 &  \nodata &  22.6 &  48.3 &  27.0 &  48.7 &  32.6 & 20     \\
 6252.56 & $-$1.65 &  2.40 & 143.7 & 100.2 &  41.6 &  51.8 &  27.8 &  53.3 &  22.4 &  44.2 & 107.8 &  63.7 &  94.5 &  62.8 & 22     \\
 6265.14 & $-$2.51 &  2.18 & 110.0 &  72.5 &  19.5 &  25.2 &  \nodata &  24.1 &  13.2 &  \nodata &  72.5 &  32.2 &  62.3 &  34.2 & 22     \\
 6297.80 & $-$2.70 &  2.22 &  92.3 &  76.0 &  16.1 &  \nodata &  \nodata &  14.6 &  \nodata &  \nodata &  53.3 &  \nodata &  70.1 &  19.2 & 22     \\
 6301.50 & $-$0.72 &  3.65 &  95.4 &  71.9 &  14.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  71.7 &  \nodata &  \nodata &  31.7 & 20     \\
 6322.69 & $-$2.39 &  2.59 &  93.4 &  50.6 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  41.0 &  17.6 &  39.4 &  23.4 & 22     \\
 6336.83 & $-$0.86 &  3.69 &  77.3 &  62.1 &  \nodata &  17.2 &  \nodata &  12.1 &  \nodata &  \nodata &  38.9 &  21.6 &  38.7 &  \nodata & 20     \\
 6344.15 & $-$2.88 &  2.43 &  67.1 &  39.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  27.6 &   8.2 &  23.2 &  \nodata & 22     \\
 6355.03 & $-$2.36 &  2.84 &  63.4 &  39.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  25.2 &   9.2 &  24.1 &  12.6 & 20     \\
 6358.69 & $-$4.43 &  0.86 & 118.0 &  64.6 &  11.8 &  \nodata &  \nodata &  19.3 &  \nodata &  \nodata &  71.9 &  24.2 &  51.9 &  18.5 & 22     \\
 6393.60 & $-$1.43 &  2.43 & 149.6 & 105.6 &  46.7 &  54.5 &  31.4 &  60.2 &  30.5 &  46.0 & 115.8 &  70.5 & 100.8 &  67.4 & 20     \\
 6408.02 & $-$1.02 &  3.68 &  68.2 &  49.4 &  \nodata &  15.4 &  \nodata &   7.2 &  \nodata &  \nodata &  29.9 &  15.6 &  31.7 &  \nodata & 20     \\
 6411.65 & $-$0.60 &  3.65 &  96.5 &  72.0 &  14.4 &  26.8 &  12.9 &  18.2 &  \nodata &  18.5 &  57.0 &  31.1 &  56.7 &  40.6 & 20     \\
 6421.36 & $-$1.99 &  2.28 & 140.6 &  93.5 &  34.9 &  39.8 &  22.7 &  45.5 &  25.8 &  34.8 &  99.3 &  55.7 &  86.8 &  54.4 & 22     \\
 6430.85 & $-$1.97 &  2.18 & 146.8 & 100.2 &  45.0 &  47.2 &  27.5 &  56.7 &  24.9 &  39.1 & 112.2 &  63.7 &  97.9 &  65.8 & 22     \\
 6481.88 & $-$2.94 &  2.28 &  73.3 &  62.8 &  \nodata &  14.8 &  \nodata &  \nodata &  \nodata &  \nodata &  37.1 &  12.5 &  35.2 &  12.0 & 22     \\
 6494.99 & $-$1.23 &  2.40 & 198.4 & 140.4 &  71.4 &  77.8 &  49.6 &  80.5 &  43.7 &  \nodata & 132.9 & \nodata & 117.1 &  88.2 & 22     \\
 6498.95 & $-$4.66 &  0.96 &  84.3 &  38.3 &   5.7 &  \nodata &  \nodata &  10.1 &  \nodata &  \nodata &  42.8 &  12.9 &  32.2 &  \nodata & 22     \\
 6581.21 & $-$4.68 &  1.48 &  29.0 &   9.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   8.4 &  \nodata &   6.0 &  \nodata & 20     \\
 6593.88 & $-$2.38 &  2.43 & 100.1 &  63.2 &  13.1 &  \nodata &  \nodata &  15.0 &  \nodata &  \nodata &  64.3 &  25.9 &  51.0 &  28.2 & 22     \\
 6609.12 & $-$2.65 &  2.56 &  66.9 &  36.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  31.5 &   8.8 &  27.3 &  12.8 & 22     \\
 6663.45 & $-$2.44 &  2.42 & 100.8 &  64.3 &  11.5 &  16.3 &  \nodata &  16.5 &  \nodata &  \nodata &  59.6 &  24.1 &  48.0 &  25.4 & 22     \\
 6677.99 & $-$1.42 &  2.68 & 141.8 & 102.1 &  38.7 &  46.7 &  27.4 &  50.3 &  24.0 &  39.0 & 102.2 &  61.5 &  92.1 &  64.8 & 21     \\
 6750.15 & $-$2.58 &  2.42 &  88.2 &  55.8 &   8.5 &  16.2 &  \nodata &  10.9 &  \nodata &  \nodata &  48.8 &  18.0 &  40.3 &  20.6 & 22     \\
 6945.20 & $-$2.43 &  2.42 &  99.3 &  63.8 &  11.9 &  \nodata &  \nodata &  16.9 &  \nodata &  \nodata &  57.5 &  22.8 & \nodata &  \nodata & 20     \\
 6978.86 & $-$2.46 &  2.48 &  95.1 &  55.8 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  53.7 &  21.8 &  45.1 &  24.4 & 22     \\
 7112.17 & $-$2.99 &  2.99 &  13.4 &  10.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  10.3 &  \nodata & 20     \\
\multicolumn{16}{c}{{FeII}} \\
 3295.81 & $-$2.90 & 1.08 & \nodata & \nodata & \nodata & 90.7 & \nodata &
\nodata & \nodata & \nodata & \nodata & 75.4 & \nodata & \nodata & 23 \\ 
 3824.93 & $-$3.35 &  2.58 &  \nodata &  \nodata &  \nodata &  23.0 &   8.0 &  17.3 &  \nodata &   9.2 &  \nodata &  22.6 &  \nodata &  \nodata & 24     \\
 3974.17 & $-$3.45 &  2.70 &  \nodata &  \nodata &  \nodata &  10.6 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 24     \\
 4075.95 & $-$3.32 & 2.54 & \nodata & \nodata & \nodata & \nodata & \nodata
& \nodata & \nodata & 4.9 & \nodata & \nodata & \nodata & \nodata & 24 \\
 4128.75 & $-$3.71 &  2.58 &  \nodata &  35.5 &  \nodata &  18.5 &  \nodata &   8.5 &  \nodata &   5.4 &  \nodata &  12.9 &  23.5 &  \nodata & 24     \\
 4178.86 & $-$2.51 &  2.58 &  \nodata &  76.8 &  41.8 &  69.1 &  33.5 &  52.3 &  32.1 &  38.1 &  71.0 &  \nodata &  75.9 &  57.8 & 24,25  \\
 4416.82 & $-$2.54 &  2.78 & \nodata &  74.6 &  32.2 &  54.3 &  23.5 &  37.6 &  20.6 &  26.0 &  63.6 &  47.8 &  73.7 &  46.0 & 24     \\
 4489.18 & $-$2.91 &  2.83 &  \nodata &  74.2 &  16.2 &  39.8 &  11.9 &  22.9 &  11.1 &  15.3 &  52.9 &  31.1 &  51.0 &  33.4 & 24     \\
 4491.40 & $-$2.71 &  2.86 &  71.7 &  60.6 &  21.0 &  44.5 &  14.6 &  30.0 &  13.5 &  18.5 &  49.0 &  36.2 &  51.7 &  33.8 & 24,25  \\
 4508.29 & $-$2.33 &  2.86 &  99.0 &  78.0 &  42.4 &  70.0 &  29.7 &  51.5 &  27.8 &  33.7 &  66.9 &  54.4 &  72.5 &  55.1 & 24     \\
 4515.34 & $-$2.48 &  2.84 &  \nodata &  74.7 &  30.7 &  65.2 &  23.7 &  44.6 &  21.6 &  28.2 &  71.4 &  47.5 &  67.5 &  47.7 & 26     \\
 4520.23 & $-$2.60 &  2.81 &  92.8 &  72.7 &  30.4 &  59.2 &  22.5 &  40.0 &  21.5 &  27.9 &  69.8 &  46.5 &  68.5 &  48.5 & 26     \\
 4541.52 & $-$2.99 &  2.86 &  57.6 &  51.8 &  15.2 &  32.1 &  10.0 &  21.5 &   9.3 &  13.3 &  41.8 &  24.9 &  43.7 &  29.8 & 24     \\
 4555.89 & $-$2.39 &  2.83 &  \nodata &  84.6 &  39.1 &  66.3 &  29.9 &  49.1 &  28.9 &  34.9 &  78.0 &  54.4 &  80.1 &  55.8 & 24     \\
 4576.33 & $-$2.94 &  2.84 &  66.4 &  53.2 &  16.4 &  34.0 &  10.7 &  21.9 &   9.7 &  13.8 &  38.2 &  26.5 &  43.4 &  27.6 & 27     \\
 4582.84 & $-$3.10 &  2.84 &  55.3 &  41.8 &   9.7 &  22.6 &   5.9 &  15.0 &   5.6 &   8.4 &  32.2 &  16.9 &  34.0 &  20.5 & 24,25  \\
 4583.84 & $-$1.92 &  2.81 & \nodata & 104.6 &  73.0 &  92.4 &  56.7 &  81.7 &  56.0 &  57.1 & 102.8 &  78.2 & 104.4 &  76.2 & 24     \\
 4620.51 & $-$3.21 &  2.83 &  40.1 &  36.8 &   7.7 &  20.5 &   5.2 &  11.7 &   5.4 &   7.2 &  25.0 &  13.4 &  28.3 &  \nodata & 27     \\
 4629.34 & $-$2.37 &  2.81 &  98.3 &  83.7 &  43.3 &  69.7 &  32.2 &  52.3 &  27.8 &  34.8 &  76.9 &  56.5 &  73.4 &  56.2 & 26     \\
 5018.45 & $-$1.22 &  2.89 & \nodata & 142.4 & 106.3 & 134.8 &  88.6 & 118.7 &  85.6 &  85.6 & 147.6 & 114.1 & 139.7 & 107.3 & 26     \\
 5197.56 & $-$2.10 &  3.23 &  90.8 &  67.2 &  27.2 &  \nodata &  21.7 &  33.8 &  20.3 &  \nodata &  58.7 &  44.1 &  62.8 &  44.6 & 25     \\
 5234.62 & $-$2.23 &  3.22 &  88.6 &  67.1 &  36.0 &  56.6 &  24.6 &  44.4 &  17.3 &  29.1 &  61.7 &  46.3 &  65.4 &  47.0 & 27     \\
 5264.79 & $-$3.25 &  3.23 &  33.5 &  27.2 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  15.6 &  10.5 &  20.5 &  13.0 & 27     \\
 5276.00 & $-$1.94 &  3.20 & 118.9 &  93.2 &  38.5 &  67.6 &  29.9 &  47.7 &  25.3 &  29.3 &  74.4 &  55.0 &  81.3 &  58.9 & 25     \\
 5325.56 & $-$3.26 &  3.22 &  30.7 &  22.3 &  \nodata &  11.3 &  \nodata &   5.8 &  \nodata &  \nodata &  15.1 &  10.1 &  18.2 &   9.7 & 24     \\
 5414.08 & $-$3.50 &  3.22 &  16.0 &  10.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   7.9 &   3.3 &   7.5 &  \nodata & 27     \\
 6369.42 & $-$4.30 &  2.89 &  \nodata &  10.6 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   6.3 &  \nodata & 24     \\
 6432.67 & $-$3.50 &  2.89 &  \nodata &  23.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  20.8 &   8.9 &  18.3 &  10.0 & 27     \\
 6516.07 & $-$3.38 &  2.89 &  61.4 &  \nodata &  \nodata &  22.8 &  \nodata &  \nodata &  \nodata &  \nodata &  58.1 &  \nodata &  29.5 &  32.8 & 27     \\
\multicolumn{16}{c}{{CoI}} \\
 3845.47 &  0.01 &  0.92 &  \nodata &  \nodata &  76.1 &  82.8 &  64.8 &  87.4 &  62.5 &  68.1 &  \nodata &  87.8 &  \nodata &  \nodata & 28     \\
 3861.16 & $-$0.89 &  1.05 &  \nodata &  \nodata &  34.1 &  36.5 &  \nodata &  41.7 &  19.3 &  21.9 &  \nodata &  \nodata &  \nodata &  \nodata & 28     \\
 3922.76 & $-$2.10 &  1.05 &  \nodata &  \nodata &  \nodata & 155.2 & 133.5 &  \nodata &  \nodata & 126.0 & 245.6 &  \nodata &  \nodata &  \nodata & 28     \\
 3941.73 & $-$2.03 &  0.43 &  \nodata &  \nodata &  25.3 &  20.5 &  16.9 &  36.1 &  12.9 &  14.7 &  \nodata &  \nodata &  \nodata &  \nodata & 28     \\
 3957.93\tablenotemark{a} & $-$2.06 &  0.58 &  \nodata &  48.6 &  17.6 &  \nodata &  14.7 &  \nodata &  12.2 &   9.7 &  \nodata &  \nodata &  63.2 &  \nodata & 28     \\
 4020.90 & $-$2.07 &  0.43 & 124.6 &  79.2 &  28.9 &  27.0 &  20.6 &  38.6 &  16.5 &  16.2 &  83.3 &  41.9 &  73.4 &  \nodata & 28     \\
 4092.39 & $-$0.94 &  0.92 &  \nodata & 124.6 &  37.8 &  48.6 &  27.6 &  57.8 &  27.6 &  32.5 &  \nodata &  61.7 & 100.9 &  \nodata & 28     \\
 4110.53 & $-$1.08 &  1.05 & 143.0 &  95.9 &  23.3 &  31.0 &  19.7 &  37.3 &  14.0 &  17.3 &  94.0 &  44.6 &  81.7 &  34.5 & 28     \\
 4121.32 & $-$0.32 &  0.92 & 142.5 & 116.0 &  77.1 &  82.8 &  64.5 &  88.5 &  62.9 &  64.5 & 122.4 &  86.8 & 113.1 &  85.6 & 28     \\
\multicolumn{16}{c}{{NiI}} \\
 3500.85 & $-$1.29 & 0.17 & \nodata & \nodata & 103.4 & 102.0 & 80.8 & 
\nodata & 81.7 & 80.0 & \nodata & 102.9 & \nodata & \nodata & 29 \\
 3515.05 & $-$0.27 & 0.11 & \nodata & \nodata & 150.2 & 144.7 & 120.5 & 
163.4 & 116.8 & \nodata & \nodata & 150.3 & \nodata & \nodata & 29 \\
 3516.21 & 0.06 & 3.54 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 30 \\
 3519.77 &  $-$1.42 & 0.28 & \nodata & \nodata & 97.3 & 96.7 & 78.8 & 
103.7 & 76.1 & \nodata & \nodata & 101.5 & \nodata & \nodata & 29 \\
 3524.54 & $-$0.01 & 0.03 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3566.37 &  $-$0.25 & 0.42 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3571.87 & $-$1.15 & 0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & 
125.1 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3597.71 & $-$1.12 & 0.21 & \nodata & \nodata & 116.1 & 113.8 & 92.0 & 
\nodata & 85.7 & 85.5 & \nodata & 108.7 & \nodata & \nodata & 29 \\
 3602.28 & $-$2.19 & 0.17  & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3612.74 & $-$1.42 & 0.28 & \nodata & \nodata & 97.4 & 98.5 & 77.3 & 
102.4 & 76.1 & \nodata & \nodata & 96.8 & \nodata & \nodata & 29 \\
 3619.39 & 0.02 & 0.42 & \nodata & \nodata & 128.0 & 136.8 & 111.1 & 
\nodata & 108.2 & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3624.73 & $-$2.45 &  0.00 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3664.10 & $-$2.13 & 0.28  & \nodata & \nodata & \nodata & 82.0 & 60.2 & 
\nodata & 56.8 & \nodata & \nodata & 85.3 & \nodata & \nodata & 29 \\
 3669.24 & $-$2.69 & 0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3670.43 & $-$2.40 & 0.17 & \nodata & \nodata & 76.5 & 73.8 & 54.1 & 
85.9 & 54.4 & 56.8 & \nodata & 79.6 & \nodata & \nodata & 29 \\
 3749.05 & $-$3.35 & 0.00 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3775.57 & $-$1.41&  0.42 &  \nodata &  \nodata & 106.5 & 103.5 &  80.6 &  \nodata &  83.5 &  76.7 &  \nodata & 103.7 &  \nodata &  \nodata & 29     \\
 3807.14 & $-$1.22 &  0.42 &  \nodata &  \nodata & 105.4 & 107.6 &  85.8 &  \nodata &  83.6 &  83.6 &  \nodata &  \nodata &  \nodata &  \nodata & 29     \\
 3831.69 & $-$2.27 &  0.42 &  \nodata &  \nodata &  71.8 &  82.2 &  50.9 &  84.6 &  51.0 &  59.2 &  \nodata &  \nodata &  \nodata &  \nodata & 29     \\
 3858.30 & $-$0.95 &  0.42 &  \nodata &  \nodata & 124.3 & 123.8 &  95.8 & 120.2 &  93.7 &  91.7 &  \nodata & 117.6 &  \nodata &  \nodata & 29     \\
 4331.65 & $-$2.10 &  1.68 &  76.9 &  52.2 &  10.6 &  14.5 &   4.1 &  15.8 &  \nodata &  10.1 &  43.8 &  18.4 &  42.4 &  18.1 & 28     \\
 4462.46 & $-$0.55 &  3.46 &  51.3 &  41.4 &  \nodata &  10.4 &  \nodata &  \nodata &  \nodata &  \nodata &  18.9 &   9.8 &  \nodata &  \nodata & 30     \\
 4470.48 & $-$0.31 &  3.40 &  44.0 &  41.0 &   4.2 &  13.7 &   3.5 &  10.1 &   2.8 &  10.2 &  23.0 &  11.2 &  24.1 &  \nodata & 30     \\
 4604.99 & $-$0.25 &  3.48 &  39.3 &  39.5 &   5.1 &  14.3 &   3.3 &  10.0 &   5.0 &   9.5 &  21.2 &  10.9 &  26.4 &  \nodata & 30     \\
 4648.65 & $-$0.10 &  3.42 &  52.6 &  47.9 &   9.2 &  18.3 &   5.6 &  15.6 &   6.1 &  13.4 &  28.2 &  16.7 &  32.6 &  21.0 & 30     \\
 4686.21 & $-$0.58 &  3.60 &  24.1 &  21.1 &  \nodata &   5.9 &  \nodata &   3.5 &  \nodata &   3.7 &   9.4 &   4.1 &   8.5 &  \nodata & 30     \\
 4715.76 & $-$0.32 &  3.54 &  \nodata &  39.6 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 30     \\
 4756.51 & $-$0.27 &  3.48 &  46.3 &  37.9 &  \nodata &  \nodata &  \nodata &   9.4 &  \nodata &  \nodata &  19.3 &  11.7 &  23.1 &  14.5 & 30     \\
 4866.27 & $-$0.21 &  3.54 &  42.0 &  38.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  18.5 &  10.6 &  24.1 &  11.9 & 30     \\
 4873.44 & $-$0.38 &  3.70 &  27.2 &  24.2 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  14.4 &  \nodata & 30     \\
 4925.56 & $-$0.77 &  3.65 &  \nodata &  16.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 30     \\
 4953.21 & $-$0.58 &  3.74 &  28.8 &  19.8 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  10.3 &  \nodata & 30     \\
 4976.35 & $-$3.10 &  1.68 &  42.8 &  20.2 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  15.0 &  \nodata &  14.5 &  \nodata & 28     \\
 4998.22 & $-$0.69 &  3.61 &  \nodata &  14.2 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   8.0 &  \nodata &  \nodata &  \nodata & 30     \\
 5003.75 & $-$2.80 &  1.68 &  35.5 &  15.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  11.8 &  \nodata &   8.8 &  \nodata & 28     \\
 5017.58 & $-$0.02 &  3.54 &  56.3 &  46.5 &  \nodata &  15.0 &  \nodata &  13.5 &  \nodata &  10.5 &  26.0 &  15.3 &  32.4 &  18.1 & 30     \\
 5035.36 &  0.29 &  3.63 &  65.6 &  56.3 &  12.0 &  26.0 &   9.3 &  24.6 &  \nodata &  14.5 &  38.5 &  22.8 &  43.9 &  29.1 & 30     \\
 5080.53 &  0.33 &  3.65 &  72.0 &  64.6 &  13.0 &  23.0 &  \nodata &  23.9 &  \nodata &  \nodata &  39.7 &  22.3 &  42.7 &  28.2 & 30     \\
 5099.32 & $-$0.44 &  3.65 &  \nodata &  27.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 30     \\
 5102.97 & $-$2.62 &  1.68 &  55.5 &  27.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  19.3 &  \nodata & 28     \\
 5137.08 & $-$1.99 &  1.68 & 117.8 &  81.5 &  19.8 &  27.9 &   9.6 &  36.4 &  \nodata &  17.4 &  77.5 &  37.6 &  70.8 &  34.7 & 28     \\
 5424.65 & $-$2.77 &  1.95 &  32.4 &  17.9 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  12.9 &  \nodata &  11.1 &  \nodata & 28     \\
 5435.87 & $-$2.59 &  1.99 &  42.3 &  22.9 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  17.0 &  \nodata &  15.6 &  \nodata & 28     \\
 5476.91 & $-$0.89 &  1.83 & 173.8 & 118.9 &  64.0 &  77.2 &  49.2 &  84.4 &  46.5 &  63.0 & 129.5 &  86.4 & 117.6 &  80.7 & 28     \\
 5578.72 & $-$2.64 &  1.68 &  59.8 &  32.3 &  \nodata &  \nodata &  \nodata &   9.4 &  \nodata &  \nodata &  27.8 &   5.8 &  24.4 &  \nodata & 28     \\
 5587.87 & $-$2.14 &  1.94 &  60.4 &  31.5 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  28.3 &   9.2 &  23.3 &   9.1 & 28     \\
 5592.28 & $-$2.57 &  1.95 &  59.3 &  33.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  26.0 &  10.8 &  23.5 &   9.7 & 28     \\
 5711.91 & $-$2.27 &  1.94 &  73.9 &  47.5 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  33.1 &  \nodata &  29.3 &  10.5 & 28     \\
 5754.68 & $-$2.33 &  1.94 &  81.4 &  50.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  39.8 &  13.5 &  35.3 &  14.9 & 28     \\
 5847.00 & $-$3.21 &  1.68 &  21.6 &   9.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   8.9 &  \nodata &   7.2 &  \nodata & 28     \\
 5892.88 & $-$2.35 &  1.99 &  82.5 &  48.4 &  15.9 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  37.4 &  \nodata &  35.9 &  \nodata & 28     \\
 6108.12 & $-$2.45 &  1.68 &  72.6 &  44.3 &  \nodata &  \nodata &  \nodata &  11.4 &  \nodata &  \nodata &  39.3 &  11.4 &  33.5 &  12.0 & 28     \\
 6128.99 & $-$3.33 &  1.68 &  24.5 &  10.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  10.9 &  \nodata &  \nodata &  \nodata & 28     \\
 6176.81 & $-$0.26 &  4.09 &  19.4 &  16.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  11.8 &  \nodata & 30     \\
 6314.66 & $-$1.77 &  1.94 &  \nodata &  44.2 &  11.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  45.0 &  10.6 &  27.3 &  \nodata & 28     \\
 6327.60 & $-$3.15 &  1.68 &  41.0 &  19.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  16.6 &  \nodata &  13.3 &  12.3 & 28     \\
 6482.80 & $-$2.63 &  1.94 &  \nodata &  19.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  29.4 &  \nodata &  27.3 &  \nodata & 28     \\
 6643.64 & $-$2.30 &  1.68 & 111.4 &  73.5 &  14.6 &  20.8 &  \nodata &  \nodata &   7.0 &  \nodata &  70.8 &  29.5 &  \nodata &  25.3 & 28     \\
 6767.77 & $-$2.17 &  1.83 &  97.8 &  61.1 &  11.1 &  17.3 &  \nodata &  25.5 &  \nodata &  \nodata &  60.9 &  26.4 &  54.8 &  23.0 & 28     \\
 7062.97 & $-$3.50 &  1.95 &  10.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  11.2 &  \nodata &  \nodata &  \nodata & 28     \\
\multicolumn{16}{c}{{ZnI}} \\
 4722.20 & $-$0.39 &  4.03 &  \nodata &  40.6 &   9.1 &  25.7 &   5.9 &  14.5 &  \nodata &  \nodata &  24.1 &  \nodata &  31.8 &  22.8 & 31     \\
 4810.55 & $-$0.17 &  4.08 &  52.5 &  50.1 &  15.0 &  32.4 &  11.1 &  15.5 &  \nodata &  \nodata &  28.9 &  23.7 &  40.6 &  30.5 & 31     \\
\multicolumn{16}{c}{{YII}} \\
 3549.01 & $-$0.28 & 0.13 & \nodata & \nodata & 44.6 & 47.6 & 35.3 &
42.8 & 28.4 & 15.1 & \nodata & 54.9 & \nodata & \nodata & 32 \\
 3600.74 & 0.28 & 0.18 & \nodata & \nodata & 67.8 & 70.8 & 56.3 &
67.7 & 47.3 & 31.5 & \nodata & 72.3 & \nodata & \nodata & 32 \\
 3611.04 & 0.01 & 0.13 & \nodata & \nodata & 53.3 & 59.6 & 44.7 &
55.2 & 36.7 & \nodata & \nodata & 64.4 & \nodata & \nodata & 32 \\
 3628.70 & $-$0.71 & 0.13 & \nodata & \nodata & 33.9 & 35.7 & 23.5 &
30.2 & 17.7 & \nodata & \nodata & 44.4 & \nodata & \nodata & 32 \\
 3710.29 & 0.46 & 0.18 & \nodata & \nodata & 77.1 & \nodata & 63.1 &
73.7 & 56.3 & \nodata & \nodata & 83.8 & \nodata & \nodata & 32 \\
 3747.55 & $-$0.91 & 0.10 & \nodata & \nodata & 23.6 & 27.9 & \nodata &
22.2 & 12.0 & \nodata & \nodata & 37.3 & \nodata & \nodata & 32 \\
 3774.34 &  0.21 &  0.13 & \nodata &  \nodata &  73.0 &  78.8 &  60.4 &  73.0 &  54.2 &  34.1 & \nodata &  79.6 &  \nodata &  \nodata & 32     \\
 3788.70 & $-$0.07 &  0.10 &  \nodata &  \nodata &  62.4 &  73.6 &  53.5 &  61.8 &  44.7 &  29.7 &  \nodata &  78.4 &  \nodata &  \nodata & 32     \\
 3950.36 & $-$0.49 &  0.10 & 110.4 &  75.1 &  47.4 &  52.0 &  37.4 &  47.2 &  28.6 &  14.0 &  78.4 &  62.3 &  92.2 &  \nodata & 32     \\
 4398.01 & $-$1.00 &  0.13 & 100.3 &  \nodata &  28.4 &  29.0 &  19.6 &  28.3 &  12.9 &   7.4 &  68.9 &  45.3 &  70.8 &  25.6 & 32     \\
 4854.87 & $-$0.38 &  0.99 &  73.2 &  44.5 &  \nodata &  12.2 &  \nodata &  \nodata &  \nodata &  \nodata &  40.3 &  25.8 &  40.6 &  \nodata & 32     \\
 4883.69 &  0.07 &  1.08 &  89.4 &  62.9 &  20.4 &  29.6 &  15.4 &  \nodata &  14.8 &  \nodata &  57.2 &  39.5 &  59.3 &  21.8 & 32     \\
 4900.11 & $-$0.09 &  1.03 &  92.2 &  56.8 &  21.1 &  \nodata &  \nodata &  19.2 &  \nodata &  \nodata &  57.0 &  40.0 &  52.6 &  18.4 & 32     \\
 5087.42 & $-$0.17 &  1.08 &  76.2 &  45.4 &  12.3 &  16.9 &  \nodata &  \nodata &  \nodata &  \nodata &  38.2 &  27.4 &  43.2 &  13.4 & 32     \\
\multicolumn{16}{c}{{ZrII}} \\
 3479.03 & $-$0.69 & 0.53 & \nodata & \nodata & 16.8 & 18.9 & 12.7 &
13.9 & \nodata & \nodata & \nodata & 28.5 & \nodata & \nodata & 33 \\
 3479.39 & 0.17 & 0.71 & \nodata & \nodata & 38.1 & 47.9 & 31.3 &
34.1 & 25.9 & 14.6 & \nodata & 50.7 & \nodata & \nodata & 33 \\
 3499.57 & $-$0.81 & 0.41 & \nodata & \nodata & 12.1 & 15.4 & 7.4 &
10.5 & \nodata & \nodata & \nodata & 23.3 & \nodata & \nodata & 33 \\
 3505.67 & $-$0.36 & 0.16 & \nodata & \nodata & 47.0 & 50.2 & 37.4 &
44.0 & 32.0 & 18.8 & \nodata & 56.3 & \nodata & \nodata & 33 \\
 3551.96 & $-$0.31 & 0.09 & \nodata & \nodata & 54.5 & 61.3 & 43.6 &
53.5 & 38.1 & 23.4 & \nodata & 65.6 & \nodata & \nodata & 33 \\
 3588.33 & $-$1.13 & 0.41 & \nodata & \nodata & 9.8 & 13.1 & \nodata &
\nodata & \nodata & \nodata & \nodata & 22.5 & \nodata & \nodata & 33 \\
 3607.38 & $-$0.64 & 1.24 & \nodata & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & 8.6 & \nodata & \nodata & 33 \\
 3714.79 & $-$0.93 & 0.53 & \nodata & \nodata & 15.0 & 18.7 & 10.5 &
12.9 & 8.3 & \nodata & \nodata & 30.2 & \nodata & \nodata & 33 \\
 3836.77 & $-$0.06 &  0.56 &  \nodata &  \nodata &  46.9 &  \nodata &  33.6 &  42.2 &  27.3 &  13.1 &  \nodata &  \nodata &  \nodata &  \nodata & 33     \\
 4050.33 & $-$1.00 &  0.71 &  \nodata &  38.1 &  12.2 &  12.7 &   5.1 &   9.1 &  \nodata &  \nodata &  36.1 &  19.6 &  35.3 &  \nodata & 33     \\
 4208.98 & $-$0.46 &  0.71 &  99.1 &  63.3 &  29.8 &  30.9 &  18.6 &  25.1 &  13.8 &   6.1 &  63.1 &  41.9 &  64.4 &  \nodata & 33     \\
 4317.32 & $-$1.38 &  0.71 &  52.4 &  25.3 &   7.9 &   6.3 &  \nodata &   4.3 &  \nodata &  \nodata &  24.6 &  12.7 &  21.7 &  \nodata & 33     \\
 5112.28 & $-$0.59 &  1.66 &  23.0 &   8.8 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   7.0 &  \nodata &   7.2 &  \nodata & 33     \\
\multicolumn{16}{c}{{BaII}} \\
 4554.03 &  0.12 &  0.00 & 266.3 & 173.8 &  90.9 & 152.6 & 135.4 &  96.7 & 116.8 &  83.6 & 195.7 & 154.6 & 181.3 & 115.7 & 34     \\
 5853.69 & $-$1.02 &  0.60 & 129.4 &  72.4 &   8.4 &  39.8 &  29.0 &   8.5 &  19.1 &  \nodata &  81.4 &  51.0 &  72.6 &  20.3 & 34     \\
 6141.73 & $-$0.07 &  0.70 & 199.6 & 119.2 &  36.1 &  93.3 &  76.4 &  43.2 &  50.3 &  33.9 & 140.5 &  94.2 & 117.6 &  61.3 & 34    \\
 6496.91 & $-$0.37 &  0.60 & 202.3 & 116.9 &  29.3 &  93.4 &  71.8 &  32.0 &  50.6 &  23.4 & 138.2 & 108.2 & 118.4 &  71.8 & 34     \\
\multicolumn{16}{c}{{LaII}} \\
 3995.75 & $-$0.02 &  0.17 &  syn & syn &  \nodata &  syn &  syn &  \nodata &  \nodata &  syn & syn & syn & syn &  \nodata & 35     \\
 4086.71 & $-$0.16 &  0.00 &  syn &  syn &  \nodata &  syn & syn &  syn & syn 
&  syn & syn &  syn & syn &  \nodata & 35     \\
 4123.23 &  0.12 &  0.32 & syn & syn &  \nodata & syn &  syn &  \nodata &  
syn &  syn &  syn &  syn &  syn & syn & 35     \\
 4333.76 & $-$0.16 &  0.17 &  syn &  syn &  \nodata &  syn &  syn &  \nodata 
&  syn & syn & syn & syn & syn & syn & 35     \\
\multicolumn{16}{c}{{CeII}} \\
 4083.23 &  0.24 &  0.70 &  \nodata &  16.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  12.6 &  \nodata & 35     \\
 4120.84 & $-$0.24 &  0.32 &  \nodata &  16.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   5.3 &  \nodata &  \nodata & 35     \\
 4222.60 & $-$0.18 &  0.12 &  \nodata &  20.9 &  \nodata &   7.6 &   6.7 &  \nodata &  \nodata &  \nodata &  27.0 &  11.7 &  21.8 &  \nodata & 35     \\
 4562.37 &  0.33 &  0.48 &  65.9 &  25.6 &  \nodata &   8.5 &   5.9 &  \nodata &  \nodata &  \nodata &  29.0 &  11.9 &  24.1 &  \nodata & 35     \\
 4628.16 &  0.26 &  0.52 &  58.4 &  25.0 &  \nodata &   5.9 &   5.0 &  \nodata &  \nodata &  \nodata &  22.5 &   9.5 &  24.4 &  \nodata & 35     \\
\multicolumn{16}{c}{{PrII}} \\
 3964.81 &  0.09 &  0.05 &  \nodata &  \nodata &  syn &  syn &  syn &  syn &  
syn &  syn &  \nodata &  \nodata &  \nodata &  \nodata & 35     \\
 3965.26 & $-$0.13 &  0.20 &  \nodata &  \nodata &  \nodata &  \nodata &  syn &  \nodata &  \nodata &  \nodata &  \nodata &  syn &  \nodata &  \nodata & 35     \\
\multicolumn{16}{c}{{NdII}} \\
 3973.27 &  0.43 &  0.63 &  \nodata &  \nodata &  \nodata &  \nodata &   5.4 &  \nodata &  \nodata &  \nodata &  \nodata &  10.2 &  \nodata &  \nodata & 35     \\
 4021.34 & $-$0.17 &  0.32 &  53.8 &  18.0 &  \nodata &   8.9 &   6.8 &  \nodata &  \nodata &  \nodata &  22.8 &  11.3 &  19.7 &  \nodata & 35     \\
 4061.09 &  0.30 &  0.47 &  89.0 &  50.3 &  \nodata &  26.0 &  18.6 &   4.5 &   7.3 &   5.7 &  52.0 &  31.2 &  54.2 &  21.2 & 35     \\
 4069.27 & $-$0.40 &  0.06 &  \nodata &  \nodata &  \nodata &   8.9 &   5.9 &  \nodata &  \nodata &  \nodata &  \nodata &  10.5 &  26.6 &  \nodata & 35     \\
 4109.46 &  0.18 &  0.32 &  \nodata &  65.1 &   5.0 &  25.7 &  21.4 &  \nodata &  10.2 &  \nodata &  \nodata &  36.9 &  69.5 &  \nodata & 35     \\
 4232.38 & $-$0.35 &  0.06 &  \nodata &  25.4 &  \nodata &   9.3 &   7.4 &  \nodata &  \nodata &  \nodata &  39.3 &  13.8 &  28.2 &  \nodata & 35     \\
 4446.39 & $-$0.63 &  0.20 &  60.1 &  24.5 &  \nodata &   8.6 &   7.2 &  \nodata &  \nodata &  \nodata &  31.3 &  11.6 &  27.8 &  \nodata & 35     \\
 4462.99 & $-$0.07 &  0.56 &  72.3 &  39.0 &  \nodata &   9.0 &   5.9 &  \nodata &  \nodata &  \nodata &  28.3 &  12.7 &  30.7 &  \nodata & 35     \\
 5130.59 &  0.10 &  1.30 &  26.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   8.8 &  \nodata &   9.4 &  \nodata & 35     \\
 5212.35 & $-$0.70 &  0.20 &  34.4 &   9.0 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  11.3 &  \nodata &  11.7 &  \nodata & 35     \\
 5234.21 & $-$0.46 &  0.55 &  36.5 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   9.7 &  \nodata &  10.2 &  \nodata & 35     \\
 5249.60 &  0.08 &  0.98 &  45.2 &  14.1 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  15.2 &   9.2 &  13.3 &  \nodata & 35     \\
 5293.17 & $-$0.20 &  0.82 &  43.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  13.9 &   7.8 &  16.7 &  \nodata & 35     \\
 5311.48 & $-$0.56 &  0.99 &  10.3 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   3.1 &  \nodata & 35     \\
 5319.82 & $-$0.35 &  0.55 &  55.7 &  18.9 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  22.5 &  10.6 &  20.8 &  \nodata & 35     \\
 5361.51 & $-$0.40 &  0.68 &  37.4 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  12.3 &   6.2 &  11.4 &  \nodata & 35     \\
\multicolumn{16}{c}{ {SmII}} \\
 4035.10 & $-$0.45 &  0.33 &  \nodata &  15.7 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   5.1 &  \nodata &  \nodata & 36     \\
 4329.02 & $-$0.30 &  0.18 &  54.1 &  \nodata &  \nodata &   7.8 &   6.7 &  \nodata &  \nodata &  \nodata &  22.8 &   9.5 &  \nodata &  \nodata & 36     \\
 4452.71 & $-$0.43 &  0.28 &  66.3 &  \nodata &  \nodata &   6.7 &   4.8 &  \nodata &  \nodata &  \nodata &  24.0 &  10.3 &  \nodata &  \nodata & 36     \\
 4499.48 & $-$1.01 &  0.25 &  \nodata &  \nodata &  \nodata &   1.7 &   2.0 &  \nodata &  \nodata &  \nodata &  \nodata &   3.1 &   5.1 &  \nodata & 36     \\
 4519.64 & $-$0.43 &  0.54 &  39.3 &  10.5 &  \nodata &   3.9 &   2.1 &  \nodata &  \nodata &  \nodata &  11.9 &   5.6 &  11.9 &  \nodata & 36     \\
 4523.91 & $-$0.58 &  0.43 &  37.5 &  11.6 &  \nodata &   3.4 &   3.4 &  \nodata &  \nodata &  \nodata &  14.2 &   6.2 &  14.0 &  \nodata & 36     \\
 4537.95 & $-$0.23 &  0.48 &  24.9 &  \nodata &  \nodata &   3.2 &  \nodata &  \nodata &  \nodata &  \nodata &  11.8 &   3.8 &  13.0 &  \nodata & 36    \\
 4577.69 & $-$0.77 &  0.25 &  47.4 &   8.5 &  \nodata &   4.8 &   3.0 &  \nodata &  \nodata &  \nodata &  13.7 &   5.8 &  11.6 &  \nodata & 36     \\
 4642.23 & $-$0.52 &  0.38 &  39.7 &  12.1 &  \nodata &   5.0 &   4.0 &  \nodata &  \nodata &  \nodata &  13.9 &   6.8 &  15.3 &  \nodata & 36     \\
 
\multicolumn{16}{c}{{EuII}} \\
 3724.95 &  $-$0.08 &  0.00 & \nodata & \nodata & \nodata & syn & syn & 
\nodata & \nodata & \nodata & \nodata & syn & \nodata & \nodata & 35 \\  
 4129.70 &  0.20 &  0.00 &  syn & syn & syn & syn & syn & syn & syn & syn &
syn & syn & syn & \nodata & 35 \\
 4205.05 &  0.12 &  0.00 &  \nodata &  \nodata &  \nodata &  \nodata & syn &  
\nodata &  \nodata &  \nodata &  \nodata & syn &  syn &  \nodata & 35     \\
\multicolumn{16}{c}{ {GdII}} \\
 3331.40 & $-$0.14 & 0.00 & \nodata & \nodata & \nodata & 9.1 & \nodata &
\nodata & \nodata & \nodata & \nodata & 10.9 & \nodata & \nodata &  37 \\
 3796.39 &  0.07 &  0.03 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   7.5 &  \nodata &  \nodata &  41.8 &  \nodata &  \nodata & 37     \\
 3768.40 & 0.25 &  0.08 &  \nodata &  \nodata &  \nodata &  23.1 &  19.0 &  \nodata &   8.2 &  \nodata &  \nodata &  27.6 &  \nodata &  \nodata & 37     \\
\multicolumn{16}{c}{{TbII}} \\
 3848.74 &  0.06 &  0.00 &  \nodata &  \nodata &  \nodata &  \nodata &  syn &  \nodata &  \nodata &  \nodata &  \nodata & \nodata &  \nodata &  \nodata & 35     \\
 3874.17 &  0.28 &  0.00 &  \nodata &  \nodata &  \nodata & syn &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & syn &  \nodata &  \nodata & 35     \\
 4005.47 &  0.25 &  0.13 &  \nodata & syn & syn &  \nodata &  syn &  syn &  
syn &  syn &  \nodata &  \nodata &  syn &  syn & 35     \\
\multicolumn{16}{c}{{DyII}} \\
 3385.02 & 0.11 &  0.10 & \nodata & \nodata & \nodata & \nodata & 18.5 &
\nodata & \nodata & \nodata & \nodata & 24.4 & \nodata & \nodata & 38 \\   
 3434.37 & $-$0.43 & 0.00 &  \nodata & \nodata & \nodata & 12.1 & \nodata &
\nodata & \nodata & \nodata & \nodata & 11.6 & \nodata & \nodata & 38 \\   
 3454.32 & $-$0.13 & 0.10 & \nodata & \nodata & \nodata & \nodata & 11.5 &
\nodata & 7.6 & 12.5 & \nodata & 23.8 & \nodata & \nodata & 38 \\   
 3531.71 & 0.79 & 0.00 & \nodata & \nodata & \nodata & \nodata & 52.7 &
\nodata & 35.9 & 16.2 & \nodata & 68.0 & \nodata & \nodata & 38 \\   
 3536.02 & 0.47 &  0.54 &  \nodata & \nodata & \nodata & 22.3 & 16.4 &
\nodata & 7.3 & \nodata & \nodata & 24.4 & \nodata & \nodata & 38 \\   
 3546.83 & $-$0.57 & 0.10 &  \nodata & \nodata & \nodata & 9.8 & 5.6 &
\nodata & \nodata & \nodata & \nodata & 12.1 & \nodata & \nodata & 38 \\   
 3563.15 & $-$0.16 &  0.10 &  \nodata & \nodata & \nodata & 10.9 & 8.3 &
\nodata & \nodata & \nodata & \nodata & 11.8 & \nodata & \nodata & 38 \\   
 3606.12 & 0.26 &  0.10 &  \nodata & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & 6.9 & \nodata & \nodata & 38 \\   
 3672.31 & $-$0.39 & 0.59 &  \nodata & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & 3.2 & \nodata & \nodata & 38 \\   
 3694.82 & 0.00 & 0.10 & \nodata & \nodata & \nodata & 21.2 & 18.4 &
\nodata & \nodata & \nodata & \nodata & 27.2 & \nodata & \nodata & 38 \\   
 4073.12 & $-$0.38 &  0.54 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   9.1 &  \nodata &  \nodata & 38     \\
 4103.31 & $-$0.39 &  0.10 &  \nodata &  \nodata &  \nodata &  \nodata &  16.7 &  \nodata &  \nodata &  \nodata &  58.1 &  27.2 &  44.9 &  \nodata & 38     \\
 4449.71 & $-$0.95 &  0.00 &  \nodata &  \nodata &  \nodata &   7.8 &   5.9 &  \nodata &  \nodata &  \nodata &  30.2 &  11.9 &  \nodata &  \nodata & 38     \\
\multicolumn{16}{c}{{HoII}} \\
 3810.74 &  0.14 &  0.00 &  \nodata &  \nodata &  syn &  \nodata &  \nodata &  syn &  \nodata &  syn &  \nodata &  \nodata &  \nodata &  \nodata & 35     \\
 4152.58 & $-$0.89 &  0.08 &  \nodata &  syn &  \nodata &  syn &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  syn &  \nodata &  \nodata & 35     \\
\multicolumn{16}{c}{ {ErII}} \\
 3692.65 &   0.13 &   0.05 & \nodata & \nodata & syn & syn & syn & syn &
syn & syn & \nodata & syn & \nodata & \nodata & 35 \\ 
 3830.48 & $-$0.36 &  0.00 &  \nodata &  \nodata &  \nodata &  syn & syn  &  \nodata &  \nodata &  \nodata &  \nodata &  syn &  \nodata &  \nodata & 35     \\
 3896.23 & $-$0.24 &  0.00 &  \nodata &  \nodata &  \nodata & syn & syn & 
 \nodata &  syn &  \nodata &  \nodata &  syn &  \nodata &  \nodata & 35     \\
\multicolumn{16}{c}{ {TmII}} \\
 3700.26 &  -0.29 & 0.03 & \nodata & \nodata & \nodata & \nodata & syn & \nodata & syn & syn & \nodata & \nodata & \nodata & \nodata & 35 \\ 
 3795.76 & $-$0.17 &  0.03 &  \nodata &  \nodata &  \nodata &  \nodata &  
syn &  \nodata &  
 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 35     \\
 3848.02 & $-$0.13 &  0.00 &  \nodata &  \nodata &  syn &  syn & syn &  \nodata & \nodata &  syn &  \nodata &  syn &  \nodata &  \nodata & 35     \\
\multicolumn{16}{c}{ {YbII}} \\
 3694.19 &   $-$0.29 &  0.0 & \nodata & \nodata & syn & syn & syn & syn & syn
& syn & \nodata & syn & \nodata & \nodata & 39 \\
\multicolumn{16}{c}{{HfII}} \\
 3719.28 & $-$0.89 & 0.61 & \nodata & \nodata & \nodata & \nodata & \nodata &
syn & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 35 \\
 3793.38 & $-$0.95 &  0.38 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & syn &  \nodata &  \nodata & 35     \\
\multicolumn{16}{c}{{OsI}} \\
 4261.85 & $-$1.44 &  0.00 &  syn &  syn &  syn &  syn &  syn &  syn &  syn &  syn &  syn &  syn & \nodata &  syn & 35     \\
\enddata
\tablenotetext{a}{Line not used in abundance analysis}
\tablenotetext{b}{Line not used if EW $>$ 50.0}
\tablerefs{(1) Wiese \& Martin 1980; (2) Wiese, Smith \& Miles 1969; (3) J\"onsson 
et al. 1984;
(4) Fuhrmann, Axer, \& Gehren 1995; (5) Garz 1973; (6) Beveridge \& Sneden 1994; 
(7) Smith \& Raggett
1981; (8) Lawler \& Dakin 1989; (9) Blackwell et al.{} 1986; 
(10) Nitz et al.{} 1998; 
(11) Bizzarri et al.{} (1993); 
(12) Martin et al.{} 1988; (13) Doerr et al.{} 1985; (14) Bi\'emont
et al.{} 1989; (15) Blackwell et al.{} 1984b; (16) Tozzi et al.{} 1985; 
(17) Booth et al.{} (1983); (18) Blackwell \& Collins 1972; (19) 
Martinson et al.{}
1977; (20)Bard, Kock, \& Kock 1991; (21) O'Brian et al.{} (1991); (22) 
Blackwell et al.{} 1979a, 1979b, 1980, 1982a, 1982b, 1982c; (23) Heise
\& Kock 1990; (24) Moity 1983; (25) Kroll \& Kock 1987; (26) Bridges 1973;
(27) Hannaford et al.{} 1992; (28) Fuhr et al.{} (1988); (29) Blackwell et al.{}
 1989; (30) Wickliffe \& Lawler 1997; (31) Bi\'emont \& Godefroid 1980; 
(32) Hannaford et al.{} 1982; (33) Bi\'emont et al.{} 1981; (34) Kastberg et al. 1993; (35)
Sneden et al.{} (1996); (36) Bi\'emont et al.{} 1989; (37) Bergstr\"om et al.{}
1988; (38)Bi\'emont et al.{} 1993 (39) Pinnington et al.{} 1997b} 
\end{deluxetable}


==> tab2b.tex <==
\begin{deluxetable}{lrccccccccccccc}
\tabletypesize{\scriptsize}
\tablenum{2B}
\tablewidth{0pt}
\tablecaption{Equivalent Widths (m\AA)}
\tablehead{
\colhead{$\lambda$ (\AA)}  & \colhead{log $gf$} & \colhead{EP} 
& \multicolumn{2}{r}{$-$17 6036} & \multicolumn{2}{r}{+4 2621} & 
\multicolumn{2}{r}{+8 2856}
& \multicolumn{2}{r}{+10 2495} 
& \multicolumn{2}{r}{+18 2890} & \colhead{}
& \colhead{Source} \\
\colhead{} & \colhead{}  & \colhead{eV} &
\multicolumn{2}{l}{$-$18 5550} &\multicolumn{2}{l}{$-$11 145} & 
\multicolumn{2}{l}{+5 3098} &
\multicolumn{2}{l}{+9 3223} & \multicolumn{2}{l}{+17 3248}  & 
\multicolumn{2}{l}{VII-18}
}
\startdata
\multicolumn{15}{c}{{NaI}} \\
 5889.97 &  0.11 &  0.00 & 159.1 &  \nodata& 196.8 &  \nodata& 218.9 & 232.8 & 210.4 & 200.0 & 218.5 & 223.3 &  \nodata& 1      \\
 5895.94 & $-$0.19 &  0.00 & 127.2 & 201.5 & 173.3 &  \nodata& 180.2 & 208.7 & 167.3 & 171.9 & 174.9 & 200.3 &  \nodata& 1      \\
\multicolumn{15}{c}{{MgI}} \\
 3829.36 & 0.13 &  2.71 & 138.6 &  \nodata&  \nodata& 183.7 & 178.6 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 2      \\
 3832.31 &  0.27 &  2.71 & 163.2 & 213.2 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 2      \\
 3838.30 &  0.46 &  2.72 & 183.2 &  \nodata&  \nodata& 247.7 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 2      \\
 4167.28 & $-$0.77 &  4.34 &  37.5 &  56.1 &  58.7 &  61.3 &  60.8 &  88.4 &  60.8 &  77.3 &  70.2 &  93.5 &  \nodata& 3      \\
 4703.00 & $-$0.52 &  4.34 &  47.3 &  71.3 &  84.3 &  80.7 &  71.9 & 116.4 &  81.8 &  94.6 &  90.0 & 123.7 &  78.0 & 4      \\
 5172.70 & $-$0.39 &  2.70 & 161.9 & 208.5 & 222.3 &  \nodata& 197.5 & 276.5 & 196.8 & 234.9 & 213.1 & 366.3 &  \nodata& 4      \\
 5183.62 & $-$0.17 &  2.72 & 184.0 & 220.8 & 251.3 &  \nodata& 222.0 & 322.0 & 217.7 & 274.0 & 251.4 & 386.2 &  \nodata& 4      \\
 5528.42 & $-$0.50 &  4.34 &  50.5 &  72.4 &  93.1 &  \nodata&  75.6 & 123.0 &  81.6 &  97.5 &  92.8 & 127.3 &  \nodata& 4      \\
\multicolumn{15}{c}{{AlI}} \\
 3961.53 & $-$0.34 &  0.01 &  96.8 & 119.4 &  \nodata& 132.9 & 135.9 & 179.2 & 115.8 & 128.6 & 123.1 & 158.4 &  \nodata& 1      \\
\multicolumn{15}{c}{{SiI}} \\
 4102.94 & $-$3.14 &  1.91 &  53.8 &  68.9 &  76.8 &  87.1 &  70.1 & 107.3 &  56.5 &  79.7 &  69.2 &  91.6 &  \nodata& 5      \\
 5708.41 & $-$1.47 &  4.95 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  25.5 &  \nodata&  \nodata&  \nodata&  30.6 &  \nodata& 5      \\
 5772.15 & $-$1.75 &  5.08 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&   9.1 &  \nodata&  \nodata&  \nodata&  13.9 &  \nodata& 5      \\
 6155.14 & $-$0.84 &  5.62 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  17.3 &  \nodata&  \nodata&  \nodata&  25.4 &  \nodata& 6      \\
\multicolumn{15}{c}{{CaI}} \\
 4318.65 & $-$0.21 &  1.90 &  39.1 &  49.3 &  66.5 &  57.8 &  58.4 &  91.0 &  60.0 &  75.0 &  73.3 &  91.1 &  94.6 & 1      \\
 4425.44 & $-$0.36 &  1.88 &  34.9 &  46.1 &  62.4 &  60.3 &  53.2 &  86.6 &  52.8 &  73.9 &  68.2 &  88.4 &  76.0 & 1      \\
 4455.89 & $-$0.51 &  1.90 &  27.9 &  36.9 &  52.0 &  49.7 &  41.8 &  83.1 &  44.1 &  63.5 &  54.2 &  87.2 &  74.2 & 1      \\
 4526.94 & $-$0.55 &  2.71 &  \nodata&  \nodata&  \nodata&  10.8 &  10.5 &  23.2 &  11.6 &  19.4 &  10.5 &  38.9 &  20.5 & 7      \\
 4578.55 & $-$0.70 &  2.52 &   5.7 &   8.2 &  12.6 &  12.2 &   9.8 &  28.5 &  11.1 &  20.6 &  17.1 &  37.4 &  23.4 & 7      \\
 5261.71 & $-$0.58 &  2.52 &  \nodata&  13.7 &  19.9 &  \nodata&  14.7 &  27.9 &  17.0 &  27.0 &  25.0 &  55.5 &  \nodata& 7      \\
 5265.56 & $-$0.11 &  2.52 &  18.5 &  29.5 &  \nodata&  \nodata&  35.6 &  \nodata&  39.5 &  \nodata&  \nodata&  \nodata&  \nodata& 7      \\
 5349.47 & $-$0.31 &  2.71 &   5.2 &  11.1 &  16.5 &  \nodata&  14.2 &  36.2 &  20.2 &  28.6 &  23.9 &  56.2 &  \nodata& 7      \\
 5512.98 & $-$0.45 &  2.93 &  \nodata&  \nodata&  11.0 &  \nodata&  \nodata&  \nodata&  \nodata&  14.2 &  12.7 &  33.8 &  \nodata& 7      \\
 5581.97 & $-$0.56 &  2.52 &  \nodata&  11.6 &  27.0 &  \nodata&  14.1 &  41.1 &  19.0 &  32.2 &  25.4 &  56.0 &  \nodata& 7      \\
 5588.76 &  0.36 &  2.52 &  36.6 &  50.0 &  67.5 &  \nodata&  55.6 &  94.9 &  62.1 &  74.0 &  69.1 &  99.7 &  \nodata& 7      \\
 5590.12 & $-$0.57 &  2.52 &  \nodata&  12.3 &  \nodata&  \nodata&  18.9 &  34.8 &  16.0 &  27.6 &  20.1 &  52.5 &  \nodata& 7      \\
 5594.47 &  0.10 &  2.52 &  26.9 &  37.2 &  51.8 &  \nodata&  40.6 &  79.7 &  49.0 &  60.8 &  58.4 &  91.2 &  \nodata& 7      \\
 5601.28 & $-$0.52 &  2.52 &   8.3 &  \nodata&  22.7 &  \nodata&  15.5 &  40.0 &  \nodata&  31.0 &  27.6 &  55.3 &  \nodata& 7      \\
 6102.73 & $-$0.79 &  1.88 &  22.4 &  34.1 &  50.7 &  \nodata&  37.0 &  85.8 &  39.7 &  62.5 &  51.4 &  86.4 &  \nodata& 1      \\
 6122.23 & $-$0.32 &  1.89 &  48.0 &  62.5 &  86.9 &  \nodata&  65.8 & 120.1 &  73.6 &  89.5 &  84.8 & 109.3 &  \nodata& 1      \\
 6161.29 & $-$1.27 &  2.52 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  22.2 &  \nodata& 7      \\
 6162.18 & $-$0.09 &  1.90 &  59.7 &  70.8 & 100.8 &  \nodata&  79.1 & 129.3 &  85.4 & 100.1 &  95.1 & 132.0 &  \nodata& 1      \\
 6166.44 & $-$1.14 &  2.52 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  25.0 &  \nodata& 7      \\
 6169.56 & $-$0.48 &  2.52 &  10.9 &  15.5 &  25.9 &  \nodata&  19.4 &  51.0 &  24.8 &  36.1 &  29.8 &  56.8 &  \nodata& 7      \\
 6439.07 &  0.39 &  2.52 &  43.1 &  60.9 &  81.0 &  \nodata&  61.0 & 110.3 &  71.9 &  85.2 &  81.0 & 105.3 &  \nodata& 7      \\
 6455.60 & $-$1.29 &  2.52 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  17.2 &  \nodata& 7      \\
 6471.66 & $-$0.69 &  2.52 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  45.1 &  13.0 &  34.1 &  21.4 &  48.4 &  \nodata& 7      \\
 6493.78 & $-$0.11 &  2.52 &  23.8 &  37.9 &  46.7 &  \nodata&  \nodata&  73.2 &  \nodata&  54.4 &  \nodata&  81.2 &  \nodata& 7      \\
 6499.65 & $-$0.82 &  2.52 &  \nodata&  12.7 &  \nodata&  \nodata&   9.5 &  28.2 &  17.1 &  20.9 &  17.2 &  43.7 &  \nodata& 7      \\
 6717.69 & $-$0.52 &  2.71 &  \nodata&  \nodata&  18.4 &  \nodata&  13.7 &  39.4 &  16.3 &  27.3 &  19.3 &  57.1 &  \nodata& 7      \\
\multicolumn{15}{c}{{ScII}} \\
 4246.84 &  0.24 &  0.31 & 101.2 & 112.1 & 142.2 & 128.7 & 105.7 & 172.1 & 121.9 & 118.9 & 137.7 & 136.1 & 176.8 & 8      \\
 4294.78 & $-$1.39 &  0.61 &  \nodata&  30.9 &  \nodata&  46.5 &  26.7 &  76.8 &  26.6 &  \nodata&  34.3 &  70.2 &  \nodata& 8      \\
 4320.75 & $-$0.25 &  0.61 &  61.9 &  79.1 &  87.8 &  85.1 &  76.5 & 123.8 &  84.2 &  94.2 &  95.1 & 105.5 &  \nodata& 8      \\
 4354.61 & $-$1.58 &  0.61 &  \nodata&  24.4 &  \nodata&  \nodata&  \nodata&  63.3 &  \nodata&  \nodata&  32.8 &  \nodata&  \nodata& 8      \\
 4400.40 & $-$0.54 &  0.61 &  48.8 &  67.1 &  90.2 &  \nodata&  64.0 &  \nodata&  69.9 &  79.9 &  81.5 &  96.1 &  \nodata& 8      \\
 4415.56 & $-$0.67 &  0.60 &  43.3 &  60.5 &  78.6 &  75.0 &  56.3 & 107.3 &  64.2 &  75.3 &  78.9 &  81.6 &  \nodata& 8      \\
 4420.67 & $-$2.27 &  0.62 &  \nodata&  \nodata&  \nodata&   7.4 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 8      \\
 4431.44 & $-$1.97 &  0.61 &  \nodata&  \nodata&  15.9 &  13.6 &  \nodata&  37.2 &  \nodata&  \nodata&  \nodata&  \nodata&  38.3 & 8      \\
 4670.41 & $-$0.58 &  1.36 &  13.0 &  25.3 &  41.3 &  31.6 &  20.5 &  \nodata&  26.5 &  33.4 &  33.9 &  49.4 &  \nodata& 8      \\
 5239.82\tablenotemark{a} & $-$0.76 &  1.45 &   7.7 &  16.7 &  27.2 &  \nodata&  12.9 &  50.0 &  13.8 &  \nodata&  23.8 &  39.1 &  \nodata& 8      \\
 5318.36 & $-$2.02 &  1.36 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 8      \\
 5526.82 &  0.02 &  1.77 &  18.0 &  28.5 &  47.3 &  \nodata&  28.6 &  85.1 &  38.3 &  39.3 &  49.3 &  62.7 &  \nodata& 8      \\
 5640.99 & $-$1.13 &  1.50 &  \nodata&  \nodata&  12.8 &  \nodata&  \nodata&  35.0 &   8.0 &  12.1 &  11.6 &  21.7 &  \nodata& 8      \\
 5657.88 & $-$0.60 &  1.51 &  10.1 &  \nodata&  38.6 &  \nodata&  21.8 &  69.9 &  \nodata&  34.6 &  36.3 &  50.5 &  \nodata& 8      \\
 6604.60 & $-$1.31 &  1.36 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  29.2 &  \nodata&  \nodata&  \nodata&  21.7 &  \nodata& 8      \\
\multicolumn{15}{c}{{TiI}} \\
 3653.50 & 0.28 & 0.05 & 46.9 & 64.4 & \nodata & 69.1 & 60.1 &
101.2 & \nodata & \nodata & \nodata & \nodata & \nodata  & 9 \\
 3729.81 & $-$0.29 & 0.00 & 30.8 & 45.5 & \nodata & 65.4 & 49.4 &
109.1 & \nodata & \nodata & \nodata & \nodata & \nodata & 9 \\
 3741.06 & $-$0.15 & 0.02 & 35.9 & 52.3 & \nodata & 63.9 & 52.7 &
92.8 & \nodata & \nodata & \nodata & \nodata & \nodata & 9 \\
 3752.86 & 0.04 &  0.05 &  43.3 &  60.6 &  \nodata&  71.0 &  60.8 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 3924.53 & $-$0.88 &  0.02 &  14.4 &  22.6 &  \nodata&  36.6 &  24.1 &  67.5 &  \nodata&  44.6 &  \nodata&  60.7 &  \nodata& 9      \\
 3929.88 & $-$1.01 &  0.00 &   8.1 &  \nodata&  \nodata&  \nodata&  15.9 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 3962.85 & $-$1.11 &  0.00 &   7.8 &  \nodata&  \nodata&  25.3 &  13.9 &  46.5 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 3964.27 & $-$1.11 &  0.02 &   7.1 &  14.5 &  \nodata&  24.1 &  14.3 &  48.8 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 4112.71 & $-$1.70 &  0.05 &  \nodata&  \nodata&  \nodata&  11.5 &  \nodata&  26.2 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 4287.41 & $-$0.38 &  0.84 &  \nodata&  14.4 &  \nodata&  23.6 &  17.1 &  42.4 &  \nodata&  \nodata&  \nodata&  42.2 &  \nodata& 9      \\
 4453.32 & 0.01 &  1.50 &  \nodata&   6.8 &  \nodata&  11.6 &   8.0 &  30.4 &  \nodata&  17.9 &  \nodata&  30.0 &  30.1 & 9      \\
 4512.73 & $-$0.42 &  0.84 &   6.0 &  11.1 &  18.8 &  20.9 &  12.0 &  43.5 &  \nodata&  24.7 &  14.5 &  42.3 &  46.1 & 9      \\
 4518.02 & $-$0.26 &  0.83 &   9.5 &  15.5 &  31.5 &  25.6 &  16.3 &  48.7 &  16.9 &  25.9 &  23.1 &  47.1 &  \nodata& 9      \\
 4533.24 &  0.54 &  0.85 &  33.6 &  44.7 &  53.1 &  56.0 &  47.8 &  88.9 &  46.3 &  64.7 &  56.9 &  82.3 &  89.8 & 9      \\
 4534.78 &  0.34 &  0.84 &  24.8 &  38.1 &  48.7 &  48.1 &  39.2 &  77.8 &  40.7 &  54.3 &  44.7 &  72.7 &  82.4 & 9      \\
 4548.76 & $-$0.29 &  0.83 &   8.7 &  14.4 &  25.2 &  23.9 &  17.1 &  47.0 &  \nodata&  27.5 &  19.2 &  49.0 &  56.5 & 9      \\
 4555.49 & $-$0.43 &  0.85 &   5.9 &   9.3 &  20.8 &  17.5 &  13.4 &  38.4 &  14.4 &  23.1 &  14.9 &  39.8 &  45.2 & 9      \\
 4617.27 &  0.45 &  1.75 &   4.2 &   6.9 &  18.8 &  12.4 &  11.2 &  28.3 &  \nodata&  15.7 &  \nodata&  31.0 &  27.9 & 9      \\
 4623.10 &  0.17 &  1.74 &   2.8 &   4.9 &  \nodata&   7.4 &  \nodata&  17.2 &  \nodata&  \nodata&  \nodata&  25.6 &  15.2 & 9      \\
 4645.19 & $-$0.50 &  1.89 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  10.2 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 4656.47 & $-$1.29 &  0.00 &   8.3 &  16.3 &  24.3 &  24.7 &  12.6 &  54.2 &  12.4 &  29.5 &  20.2 &  46.2 &  79.0 & 9      \\
 4681.91 & $-$1.01 &  0.05 &  11.5 &  21.4 &  30.9 &  34.6 &  24.2 &  67.9 &  \nodata&  38.9 &  26.3 &  58.0 &  89.5 & 9      \\
 4820.42 & $-$0.38 &  1.50 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  26.0 &  \nodata&  13.4 &  \nodata&  25.3 &  \nodata& 9      \\
 4840.87 & $-$0.45 &  0.90 &  \nodata&  \nodata&  \nodata&  \nodata&  10.2 &  34.8 &  \nodata&  18.7 &  \nodata&  39.6 &  \nodata& 9      \\
 4913.62 &  0.22 &  1.87 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  17.5 &  \nodata&  \nodata&  \nodata&  19.0 &  \nodata& 9      \\
 4981.73 &  0.56 &  0.85 &  39.0 &  51.5 &  66.9 &  \nodata&  55.5 & 100.3 &  56.6 &  70.5 &  61.9 &  88.8 &  \nodata& 9      \\
 4999.50 &  0.31 &  0.83 &  27.3 &  40.6 &  60.7 &  \nodata&  44.2 &  94.9 &  40.7 &  62.1 &  55.8 &  84.8 &  \nodata& 9      \\
 5016.16 & $-$0.51 &  0.85 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  40.4 &  \nodata&  23.5 &  \nodata&  43.5 &  \nodata& 9      \\
 5020.03 & $-$0.35 &  0.84 &  \nodata&  15.5 &  28.6 &  \nodata&  14.4 &  54.5 &  \nodata&  34.8 &  20.0 &  53.0 &  \nodata& 9      \\
 5022.87 & $-$0.37 &  0.83 &  \nodata&  15.3 &  22.6 &  \nodata&  16.4 &  51.5 &  11.6 &  30.2 &  16.8 &  45.7 &  \nodata& 9      \\
 5024.84 & $-$0.54 &  0.82 &  \nodata&  12.6 &  16.0 &  \nodata&  14.6 &  46.3 &  \nodata&  19.6 &  \nodata&  43.4 &  \nodata& 9      \\
 5036.47 &  0.19 &  1.44 &  \nodata&  \nodata&  18.3 &  \nodata&  \nodata&  28.6 &  \nodata&  21.5 &  17.6 &  44.3 &  \nodata& 9      \\
 5038.40 &  0.07 &  1.43 &  \nodata&   7.4 &  \nodata&  \nodata&  \nodata&  37.4 &  \nodata&  20.3 &  14.1 &  34.9 &  \nodata& 9      \\
 5039.96 & $-$1.07 &  0.21 &  11.1 &  24.2 &  32.9 &  \nodata&  26.0 &  69.9 &  19.2 &  38.6 &  31.7 &  55.8 &  \nodata& 9      \\
 5064.65 & $-$0.93 &  0.05 &  16.0 &  24.7 &  41.3 &  \nodata&  31.8 &  79.9 &  26.7 &  45.0 &  30.8 &  63.8 &  \nodata& 9      \\
 5071.47 & $-$1.00 &  1.46 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 5113.44 & $-$0.72 &  1.44 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 5147.48 & $-$1.95 &  0.00 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  21.7 &  \nodata&   8.1 &  \nodata&  19.4 &  \nodata& 9      \\
 5173.74 & $-$1.06 &  0.00 &  11.8 &  24.6 &  40.5 &  \nodata&  25.0 &  75.8 &  18.2 &  47.5 &  24.6 &  61.2 &  \nodata& 9      \\
 5192.97 & $-$0.95 &  0.02 &  18.5 &  26.0 &  42.7 &  \nodata&  28.7 &  91.4 &  21.4 &  49.6 &  36.5 &  73.4 &  \nodata& 9      \\
 5210.39 & $-$0.82 &  0.05 &  19.2 &  33.5 &  47.4 &  \nodata&  35.9 &  82.7 &  25.5 &  55.8 &  37.9 &  72.9 &  \nodata& 9      \\
 5219.70 & $-$2.23 &  0.02 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 5224.30 &  0.13 &  2.13 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 10     \\
 5426.26 & $-$2.95 &  0.02 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 5866.45 & $-$0.78 &  1.07 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  20.8 &  \nodata&   9.5 &  \nodata&  23.9 &  \nodata& 9      \\
 5978.54 & $-$0.44 &  1.89 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
 6258.10 & $-$0.29 &  1.44 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  12.6 &  \nodata&  24.7 &  \nodata& 9      \\
 6261.10 & $-$0.42 &  1.43 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&   8.2 &  \nodata&  21.1 &  \nodata& 9      \\
 6556.06 & $-$1.01 &  1.46 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 9      \\
\multicolumn{15}{c}{{TiII}} \\
 4056.19 & $-$3.30 &  0.61 &   7.9 &  13.9 &  \nodata&  27.9 &  15.1 &  53.4 &  \nodata&  \nodata&  \nodata&  37.4 &  \nodata& 11     \\
 4394.06 & $-$1.77 &  1.22 &  36.0 &  54.0 &  71.7 &  68.6 &  44.1 & 103.6 &  61.5 &  67.6 &  71.0 &  91.1 & 102.9 & 11     \\
 4395.04 & $-$0.51 &  1.08 &  99.7 &  \nodata& 131.3 & 129.6 & 110.5 &  \nodata& 134.3 &  \nodata& 134.4 &  \nodata&  \nodata& 11     \\
 4395.84 & $-$1.97 &  1.24 &  24.7 &  38.1 &  58.1 &  51.7 &  33.8 &  85.9 &  49.4 &  57.3 &  58.9 &  68.5 &  77.2 & 11     \\
 4398.29 & $-$2.78 &  1.22 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  43.7 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 11     \\
 4409.52 & $-$2.57 &  1.23 &   7.4 &  12.7 &  \nodata&  26.6 &  15.1 &  64.4 &  19.8 &  23.7 &  \nodata&  \nodata&  \nodata& 11     \\
 4443.80 & $-$0.70 &  1.08 &  91.3 & 106.2 & 117.5 & 112.8 & 100.3 & 161.6 & 121.5 & 115.1 & 122.6 & 143.5 &  \nodata& 11     \\
 4444.56 & $-$2.21 &  1.12 &  20.3 &  35.8 &  62.5 &  49.6 &  35.5 &  88.8 &  37.7 &  51.7 &  54.9 &  69.6 &  \nodata& 11     \\
 4450.48 & $-$1.51 &  1.08 &  58.1 &  75.4 &  92.1 &  87.9 &  71.7 &  \nodata&  82.3 &  81.9 &  93.3 &  97.4 &  \nodata& 11     \\
 4468.49 & $-$0.60 &  1.13 &  92.2 & 107.2 & 130.9 & 123.1 & 104.9 & 166.5 & 122.4 & 115.6 & 128.4 & 122.4 & 176.3 & 11     \\
 4493.52 & $-$2.83 &  1.08 &   7.9 &  13.7 &  24.8 &  23.2 &  11.7 &  49.5 &  15.0 &  22.4 &  21.6 &  34.3 &  48.0 & 11     \\
 4501.27 & $-$0.76 &  1.12 &  88.5 & 104.7 & 121.8 & 118.7 &  98.9 & 159.7 & 119.4 & 110.0 & 119.1 & 122.1 & 158.2 & 11     \\
 4506.74 & $-$3.49 & 1.13 & \nodata & \nodata & \nodata & 6.6 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 11 \\
 4583.41 & $-$2.87 &  1.16 &   5.9 &  11.0 &  19.4 &  21.0 &   9.7 &  44.0 &  13.7 &  17.3 &  19.6 &  28.6 &  42.6 & 11     \\
 4609.27 & $-$3.43 &  1.18 &  \nodata&  \nodata&  \nodata&   7.9 &  \nodata&  17.8 &  \nodata&  \nodata&  \nodata&  12.2 &  21.9 & 11     \\
 4636.32 & $-$3.23 &  1.16 &   3.5 &   6.0 &  \nodata&  11.4 &  \nodata&  27.3 &  \nodata&  12.7 &  \nodata&  23.0 &  27.0 & 11     \\
 4657.20 & $-$2.32 &  1.24 &  15.6 &  24.9 &  46.7 &  39.6 &  28.4 &  70.3 &  29.3 &  37.2 &  42.5 &  54.8 &  \nodata& 11     \\
 4708.66 & $-$2.37 &  1.24 &  13.7 &  25.5 &  41.3 &  43.1 &  24.3 &  68.5 &  31.3 &  38.6 &  37.9 &  53.2 &  65.7 & 11     \\
 4764.53 & $-$2.77 &  1.24 &  \nodata&   9.3 &  26.9 &  \nodata&  11.6 &  49.1 &  14.9 &  23.0 &  20.7 &  27.5 &  \nodata& 11     \\
 4798.53 & $-$2.67 &  1.08 &  \nodata&  21.9 &  40.0 &  \nodata&  21.6 &  68.8 &  22.4 &  32.9 &  31.5 &  48.8 &  \nodata& 11     \\
 5005.17 & $-$2.73 &  1.57 &  \nodata&   8.5 &  11.8 &  \nodata&  \nodata&  31.1 &  \nodata&  \nodata&   8.5 &  18.4 &  \nodata& 11     \\
 5336.79 & $-$1.63 &  1.58 &  29.9 &  41.3 &  65.9 &  \nodata&  42.4 &  91.1 &  49.7 &  \nodata&  60.3 &  73.8 &  \nodata& 11     \\
\multicolumn{15}{c}{{VI}} \\
 3864.86\tablenotemark{b} & $-$0.44 &  0.02 &  \nodata&  \nodata&  \nodata&   6.8 &  \nodata&  20.1 &  \nodata&  \nodata&  \nodata&  \nodata&  23.7 & 12     \\
 4111.78\tablenotemark{b} &  0.41 &  0.30 &   9.8 &  13.4 &  \nodata&  23.9 &  17.4 &  46.8 &  \nodata&  29.5 &  17.7 &  53.1 &  \nodata& 12     \\
 4379.23\tablenotemark{b} &  0.55 &  0.30 &  14.8 &  21.3 &  23.1 &  38.5 &  23.8 &  73.0 &  17.3 &  45.6 &  24.6 &  74.4 &  83.6 & 13     \\
 4389.98\tablenotemark{b} &  0.27 &  0.28 &  \nodata&  15.3 &  21.9 &  27.5 &  12.3 &  48.8 &  \nodata&  \nodata&  13.0 &  54.3 &  \nodata& 13     \\
 4459.75 & $-$0.50 &  0.29 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  13.4 &  \nodata&  \nodata&  \nodata&  17.6 &  19.6 & 12     \\
 4577.18\tablenotemark{b} & $-$1.05 &  0.00 &  \nodata&  \nodata&  \nodata&   3.5 &  \nodata&  12.8 &  \nodata&  \nodata&  \nodata&  \nodata&  16.0 & 12     \\
\multicolumn{15}{c}{{VII}} \\
 3517.30\tablenotemark{b} & $-$0.21 & 1.13  &  39.6 &  56.8 & \nodata &  65.9 & 54.2 
&  90.7 &  \nodata &  \nodata &  \nodata &   \nodata &  \nodata & 
14 \\
 3545.19\tablenotemark{b} & $-$0.26 & 1.10 & 37.5 & 51.0 & \nodata & 68.0 & 60.4 
&  81.3 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata & 
14 \\ 
 3592.02\tablenotemark{b} & $-$0.26 & 1.10 &  39.6 & 53.4 & \nodata & 65.0 & 48.4 
&  85.5 &  \nodata &  \nodata &  \nodata &   \nodata &  \nodata & 
14 \\
 3732.75\tablenotemark{b} & $-$0.35 & 1.56 & 26.9 &  44.6 & \nodata & 52.6 &  33.5 
&  75.5 &  \nodata & \nodata &  \nodata &   \nodata &  \nodata  & 
14  \\
 3884.84\tablenotemark{b} & $-$1.41 &  1.79 &  \nodata&  \nodata&  \nodata&   7.1 &  \nodata&  17.4 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 14     \\
 3951.96\tablenotemark{b} & $-$0.78 &  1.48 &  15.7 &  26.8 &  \nodata&  \nodata&  25.3 &  65.3 &  35.8 &  42.4 &  50.0 &  50.8 &  \nodata& 14     \\
 4036.78\tablenotemark{b} & $-$1.59 &  1.48 &  \nodata&  \nodata&  \nodata&  14.0 &  \nodata&  26.3 &  \nodata&  \nodata&  \nodata&  32.5 &  \nodata& 14     \\
\multicolumn{15}{c}{{CrI}} \\
 4254.35\tablenotemark{a} & $-$0.11 &  0.00 &  85.2 & 101.0 & 115.8 & 117.6 &  95.9 & 152.5 & 108.5 & 114.8 & 116.0 & 135.5 &  \nodata& 15     \\
 4351.06 & $-$1.45 &  0.97 &   8.7 &  15.0 &  \nodata&  20.7 &  16.0 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 15     \\
 4545.96 & $-$1.38 &  0.94 &   7.1 &  12.3 &  19.4 &  21.4 &  \nodata&  48.0 &  13.3 &  30.6 &  14.2 &  48.1 &  52.3 & 15     \\
 4591.40 & $-$1.76 &  0.97 &   3.2 &  \nodata&  \nodata&  10.4 &  \nodata&  29.6 &  \nodata&  14.4 &  \nodata&  34.5 &  31.6 & 15     \\
 4600.76 & $-$1.26 &  1.00 &   7.1 &  11.8 &  18.1 &  23.3 &  13.1 &  50.9 &  11.2 &  30.8 &  20.1 &  53.4 &  55.7 & 15,16  \\
 4616.13 & $-$1.20 &  0.98 &   9.1 &  15.0 &  26.6 &  25.2 &  18.8 &  56.4 &  14.5 &  34.4 &  22.7 &  55.2 &  58.5 & 15,16  \\
 4626.18 & $-$1.32 &  0.97 &   7.2 &  12.9 &  16.6 &  22.1 &  13.0 &  48.7 &  \nodata&  33.3 &  19.3 &  53.5 &  54.1 & 15,16  \\
 4646.17 & $-$0.72 &  1.03 &  17.8 &  28.1 &  41.3 &  50.3 &  31.8 &  79.9 &  29.1 &  55.3 &  34.9 &  67.6 &  80.7 & 15,16  \\
 4651.29 & $-$1.46 &  0.98 &   4.8 &   9.3 &  14.2 &  17.1 &   8.7 &  43.1 &  \nodata&  25.0 &  20.2 &  42.3 &  47.0 & 15,16  \\
 5247.57 & $-$1.64 &  0.96 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  43.8 &  \nodata&  24.9 &  14.3 &  43.1 &  \nodata& 15,16  \\
 5296.70 & $-$1.40 &  0.98 &  \nodata&   9.6 &  19.8 &  \nodata&  14.1 &  54.5 &  13.5 &  30.8 &  17.9 &  53.4 &  \nodata& 15,16  \\
 5300.75 & $-$2.13 &  0.98 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  20.6 &  \nodata&   7.8 &  \nodata&  18.2 &  \nodata& 15,16  \\
 5345.81 & $-$0.98 &  1.00 &  15.4 &  22.1 &  41.3 &  \nodata&  23.9 &  73.7 &  26.0 &  50.8 &  35.2 &  69.3 &  \nodata& 15,16  \\
 5348.33 & $-$1.29 &  1.00 &  \nodata&  13.3 &  25.6 &  \nodata&  12.8 &  54.7 &  13.0 &  36.4 &  23.9 &  56.4 &  \nodata& 15,16  \\
 5409.80 & $-$0.72 &  1.03 &  23.0 &  31.8 &  50.1 &  \nodata&  34.2 &  90.8 &  36.7 &  65.7 &  44.8 &  87.6 &  \nodata& 15,16  \\
 4652.17 & $-$1.03 &  1.00 &  11.3 &  18.0 &  29.0 &  34.8 &  21.3 &  67.9 &  22.5 &  43.8 &  29.5 &  64.1 &  \nodata& 16     \\
\multicolumn{15}{c}{{CrII} } \\
 4558.66 & $-$0.66 &  4.07 &  10.5 &  16.2 &  35.4 &  28.4 &  20.2 &  54.3 &  34.6 &  33.2 &  38.8 &  51.2 &  \nodata& 12     \\
 4634.10 & $-$1.24 &  4.07 &   2.4 &   4.6 &  12.9 &  10.3 &  10.3 &  23.4 &  11.2 &  18.9 &  17.3 &  24.8 &  15.3 & 12     \\
\multicolumn{15}{c}{{MnI}} \\
 3823.51 &  0.06 &  2.14 &  10.0 &  19.1 &  \nodata&  28.9 &  17.3 &  46.6 &  \nodata&  \nodata&  31.4 &  \nodata&  34.3 & 17     \\
 4030.76\tablenotemark{a} & $-$0.47 &  0.00 &  99.3 & 117.1 & 101.2 & 136.5 & 112.4 & 182.5 & 108.1 & 134.7 & 117.0 & 163.2 &  \nodata& 17     \\
 4033.07\tablenotemark{a} & $-$0.62 &  0.00 &  83.3 & 100.1 & 117.8 & 117.0 &  97.5 & 174.0 & 100.8 & 124.3 & 113.4 & 147.9 &  \nodata& 17     \\
 4034.49\tablenotemark{a} & $-$0.81 &  0.00 &  80.7 &  99.3 & 105.6 & 114.7 &  98.2 & 151.5 &  89.8 & 131.3 & 104.4 & 133.5 &  \nodata& 17     \\
 4055.55 & $-$0.07 &  2.14 &   9.8 &  14.8 &  \nodata&  27.6 &  15.3 &  50.7 &  \nodata&  32.2 &  31.7 &  63.3 &  45.2 & 17     \\
 4082.94 & $-$0.35 &  2.18 &   4.3 &   8.8 &  \nodata&  17.3 &  \nodata&  29.4 &  \nodata&  \nodata&  \nodata&  44.1 &  28.4 & 17     \\
 4709.72 & $-$0.34 &  2.89 &  \nodata&  \nodata&   9.3 &   3.2 &  \nodata&  16.6 &  \nodata&  \nodata&  \nodata&  16.0 &  12.5 & 17     \\
 4754.04 & $-$0.09 &  2.28 &  \nodata&  \nodata&  17.9 &  \nodata&  11.8 &  49.0 &  14.9 &  31.2 &  18.8 &  58.0 &  \nodata& 17     \\
 4761.53 & $-$0.14 &  2.95 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  10.2 &  \nodata& 17     \\
 4783.42 &  0.04 &  2.30 &  11.5 &  \nodata&  22.4 &  \nodata&  16.3 &  65.4 &  \nodata&  38.3 &  22.3 &  59.2 &  \nodata& 17     \\
 5432.55 & $-$3.80 &  0.00 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 17     \\
 6021.80 &  0.03 &  3.08 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  18.1 &  \nodata& 17     \\
 4070.28 & $-$0.95 &  2.19 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  35.3 &  \nodata& 18     \\
\multicolumn{15}{c}{{MnII} } \\
 3441.99 & $-$0.27 & 1.78 & 76.1 & 93.4 & \nodata & 99.2 & \nodata & 
123.9 & \nodata & \nodata & \nodata & \nodata & \nodata & 19 \\
 3460.32 & $-$0.54 & 1.81 & 63.7 & 82.3 & \nodata & 95.0 & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 19 \\
 3488.68 & $-$0.86 & 1.85 & 57.8 & 65.8 & \nodata & 81.6 & 55.1 & 
107.8 & \nodata & \nodata & \nodata & \nodata & \nodata & 19 \\
 3497.53 & $-$1.33 & 1.85 & 39.8 & 50.6 & \nodata & 69.8 & 48.1 & 
77.3 & \nodata & \nodata & \nodata & \nodata & \nodata & 19 \\
\multicolumn{15}{c}{{FeI} } \\
 3246.48 & $-$1.41 &  2.59 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata  & 20 \\
 3406.79 & $-$1.04 &  2.22 & \nodata & 56.4 & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 20 \\
 3442.36 & $-$1.35 &  2.28 & 24.0 & 39.7 & \nodata & 43.0 & \nodata  & 
61.0 & \nodata & \nodata & \nodata & \nodata & \nodata &  22 \\
 3617.78 & $-$0.05 &  3.02 & 38.9 & 49.5 & \nodata & 56.4 & 51.1 & 
89.1 & \nodata & \nodata & \nodata & \nodata & \nodata & 20 \\
 3628.81 & $-$2.21 &  2.99 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 20 \\
 3633.83 & $-$1.54 &  2.99 & \nodata & \nodata & \nodata & 13.7 & \nodata & 
36.5 & \nodata & \nodata & \nodata & \nodata & \nodata & 20 \\
 3709.25 & $-$0.61 &  0.92 & 117.9 & 136.2 & \nodata & \nodata & 127.7 & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 22 \\
 3715.91 & $-$1.53 &  2.28 & 23.1 & 39.0 & \nodata & 47.5 & 33.2 & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 22 \\
 3760.05 & $-$0.81 &  2.40 &  48.3 &  60.4 &  \nodata&  72.8 &  63.9 &  99.8 &
\nodata&  \nodata&  \nodata&  \nodata&  \nodata& 22     \\
 3767.19 & $-$0.35 &  1.01 & 127.2 & 140.8 &  \nodata&  \nodata& 136.9 &  
\nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 22     \\
 3777.45 & $-$1.74 &  2.56 &  \nodata&  18.9 &  \nodata&  29.0 &  14.5 &  63.9
& \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 22     \\
 3786.67 & $-$2.16 &  1.01 &  63.8 &  77.9 &  \nodata&  87.0 &  74.0 &  
\nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 20     \\
 3787.88 & $-$0.82 &  1.01 & 108.8 & 126.4 &  \nodata& 137.2 & 122.8 & 183.7 &
\nodata&  \nodata&  \nodata&  \nodata&  \nodata& 22     \\
 3790.10 & $-$1.72 &  0.99 &  79.5 &  92.7 &  \nodata&  \nodata&  77.2 &  
\nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 22     \\
 3808.73 & $-$1.12 &  2.56 &  29.0 &  43.6 &  \nodata&  53.6 &  41.6 &  81.9 
&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 22     \\
 3849.97 & $-$0.83 &  1.01 & 110.2 & 129.4 &  \nodata& 133.9 & 112.4 &  
\nodata&  \nodata&  \nodata& 129.2 &  \nodata&  \nodata& 22     \\
 3856.37 & $-$1.25 &  0.05 & 140.6 & 155.1 &  \nodata& 162.9 & 146.2 &  
\nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 22     \\
 3886.28 & $-$1.04 &  0.05 & 155.4 & 175.7 &  \nodata&  \nodata& 168.6 &  
\nodata&  \nodata&  \nodata& 169.0 &  \nodata&  \nodata& 22     \\
 3887.05 & $-$1.10 &  0.92 & 104.5 & 117.8 &  \nodata& 135.1 & 111.4 &  
\nodata&  \nodata&  \nodata& 127.6 &  \nodata&  \nodata& 22     \\
 3899.71 & $-$1.49 &  0.09 & 128.8 & 143.5 &  \nodata& 153.7 & 138.6 & 205.5 &
\nodata&  \nodata& 142.4 &  \nodata&  \nodata& 22     \\
 3906.48 & $-$2.20 & 0.11 & \nodata & \nodata & \nodata & 129.7 & \nodata 
& \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 22 \\
 3916.74 & $-$0.56 &  3.24 &  18.9 &  27.8 &  \nodata&  39.2 &  31.5 &  48.6 & 
\nodata&  49.1 &  \nodata&  \nodata&  \nodata& 20     \\
 3917.18 & $-$2.15 &  0.99 &  73.2 &  84.9 &  \nodata& 102.4 &  79.3 & 129.6 &
\nodata&  92.0 &  89.5 &  98.6 &  \nodata& 21     \\
 3920.26 & $-$1.71 &  0.12 & 117.6 & 130.9 &  \nodata&  \nodata& 125.5 &  
\nodata&  \nodata& 134.7 & 130.3 & 147.8 &  \nodata& 22     \\
 3922.91 & $-$1.61 &  0.05 & 128.8 & 143.2 &  \nodata& 164.0 & 138.9 & 222.5 &
\nodata& 162.2 &  \nodata&  \nodata&  \nodata& 22     \\
 3949.96 & $-$1.25 &  2.17 &  46.2 &  56.5 &  \nodata&  62.2 &  61.1 &  96.7 &
55.2 &  66.4 &  67.4 &  80.9 &  \nodata& 21     \\
 4067.28 & $-$1.38 &  2.56 &  22.0 &  33.2 &  \nodata&  45.1 &  37.0 &  85.2 &
38.6 &  56.8 &  56.7 &  71.6 &  \nodata& 22     \\
 4072.51 & $-$1.44 &  3.43 &  \nodata&  \nodata&  \nodata&  \nodata&  
\nodata&  21.5 &  \nodata&  \nodata&  \nodata&  35.2 &  \nodata& 20     \\
 4076.64 & $-$0.53 &  3.21 &  28.9 &  37.0 &  \nodata&  53.6 &  42.9 &  
\nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 21     \\
 4091.55 & $-$2.07 &  2.83 &  \nodata&  \nodata&  \nodata&   8.0 &  \nodata&  
21.7 &  \nodata&  \nodata&  \nodata&  23.5 &  \nodata& 20     \\
 4114.45 & $-$1.30 &  2.83 &  14.4 &  23.5 &  \nodata&  35.1 &  24.8 &  59.3 &
25.9 &  42.6 &  34.5 &  62.0 &  \nodata& 21     \\
 4132.91 & $-$1.00 &  2.84 &  22.7 &  33.9 &  39.6 &  43.8 &  34.5 &  77.3 & 
41.0 &  59.3 &  47.0 &  73.7 &  \nodata& 21     \\
 4139.93 & $-$3.59 &  0.99 &  11.7 &  20.1 &  \nodata&  35.6 &  15.6 &  69.0 &
\nodata&  38.3 &  18.7 &  55.1 &  82.3 & 22     \\
 4147.68 & $-$2.06 &  1.49 &  49.6 &  65.8 &  75.4 &  80.0 &  59.2 & 111.1 & 
 58.0 &  78.0 &  71.2 &  90.4 &  \nodata& 22     \\
 4154.50 & $-$0.69 &  2.83 &  34.1 &  46.3 &  56.7 &  \nodata&  48.8 &  78.2 
& 48.9 &  62.9 &  58.7 &  81.9 &  \nodata& 21     \\
 4156.81 & $-$0.81 &  2.83 &  33.9 &  46.3 &  63.4 &  \nodata&  50.4 &  
\nodata&  56.4 &  \nodata&  63.0 &  \nodata&  \nodata& 21     \\
 4157.79 & $-$0.40 &  3.42 &  23.8 &  33.4 &  38.0 &  44.3 &  34.3 &  70.2 &  
40.8 &  59.9 &  41.1 &  66.4 &  \nodata& 21     \\
 4174.92 & $-$2.93 &  0.92 &  43.8 &  56.2 &  64.6 &  \nodata&  58.9 & 110.4 
& 48.7 &  83.0 &  60.3 &  90.8 &  \nodata& 22     \\
 4175.64 & $-$0.83 &  2.85 &  31.1 &  44.2 &  50.4 &  50.5 &  43.5 &  86.7 & 
 51.5 &  67.4 &  59.5 &  78.9 &  \nodata& 21     \\
 4182.39 & $-$1.18 &  3.02 &   9.9 &  18.9 &  \nodata&  26.2 &  22.0 &  54.2 &
 20.9 &  38.1 &  \nodata&  57.3 &  \nodata& 21     \\
 4187.04 & $-$0.51 &  2.45 &  65.0 &  77.0 &  85.7 &  87.4 &  73.6 &  \nodata&
  84.2 &  94.3 &  88.2 & 102.7 &  \nodata& 22     \\
 4195.34 & $-$0.49 &  3.33 &  27.5 &  41.2 &  39.6 &  51.8 &  42.6 &  78.2 &  
\nodata&  67.6 &  47.4 &  76.4 &  \nodata& 21     \\
 4202.03 & $-$0.67 &  1.49 & 103.7 & 112.0 & 126.1 &  \nodata& 110.4 &  
\nodata& 111.5 & 126.2 & 119.8 & 150.9 &  \nodata& 22     \\
 4216.19 & $-$3.32 &  0.00 &  77.0 &  89.4 & 105.4 &  99.6 &  81.0 & 142.7 &  
80.7 &  95.4 &  88.6 & \nodata &  \nodata& 22     \\
 4222.22 & $-$0.93 &  2.45 &  47.7 &  64.0 &  70.9 &  66.7 &  61.1 & 106.6 &  
64.3 &  79.3 &  67.9 &  88.8 & 108.7 & 22     \\
 4224.18 & $-$0.51 &  3.37 &  20.7 &  26.7 &  32.9 &  37.8 &  28.8 &  68.8 &  
36.7 &  51.7 &  46.7 &  \nodata&  \nodata& 21     \\
 4227.44 &  0.27 &  3.33 &  58.9 &  78.6 &  72.1 &  92.9 &  78.4 &  \nodata&  
86.7 & 112.9 & 103.8 &  \nodata&  \nodata& 21     \\
 4233.61 & $-$0.56 &  2.48 &  62.5 &  75.8 &  76.7 &  84.7 &  72.0 &  \nodata&
 73.8 &  90.3 &  85.2 &  \nodata &  \nodata& 22     \\
 4250.13 & $-$0.37 &  2.47 &  69.7 &  80.4 &  98.1 &  96.6 &  76.5 & 125.9 &  
88.9 &  99.6 &  94.8 & 107.9 &  \nodata& 22     \\
 4260.47 &  0.14 &  2.40 &  89.5 & 104.1 & 123.2 & 116.7 & 102.3 & 156.9 & 
111.4 & 128.2 & 113.9 &  \nodata&  \nodata& 20     \\
 4271.76 & $-$0.12 &  1.49 &  \nodata& 141.6 & 168.6 & 154.4 & 138.7 &  
\nodata& 143.2 & 184.1 & 158.9 & 225.4 &  \nodata& 22     \\
 4282.41 & $-$0.78 &  2.17 &  65.6 &  78.1 &  92.6 &  87.0 &  77.3 &  \nodata&
76.1 &  96.9 &  92.3 & 111.4 &  \nodata& 21     \\
 4337.05 & $-$1.66 &  1.56 &  65.7 &  76.1 &  91.4 &  90.6 &  73.2 & 129.3 &  
76.4 &  97.0 &  \nodata& 103.8 &  \nodata& 22     \\
 4347.24 & $-$5.46 &  0.00 &  \nodata&   6.3 &  \nodata&  13.4 &  \nodata&  
39.9 &  \nodata&  \nodata&  \nodata&  26.5 &  \nodata& 22     \\
 4375.93 & $-$2.99 &  0.00 &  91.5 & 103.3 & 114.8 & 113.4 &  99.2 & 159.5 &  
89.6 & 110.3 & 100.2 & 120.0 &  \nodata& 22     \\
 4383.55 &  0.24 &  1.49 &  \nodata& 163.6 & 184.0 &  \nodata& 164.0 &  
\nodata & 168.2 &  \nodata& 181.3 &  \nodata&  \nodata& 22     \\
 4388.41 & $-$0.68 &  3.60 &  11.6 &  14.9 &  21.7 &  24.1 &  19.4 &  47.7 &  
19.7 &  36.2 &  25.4 &  52.5 &  \nodata& 21     \\
 4389.24 & $-$4.54 &  0.05 &  19.6 &  30.5 &  40.8 &  46.8 &  29.5 &  92.6 &  
17.2 &  45.5 &  28.9 &  60.7 & 117.9 & 22     \\
 4404.75 & $-$0.10 &  1.56 & 128.0 & 136.0 & 150.8 & 160.0 & 135.8 &  \nodata& 
144.0 & 178.6 & 154.9 &  \nodata&  \nodata& 22     \\
 4415.13 & $-$0.62 &  1.61 & 102.2 & 120.3 & 130.2 &  \nodata& 114.8 & 175.5 &
116.0 &  \nodata& 128.4 & 164.1 &  \nodata& 21     \\
 4427.31 & $-$3.00 &  0.05 &  94.9 & 103.5 & 111.7 & 118.6 &  99.6 & 165.3 &  
93.2 & 117.1 & 109.4 & 121.0 &  \nodata& 22     \\
 4430.62 & $-$1.62 &  2.22 &  29.4 &  42.8 &  50.1 &  52.3 &  41.9 &  94.1 &  
39.5 &  65.5 &  49.4 &  83.3 &  \nodata& 22     \\
 4439.88 & $-$2.96 &  2.28 &   3.3 &  \nodata&  \nodata&   5.9 &  \nodata&  19
.2 &  \nodata&  \nodata&  \nodata&  20.6 &  19.7 & 22     \\
 4443.20 & $-$1.04 &  2.86 &  21.3 &  30.4 &  43.7 &  37.7 &  30.4 &  77.1 &  
32.1 &  60.0 &  47.0 &  72.9 &  \nodata& 21     \\
 4445.48 & $-$5.40 &  0.09 &  \nodata&   4.6 &  11.5 &  12.1 &  \nodata&  38.9
 &  \nodata&  \nodata&  \nodata&  23.8 &  66.9 & 22     \\
 4447.73 & $-$1.34 &  2.22 &  44.9 &  61.9 &  74.0 &  70.1 &  61.7 & 112.1 &  
57.8 &  82.1 &  70.5 &  97.5 &  \nodata& 21     \\
 4454.39 & $-$1.30 &  2.83 &  15.3 &  23.7 &  35.3 &  33.2 &  25.6 &  66.9 &  
25.7 &  51.4 &  34.3 &  61.7 &  \nodata& 21     \\
 4461.65 & $-$3.17 &  0.09 &  84.5 &  93.9 & 112.0 & 112.8 &  86.7 &  \nodata&
  82.3 &  95.4 &  72.4 & 107.8 &  \nodata& 22     \\
 4471.68 & $-$5.95 &  0.11 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  15.0 &  \nodata&  \nodata&  \nodata&  \nodata&  28.3 & 22     \\
 4484.23 & $-$0.86 &  3.60 &   9.1 &  13.7 &  23.0 &  22.2 &  21.0 &  49.1 &  
20.6 &  33.8 &  23.3 &  52.5 &  \nodata& 21     \\
 4489.74 & $-$3.93 &  0.12 &  45.5 &  59.8 &  75.2 &  73.8 &  57.8 & 122.9 &  
41.6 &  80.3 &  53.4 &  87.7 &  \nodata& 22     \\
 4494.57 & $-$1.10 &  2.20 &  57.0 &  71.0 &  82.9 &  80.8 &  67.7 & 122.7 &  
69.3 &  85.2 &  83.1 &  96.1 & 130.8 & 22     \\
 4531.15 & $-$2.11 &  1.49 &  49.6 &  63.5 &  79.2 &  82.5 &  57.5 &  91.9 &  
57.7 &  82.2 &  66.6 &  97.7 &  \nodata& 22     \\
 4602.01 & $-$3.11 &  1.61 &   8.5 &  15.1 &  29.8 &  23.3 &  11.9 &  57.5 &  
 8.6 &  30.9 &  16.7 &  47.1 &  72.0 & 22     \\
 4602.94 & $-$2.18 &  1.49 &  48.3 &  64.2 &  84.9 &  75.3 &  64.5 & 119.3 &  
54.3 &  78.1 &  67.8 &  89.9 & 131.1 & 22     \\
 4630.13 & $-$2.59 &  2.28 &   6.1 &   7.7 &  19.5 &  17.9 &  10.3 &  49.2 &  
\nodata&  26.2 &  15.1 &  41.4 &  \nodata& 21     \\
 4632.92 & $-$2.90 &  1.61 &  13.7 &  22.5 &  33.1 &  37.5 &  24.3 &  78.2 &  
\nodata&  46.4 &  23.8 &  71.3 &  \nodata& 21     \\
 4635.85 & $-$2.36 &  2.84 &  \nodata&  \nodata&  \nodata&   5.5 &  \nodata&  
17.8 &  \nodata&  \nodata&  \nodata&  24.9 &  \nodata& 21     \\
 4643.46 & $-$1.15 &  3.64 &   3.1 &  \nodata&  13.2 &   7.4 &  \nodata&  22.4
 &   6.4 &  \nodata&  \nodata&  29.9 &  \nodata& 21     \\
 4647.43 & $-$1.35 &  2.94 &  11.6 &  20.7 &  32.1 &  31.2 &  22.6 &  63.9 &  
19.1 &  41.4 &  33.2 &  61.2 &  \nodata& 21     \\
 4673.17 & $-$1.06 &  3.65 &   3.4 &  \nodata&  \nodata&  10.0 &  \nodata&  24
.1 &  \nodata&  17.9 &  13.2 &  39.4 &  \nodata& 21     \\
 4678.85 & $-$0.83 &  3.59 &  10.6 &  16.5 &  25.8 &  20.9 &  20.4 &  51.7 &  
18.0 &  38.4 &  26.9 &  57.4 &  \nodata& 21     \\
 4683.57 & $-$2.32 &  2.83 &  \nodata&  \nodata&  \nodata&   4.1 &  \nodata&  
14.4 &  \nodata&  \nodata&  \nodata&  19.0 &  \nodata& 21     \\
 4690.14 & $-$1.64 &  3.69 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
   9.8 &  \nodata&  \nodata&  \nodata&  17.1 &  \nodata& 21     \\
 4691.41 & $-$1.52 &  2.98 &   8.6 &  15.2 &  25.7 &  27.0 &  19.0 &  65.3 &  
22.0 &  39.2 &  26.9 &  66.6 &  \nodata& 21     \\
 4710.28 & $-$1.61 &  3.00 &   7.6 &  12.2 &  19.7 &  21.0 &  11.3 &  51.4 &  
12.9 &  31.5 &  19.5 &  56.8 &  \nodata& 21     \\
 4733.60 & $-$2.95 &  1.49 &  17.5 &  22.8 &  41.3 &  \nodata&  27.8 &  76.6 &
  19.9 &  48.3 &  28.1 &  66.0 &  \nodata& 22     \\
 4736.77 & $-$0.75 &  3.20 &  24.6 &  33.8 &  50.8 &  \nodata&  33.4 &  83.4 &
  36.9 &  58.2 &  47.1 &  76.1 &  \nodata& 21     \\
 4800.65 & $-$1.03 &  4.12 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  29.3 &  \nodata& 21     \\
 4859.74 & $-$0.76 &  2.86 &  \nodata&  \nodata&  \nodata&  \nodata&  64.6 & 
102.2 &  \nodata&  67.2 &  \nodata&  \nodata&  \nodata& 21     \\
 4871.32 & $-$0.36 &  2.85 &  53.2 &  65.7 &  83.2 &  \nodata&  69.6 & 121.7 &
  78.2 &  87.6 &  82.6 & 109.8 &  \nodata& 21     \\
 4872.14 & $-$0.57 &  2.87 &  44.2 &  54.9 &  68.6 &  \nodata&  59.8 &  94.0 &
  55.6 &  83.6 &  71.8 &  99.3 &  \nodata& 21     \\
 4890.75 & $-$0.39 &  2.86 &  50.3 &  66.4 &  82.4 &  \nodata&  69.3 & 123.2 &
  72.4 &  89.8 &  85.6 & 108.8 &  \nodata& 21     \\
 4891.49 & $-$0.11 &  2.84 &  68.1 &  81.8 &  95.2 &  \nodata&  77.1 & 124.7 &
  86.6 & 102.6 &  98.3 & 121.6 &  \nodata& 21     \\
 4903.31 & $-$0.93 &  2.87 &  30.5 &  40.8 &  60.1 &  \nodata&  40.9 &  92.4 &
  45.1 &  70.9 &  58.8 &  86.5 &  \nodata& 21     \\
 4918.99 & $-$0.34 &  2.85 &  50.3 &  66.6 &  81.1 &  \nodata&  67.8 & 121.7 &
  72.3 &  92.3 &  75.9 & 108.8 &  \nodata& 21     \\
 4920.50 &  0.07 &  2.82 &  75.2 &  86.8 & 120.5 &  \nodata&  88.6 & 160.0 &  
95.2 & 118.0 & 114.4 & 142.0 &  \nodata& 21     \\
 4924.77 & $-$2.25 &  2.28 &  \nodata&  18.6 &  30.9 &  \nodata&  21.3 &  69.4
 &  15.5 &  40.1 &  \nodata&  62.0 &  \nodata& 20     \\
 4930.32 & $-$1.20 &  3.96 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  14.9 &  \nodata&  \nodata&  \nodata&  17.9 &  \nodata& 20     \\
 4938.81 & $-$1.08 &  2.86 &  21.1 &  29.6 &  47.5 &  \nodata&  32.2 &  83.9 &
  31.3 &  55.9 &  43.2 &  78.8 &  \nodata& 21     \\
 4939.69 & $-$3.30 &  0.86 &  33.1 &  50.3 &  67.6 &  \nodata&  45.5 & 112.2 &
  29.5 &  66.9 &  49.7 &  81.3 &  \nodata& 22     \\
 4994.13 & $-$3.04 &  0.92 &  44.3 &  57.7 &  81.2 &  \nodata&  57.3 & 121.4 &
  45.1 &  77.4 &  60.8 &  89.6 &  \nodata& 22     \\
 5006.12 & $-$0.66 &  2.83 &  51.5 &  59.6 &  64.4 &  \nodata&  61.0 & 105.7 &
  65.1 &  81.3 &  76.6 &  95.3 &  \nodata& 20     \\
 5039.25 & $-$1.57 &  3.35 &  \nodata &   6.3 &  14.5 &  \nodata&  \nodata&  31.1
 &  \nodata&  17.7 &  \nodata&  44.2 &  \nodata& 21     \\
 5041.07 & $-$3.09 &  0.95 &  43.0 &  65.3 &  81.2 &  \nodata&  60.8 &  
\nodata&  49.9 &  94.2 &  69.5 &  \nodata&  \nodata& 21     \\
 5048.44 & $-$1.03 &  3.94 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  23.8 &  \nodata& 21     \\
 5049.82 & $-$1.34 &  2.28 &  43.2 &  58.7 &  73.7 &  \nodata&  60.3 & 108.2 &
  54.2 &  78.4 &  71.3 &  98.7 &  \nodata& 20     \\
 5051.64 & $-$2.76 &  0.92 &  62.8 &  75.3 &  93.6 &  \nodata&  70.7 & 137.7 &
  63.6 &  88.6 &  76.9 & 105.3 &  \nodata& 22     \\
 5068.77 & $-$1.04 &  2.93 &  21.8 &  27.8 &  46.0 &  \nodata&  35.9 &  76.7 &
  31.3 &  56.2 &  41.6 &  75.2 &  \nodata& 21     \\
 5079.23 & $-$2.03 &  2.20 &  22.8 &  27.0 &  42.8 &  \nodata&  26.0 &  91.9 &
  28.4 &  55.1 &  36.8 &  75.4 &  \nodata& 22     \\
 5079.74 & $-$3.18 &  0.99 &  31.4 &  42.6 &  67.7 &  \nodata&  46.0 & 113.5 &
  31.7 &  72.1 &  49.6 &  88.2 &  \nodata& 22     \\
 5083.34 & $-$2.92 &  0.96 &  48.4 &  66.7 &  83.4 &  \nodata&  61.7 & 123.9 &
  49.1 &  81.2 &  65.4 &  94.1 &  \nodata& 22     \\
 5123.72 & $-$3.03 &  1.01 &  41.1 &  55.9 &  75.4 &  \nodata&  51.2 & 122.2 &
  40.2 &  79.2 &  64.3 &  98.8 &  \nodata& 22     \\
 5127.36 & $-$3.27 &  0.92 &  32.9 &  46.8 &  66.2 &  \nodata&  45.8 & 115.2 &
  30.1 &  69.5 &  52.2 &  80.9 &  \nodata& 22     \\
 5141.73 & $-$1.96 &  2.42 &   9.1 &  12.9 &  21.7 &  \nodata&  14.3 &  25.9 &
  12.4 &  33.8 &  19.2 &  51.5 &  \nodata& 20     \\
 5142.93 & $-$3.08 &  0.96 &  38.3 &  \nodata&  76.4 &  \nodata&  54.6 & 131.7
 &  42.2 &  81.1 &  58.4 & 112.8 &  \nodata& 20     \\
 5151.92 & $-$3.28 &  1.01 &  26.0 &  43.7 &  59.3 &  \nodata&  \nodata& 104.7
 &  25.7 &  62.5 &  \nodata&  74.8 &  \nodata& 22     \\
 5166.29 & $-$4.16 &  0.00 &  49.5 &  65.9 &  82.4 &  \nodata&  59.0 & 128.0 &
  40.5 &  83.8 &  58.3 &  90.4 &  \nodata& 22     \\
 5171.60 & $-$1.75 &  1.49 &  75.4 &  86.3 & 102.9 &  \nodata&  85.9 & 146.2 &
  86.1 &  99.8 &  92.4 & 120.5 &  \nodata& 22     \\
 5191.45 & $-$0.55 &  3.03 &  36.2 &  47.5 &  71.7 &  \nodata&  53.8 & 111.5 &
  55.8 &  78.5 &  69.7 & 104.9 &  \nodata& 21     \\
 5192.34 & $-$0.42 &  2.99 &  44.3 &  57.5 &  71.4 &  \nodata&  59.9 & 107.1 &
  61.6 &  78.8 &  70.7 & 101.9 &  \nodata& 21     \\
 5194.94 & $-$2.05 &  1.56 &  57.3 &  68.2 &  93.3 &  \nodata&  69.8 &  
\nodata&  \nodata&  85.0 &  76.3 &  96.8 &  \nodata& 22     \\
 5198.71 & $-$2.09 &  2.22 &  \nodata&  23.9 &  \nodata&  \nodata&  \nodata&  
77.4 &  21.4 &  42.1 &  \nodata&  72.2 &  \nodata& 22     \\
 5215.18 & $-$0.87 &  3.27 &  15.8 &  22.1 &  32.6 &  \nodata&  22.8 &  64.2 &
  22.7 &  44.1 &  32.4 &  64.4 &  \nodata& 20     \\
 5216.28 & $-$2.11 &  1.61 &  49.6 &  62.1 &  84.1 &  \nodata&  62.3 & 117.8 &
  53.1 &  83.9 &  67.8 &  91.4 &  \nodata& 22     \\
 5217.39 & $-$1.07 &  3.21 &  11.9 &  16.3 &  29.8 &  \nodata&  20.4 &  62.0 &
  21.3 &  38.7 &  29.2 &  63.8 &  \nodata& 20     \\
 5225.53 & $-$4.75 &  0.11 &  15.6 &  24.8 &  38.2 &  \nodata&  23.0 &  90.9 &
  10.2 &  45.5 &  18.5 &  59.8 &  \nodata& 22     \\
 5232.94 & $-$0.10 &  2.94 &  66.9 &  78.8 & 101.7 &  \nodata&  76.7 & 130.0 &
  82.4 &  99.1 &  88.8 & 123.1 &  \nodata& 20     \\
 5242.49 & $-$0.97 &  3.62 &  \nodata&  \nodata&  15.6 &  \nodata&  11.1 &  
\nodata&  \nodata&  25.0 &  16.2 &  40.7 &  \nodata& 21     \\
 5247.05 & $-$4.91 &  0.09 &  10.7 &  17.8 &  25.5 &  \nodata&  18.8 &  77.2 &
  \nodata&  36.0 &  15.5 &  55.6 &  \nodata& 22     \\
 5250.21 & $-$4.90 &  0.12 &   9.8 &  17.1 &  25.7 &  \nodata&  17.2 &  80.9 &
   7.4 &  40.5 &  15.7 &  50.6 &  \nodata& 22     \\
 5253.46 & $-$1.57 &  3.28 &  \nodata&  \nodata&  \nodata&  \nodata&   8.3 &  
33.0 &  \nodata&  15.0 &  \nodata&  34.2 &  \nodata& 20     \\
 5263.31 & $-$0.88 &  3.27 &  13.8 &  24.3 &  36.6 &  \nodata&  24.4 &  71.4 &
  27.0 &  46.0 &  36.0 &  67.9 &  \nodata& 20     \\
 5266.56 & $-$0.38 &  2.99 &  49.1 &  59.0 &  76.8 &  \nodata&  57.3 & 112.6 &
  61.8 &  85.1 &  75.2 & 105.6 &  \nodata& 21     \\
 5269.54 & $-$1.33 &  0.86 & 129.3 & 138.6 & 164.9 &  \nodata& 132.9 & 216.0 &
 136.5 & 156.1 & 149.1 & 192.8 &  \nodata& 21     \\
 5281.79 & $-$0.83 &  3.03 &  23.3 &  34.9 &  51.0 &  \nodata&  39.3 &  88.8 &
  37.6 &  60.9 &  49.2 &  83.3 &  \nodata& 21     \\
 5283.62 & $-$0.52 &  3.23 &  32.8 &  43.3 &  63.6 &  \nodata&  44.6 & 101.3 &
  47.9 &  70.2 &  57.2 &  88.0 &  \nodata& 21     \\
 5288.53 & $-$1.51 &  3.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  16.8 &  \nodata& 21     \\
 5302.30 & $-$0.72 &  3.28 &  20.5 &  26.9 &  42.5 &  \nodata&  27.6 &  77.8 &
  30.8 &  54.9 &  40.2 &  73.9 &  \nodata& 20     \\
 5307.37 & $-$2.95 &  1.61 &  12.6 &  19.5 &  33.3 &  \nodata&  22.4 &  74.3 &
  15.4 &  43.9 &  27.5 &  64.2 &  \nodata& 22     \\
 5332.90 & $-$2.78 &  1.55 &  17.6 &  26.8 &  48.2 &  \nodata&  28.4 &  87.0 &
  20.3 &  55.0 &  31.5 &  70.4 &  \nodata& 21     \\
 5339.93 & $-$0.65 &  3.27 &  19.1 &  31.4 &  48.1 &  \nodata&  37.2 &  82.3 &
  \nodata&  57.7 &  44.1 &  76.1 &  \nodata& 20     \\
 5341.02 & $-$1.95 &  1.60 &  62.1 &  \nodata&  96.7 &  \nodata&  73.1 & 132.4
 &  67.2 &  92.3 &  83.2 & 112.2 &  \nodata& 21     \\
 5365.40 & $-$1.02 &  3.56 &  \nodata&  \nodata&  \nodata&  \nodata&   7.6 &  
28.0 &  \nodata&  20.5 &   8.8 &  35.8 &  \nodata& 21     \\
 5367.48 &  0.44 &  4.41 &  13.2 &  18.8 &  32.2 &  \nodata&  21.9 &  61.5 &  
29.5 &  43.0 &  36.9 &  64.9 &  \nodata& 20     \\
 5369.96 &  0.54 &  4.35 &  14.9 &  25.2 &  38.2 &  \nodata&  25.9 &  69.3 &  
35.7 &  48.1 &  40.5 &  70.6 &  \nodata& 21     \\
 5371.49 & $-$1.64 &  0.95 & 113.3 & 126.7 & 147.0 &  \nodata& 118.6 & 188.1 &
 119.1 & 137.3 & 129.8 & 154.6 &  \nodata& 21     \\
 5383.37 &  0.64 &  4.31 &  24.3 &  30.0 &  43.3 &  \nodata&  35.1 &  69.2 &  
39.5 &  56.0 &  49.2 &  76.2 &  \nodata& 21     \\
 5393.17 & $-$0.71 &  3.24 &  19.3 &  31.5 &  43.2 &  \nodata&  28.9 &  79.4 &
  35.3 &  57.3 &  42.6 &  76.7 &  \nodata& 20     \\
 5397.13 & $-$1.95 &  0.92 & 103.4 & 113.6 & 134.1 &  \nodata& 105.7 & 172.3 &
 109.3 & 122.6 & 120.2 & 132.8 &  \nodata& 22     \\
 5404.15 &  0.52 &  4.42 &  25.3 &  33.2 &  47.2 &  \nodata&  31.5 &  79.4 &  
42.5 &  61.8 &  50.4 &  87.9 &  \nodata& 21     \\
 5405.78 & $-$1.80 &  0.99 & 102.9 & 118.4 & 138.2 &  \nodata& 105.5 & 177.1 &
 106.4 & 123.2 & 115.6 & 130.6 &  \nodata& 22     \\
 5410.91 &  0.40 &  4.45 &  12.9 &  16.6 &  26.3 &  \nodata&  19.1 &  44.7 &  
22.6 &  37.4 &  28.2 &  59.8 &  \nodata& 21     \\
 5415.20 &  0.64 &  4.37 &  22.2 &  29.3 &  41.3 &  \nodata&  28.9 &  68.4 &  
38.1 &  52.5 &  46.5 &  75.3 &  \nodata& 21     \\
 5429.70 & $-$1.88 &  0.95 & 106.1 & 121.6 & 136.6 &  \nodata& 111.1 & 187.4 &
 116.4 & 138.0 & 121.4 & 150.3 &  \nodata& 21     \\
 5434.53 & $-$2.08 &  1.01 &  92.8 & 103.4 & 126.4 &  \nodata&  98.1 & 161.6 &
  91.1 & 111.5 & 110.2 & 126.4 &  \nodata& 22     \\
 5497.52 & $-$2.83 &  1.01 &  \nodata&  73.8 &  \nodata&  \nodata&  62.9 & 130.7 &  61.3 &  89.9 &  \nodata& 102.7 &  \nodata& 21     \\
 5501.46 & $-$3.05 &  0.95 &  47.9 &  60.9 &  85.4 &  \nodata&  60.9 & 126.4 &
  47.3 &  78.0 &  63.5 &  89.9 &  \nodata& 21     \\
 5506.78 & $-$2.70 &  0.99 &  60.8 &  74.3 &  90.8 &  \nodata&  75.5 & 131.2 &
  60.2 &  88.5 &  77.7 & 102.1 &  \nodata& 22     \\
 5567.39 & $-$2.56 &  2.61 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  23.0 &  \nodata& 20     \\
 5569.62 & $-$0.49 &  3.42 &  22.5 &  29.8 &  43.6 &  \nodata&  35.2 &  82.9 &
  34.2 &  59.2 &  46.2 &  79.7 &  \nodata& 20     \\
 5572.84 & $-$0.28 &  3.40 &  29.8 &  41.9 &  58.4 &  \nodata&  43.9 &  93.6 &
  48.3 &  64.1 &  55.7 &  90.4 &  \nodata& 20     \\
 5586.76 & $-$0.14 &  3.35 &  39.8 &  48.2 &  66.9 &  \nodata&  53.6 & 102.4 &
  54.6 &  77.9 &  69.4 &  98.3 &  \nodata& 21     \\
 5658.82 & $-$0.84 &  3.38 &  12.5 &  \nodata&  35.5 &  \nodata&  20.4 &  66.3
 &  21.5 &  51.3 &  37.9 &  73.3 &  \nodata& 21     \\
 5701.55 & $-$2.18 &  2.56 &  \nodata &  10.1 &  27.1 &  \nodata&  \nodata&  49.9
 &   9.0 &  28.0 &  \nodata&  49.4 &  \nodata& 22     \\
 5753.12 & $-$0.69 &  4.24 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  11.9 &  \nodata&  30.7 &  \nodata& 21     \\
 5778.46 & $-$3.43 &  2.59 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 20     \\
 5916.25 & $-$2.95 &  2.45 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  18.3 &  \nodata&  \nodata&  \nodata&  19.2 &  \nodata& 22     \\
 6065.49 & $-$1.49 &  2.61 &  \nodata&  34.4 &  \nodata&  \nodata&  35.4 &  93.6 &  33.9 &  60.4 &  43.2 &  74.7 &  \nodata& 22     \\
 6136.61 & $-$1.41 &  2.44 &  39.3 &  52.7 &  69.6 &  \nodata&  49.9 & 112.9 &
  45.7 &  76.4 &  59.9 &  91.0 &  \nodata& 21     \\
 6137.70 & $-$1.36 &  2.59 &  29.5 &  42.7 &  63.8 &  \nodata&  43.4 & 109.1 &
  41.9 &  71.2 &  51.8 &  90.5 &  \nodata& 22     \\
 6151.62 & $-$3.26 &  2.18 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  24.8 &  \nodata&  \nodata&  \nodata&  18.6 &  \nodata& 22     \\
 6173.34 & $-$2.84 &  2.22 &  \nodata&   7.2 &  13.0 &  \nodata&  \nodata&  41.3 &  \nodata&  20.9 &  \nodata&  36.3 &  \nodata& 22     \\
 6180.21 & $-$2.59 &  2.73 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  21.5 &  \nodata& 20     \\
 6200.32 & $-$2.40 &  2.61 &  \nodata&  \nodata&  13.4 &  \nodata&  \nodata&  
39.6 &  \nodata&  19.4 &  \nodata&  34.6 &  \nodata& 22     \\
 6219.29 & $-$2.39 &  2.20 &   9.8 &  19.6 &  29.4 &  \nodata&  19.5 &  75.6 &
  15.2 &  40.8 &  21.3 &  59.1 &  \nodata& 22     \\
 6229.23 & $-$2.81 &  2.84 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 20     \\
 6232.64 & $-$1.22 &  3.65 &   3.4 &  \nodata&  \nodata&  \nodata&  \nodata&  
\nodata&  \nodata&  15.5 &  \nodata&  32.7 &  \nodata& 20     \\
 6240.65 & $-$3.23 &  2.22 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 20     \\
 6246.32 & $-$0.73 &  3.60 &  10.7 &  17.8 &  23.9 &  \nodata&  15.6 &  56.3 &
  18.2 &  32.0 &  24.0 &  57.2 &  \nodata& 20     \\
 6252.56 & $-$1.65 &  2.40 &  27.4 &  41.8 &  59.6 &  \nodata&  40.3 & 102.7 &
  36.4 &  68.7 &  49.6 &  81.3 &  \nodata& 22     \\
 6265.14 & $-$2.51 &  2.18 &  \nodata&  13.3 &  24.7 &  \nodata&  15.5 &  71.8
 &  13.5 &  38.2 &  17.4 &  55.5 &  \nodata& 22     \\
 6297.80 & $-$2.70 &  2.22 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  55.8 &  \nodata&  23.7 &  \nodata&  41.9 &  \nodata& 22     \\
 6301.50 & $-$0.72 &  3.65 &  \nodata&  39.3 &  \nodata&  \nodata&  \nodata&  
48.1 &  15.0 &  39.2 &  \nodata&  41.3 &  \nodata& 20     \\
 6322.69 & $-$2.39 &  2.59 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  46.0 &  \nodata&  18.5 &  21.4 &  40.2 &  \nodata& 22     \\
 6336.83 & $-$0.86 &  3.69 &   9.0 &  13.9 &  20.7 &  \nodata&  16.1 &  46.8 &
  13.4 &  30.4 &  \nodata&  48.6 &  \nodata& 20     \\
 6344.15 & $-$2.88 &  2.43 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  24.4 &  \nodata&  10.7 &  \nodata&  25.5 &  \nodata& 22     \\
 6355.03 & $-$2.36 &  2.84 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  23.2 &  \nodata&  15.9 &  \nodata&  25.8 &  \nodata& 20     \\
 6358.69 & $-$4.43 &  0.86 &  \nodata&  10.7 &  17.8 &  \nodata&   8.5 &  55.9
 &  \nodata&  20.7 &  10.3 &  41.1 &  \nodata& 22     \\
 6393.60 & $-$1.43 &  2.43 &  31.5 &  49.0 &  64.3 &  \nodata&  48.1 & 105.8 &
  49.8 &  69.1 &  55.8 &  85.7 &  \nodata& 20     \\
 6408.02 & $-$1.02 &  3.69 &  \nodata&   9.3 &  12.5 &  \nodata&  12.3 &  32.8
 &  \nodata&  22.6 &  14.5 &  41.4 &  \nodata& 20     \\
 6411.65 & $-$0.60 &  3.65 &  11.7 &  16.8 &  29.3 &  \nodata&  23.1 &  60.9 &
  21.5 &  44.6 &  30.0 &  65.3 &  \nodata& 20     \\
 6421.36 & $-$1.99 &  2.28 &  20.9 &  31.5 &  53.9 &  \nodata&  32.0 &  94.9 &
  29.8 &  56.4 &  42.4 &  74.8 &  \nodata& 22     \\
 6430.85 & $-$1.97 &  2.18 &  26.4 &  40.7 &  59.7 &  \nodata&  41.2 & 104.8 &
  44.4 &  66.4 &  49.4 &  80.8 &  \nodata& 22     \\
 6481.88 & $-$2.94 &  2.28 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  30.5 &  \nodata&  13.0 &  \nodata&  26.6 &  \nodata& 22     \\
 6494.99 & $-$1.23 &  2.40 &  54.4 &  71.3 &  84.3 &  \nodata&  61.5 & 139.8 &
  59.3 &  87.1 &  74.6 & 102.1 &  \nodata& 22     \\
 6498.95 & $-$4.66 &  0.96 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  35.8 &  \nodata&  \nodata&  \nodata&  23.0 &  \nodata& 22     \\
 6581.21 & $-$4.68 &  1.48 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 20     \\
 6593.88 & $-$2.38 &  2.43 &  \nodata&  15.6 &  18.3 &  \nodata&  12.1 &  54.3
 &  10.2 &  32.3 &  14.0 &  51.5 &  \nodata& 22     \\
 6609.12 & $-$2.65 &  2.56 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  25.2 &  \nodata&  13.2 &  \nodata&  29.3 &  \nodata& 22     \\
 6663.45 & $-$2.44 &  2.42 &   6.2 &   9.7 &  20.1 &  \nodata&  11.4 &  57.1 &
  \nodata&  32.9 &  13.6 &  47.8 &  \nodata& 22     \\
 6677.99 & $-$1.42 &  2.68 &  26.3 &  37.8 &  56.1 &  \nodata&  39.7 &  98.7 &
  35.3 &  65.2 &  46.0 &  88.5 &  \nodata& 21     \\
 6750.15 & $-$2.58 &  2.42 &   4.7 &  10.8 &  \nodata&  \nodata&  10.6 &  44.7
 &  \nodata&  22.8 &  12.3 &  42.3 &  \nodata& 22     \\
 6945.20 & $-$2.43 &  2.42 &  \nodata&  10.8 &  \nodata&  \nodata&  \nodata&  
48.3 &  \nodata&  37.5 &  \nodata&  \nodata&  \nodata& 20     \\
 6978.86 & $-$2.46 &  2.48 &  11.4 &  15.7 &  25.7 &  \nodata&   9.9 &  44.4 &
  \nodata&  30.2 &  \nodata&  61.7 &  \nodata& 22     \\
 7112.17 & $-$2.99 &  2.99 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&
  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 20     \\
\multicolumn{15}{c}{{FeII}} \\
 3295.81 & $-$2.90 & 1.08 & \nodata & \nodata & \nodata & 80.0 & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 23 \\ 
 3824.93 & $-$3.35 &  2.58 &  \nodata&  15.1 &  \nodata&  18.6 &  16.5 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 24     \\
 3974.17 & $-$3.45 &  2.70 &  \nodata&  \nodata&  \nodata&   8.0 &  \nodata&  13.7 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 24     \\
 4128.75 & $-$3.71 &  2.58 &   6.5 &  \nodata&  \nodata&  11.8 &  \nodata&  28.7 &  \nodata&  19.3 &  \nodata&  \nodata&  \nodata& 24     \\
 4178.86 & $-$2.51 &  2.58 &  33.3 &  44.8 &  57.4 &  51.9 &  42.7 &  81.8 &  62.8 &  59.0 &  66.9 &  70.8 &  \nodata& 24,25  \\
 4416.82 & $-$2.54 &  2.78 &  23.7 &  33.3 &  56.4 &  47.4 &  32.2 &  77.1 &  47.2 &  56.3 &  59.4 &  60.6 &  63.6 & 24     \\
 4489.18 & $-$2.91 &  2.83 &  12.3 &  18.2 &  36.5 &  29.1 &  17.8 &  61.3 &  34.1 &  38.1 &  40.0 &  53.1 &  \nodata& 24     \\
 4491.40 & $-$2.71 &  2.86 &  15.8 &  24.4 &  44.0 &  32.9 &  28.1 &  67.3 &  38.8 &  42.9 &  42.1 &  49.3 &  47.6 & 24,25  \\
 4508.29 & $-$2.33 &  2.86 &  29.9 &  38.1 &  63.5 &  51.4 &  41.9 &  88.4 &  57.3 &  59.7 &  66.3 &  68.2 &  76.2 & 24     \\
 4515.34 & $-$2.48 &  2.84 &  23.2 &  33.8 &  52.7 &  47.1 &  35.1 &  76.9 &  53.2 &  55.0 &  58.5 &  63.6 &  \nodata& 26     \\
 4520.23 & $-$2.60 &  2.81 &  22.3 &  33.0 &  52.0 &  50.8 &  34.3 &  85.2 &  49.2 &  58.8 &  57.3 &  62.8 &  \nodata& 26     \\
 4541.52 & $-$2.99 &  2.86 &  11.1 &  14.2 &  33.8 &  25.2 &  14.9 &  50.5 &  28.3 &  36.3 &  35.7 &  45.3 &  \nodata& 24     \\
 4555.89 & $-$2.39 &  2.83 &  31.0 &  41.4 &  60.0 &  48.4 &  39.4 &  78.0 &  60.6 &  63.0 &  70.1 &  68.4 &  \nodata& 24     \\
 4576.33 & $-$2.94 &  2.84 &  11.0 &  15.6 &  35.6 &  25.7 &  18.3 &  52.4 &  32.6 &  33.0 &  34.9 &  46.0 &  39.8 & 27     \\
 4582.84 & $-$3.10 &  2.84 &   6.0 &   9.8 &  24.0 &  16.5 &  13.0 &  39.3 &  19.3 &  21.7 &  23.6 &  32.2 &  27.3 & 24,25  \\
 4583.84 & $-$1.92 &  2.81 &  55.5 &  67.5 &  91.9 &  82.9 &  65.4 & 110.3 &  88.1 &  80.9 &  90.2 &  94.6 &  \nodata& 24     \\
 4620.51 & $-$3.21 &  2.83 &   5.0 &   8.0 &  23.9 &  13.9 &   9.9 &  34.4 &  15.0 &  18.8 &  22.1 &  30.5 &  24.0 & 27     \\
 4629.34 & $-$2.37 &  2.81 &  30.8 &  43.7 &  64.9 &  56.1 &  39.1 &  85.2 &  58.7 &  60.3 &  65.8 &  68.9 &  72.0 & 26     \\
 5018.45 & $-$1.22 &  2.89 &  89.8 &  98.0 & 125.9 &  \nodata&  90.7 & 157.7 & 125.6 & 114.8 & 125.3 & 129.0 &  \nodata& 26     \\
 5197.56 & $-$2.10 &  3.23 &  \nodata&  27.5 &  \nodata&  \nodata&  31.4 &  70.7 &  49.3 &  50.2 &  55.8 &  61.2 &  \nodata& 25     \\
 5234.62 & $-$2.23 &  3.22 &  26.1 &  31.2 &  55.7 &  \nodata&  33.9 &  76.7 &  54.4 &  54.6 &  59.5 &  63.3 &  \nodata& 27     \\
 5264.79 & $-$3.25 &  3.23 &  \nodata&  \nodata&  14.1 &  \nodata&  \nodata&  27.5 &  \nodata&  17.1 &  15.3 &  26.6 &  \nodata& 27     \\
 5276.00 & $-$1.94 &  3.20 &  28.5 &  36.7 &  67.4 &  \nodata&  41.0 &  89.6 &  58.6 &  64.3 &  68.5 &  83.7 &  \nodata& 25     \\
 5325.56 & $-$3.26 &  3.22 &  \nodata&  \nodata&  10.6 &  \nodata&  \nodata&  \nodata&  \nodata&  12.3 &  10.7 &  23.8 &  \nodata& 24     \\
 5414.08 & $-$3.50 &  3.22 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 27     \\
 6369.42 & $-$4.30 &  2.89 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 24     \\
 6432.67 & $-$3.50 &  2.89 &  \nodata&  \nodata&  12.6 &  \nodata&  \nodata&  25.2 &  \nodata&  10.6 &  10.6 &  18.8 &  \nodata& 27     \\
 6516.07 & $-$3.38 &  2.89 &  11.4 &  \nodata &  19.8 &  \nodata&  16.5 &  36.8 &  34.2 &  19.8 &  20.1 &  \nodata&  \nodata& 27     \\
\multicolumn{15}{c}{{CoI} } \\
 3845.47 &  0.01 &  0.92 &  66.4 &  80.0 &  \nodata&  84.8 &  73.9 & 119.9 &  \nodata&  \nodata&  67.7 &  \nodata&  \nodata& 28     \\
 3861.16 & $-$0.89 &  1.05 &  21.4 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 28     \\
 3922.76 & $-$2.10 &  1.05 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 28     \\
 3941.73 & $-$2.03 &  0.43 &  17.0 &  24.2 &  \nodata&  \nodata&  13.4 &  \nodata&  \nodata&  25.1 &  \nodata&  \nodata&  \nodata& 28     \\
 3957.93\tablenotemark{a} & $-$2.06 &  0.58 &   9.9 &  \nodata&  \nodata&  26.9 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  48.2 &  \nodata& 28     \\
 4020.90 & $-$2.07 &  0.43 &  15.9 &  25.4 &  \nodata&  37.8 &  24.1 &  74.3 &  \nodata&  40.4 &  29.2 &  57.0 &  86.5 & 28     \\
 4092.39 & $-$0.94 &  0.92 &  27.4 &  37.5 &  46.4 &  54.4 &  35.7 &  \nodata&  24.7 &  64.3 &  \nodata& 109.3 &  \nodata& 28     \\
 4110.53 & $-$1.08 &  1.05 &  15.1 &  22.6 &  43.1 &  37.1 &  25.8 &  85.2 &  \nodata&  43.5 &  36.5 &  65.8 &  97.6 & 28     \\
 4121.32 & $-$0.32 &  0.92 &  65.6 &  79.2 &  69.7 &  83.9 &  74.5 & 115.9 &  65.7 &  84.9 &  76.6 &  93.3 & 125.9 & 28     \\
\multicolumn{15}{c}{{NiI} } \\
 3500.85 & $-$1.29 & 0.17 & 79.8 & 96.6 & \nodata & 113.9 & 83.9 & 
126.2 & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3515.05 & $-$0.27 & 0.11 & 112.5 & 133.3 & \nodata & \nodata & \nodata & 
190.0 & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3516.21 & 0.06 & 3.54 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 30 \\
 3519.77 &  $-$1.42 & 0.28 & 74.1 & 88.8 & \nodata & 107.0 & 87.6 & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3524.54 & $-$0.01 & 0.03 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3566.37 &  $-$0.25 & 0.42 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3571.87 & $-$1.15 & 0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3597.71 & $-$1.12 & 0.21 & 87.7 & 99.8 & \nodata & 104.8 & 89.2 & 144.6 & 
\nodata & \nodata & \nodata & 108.7 & \nodata & 29 \\
 3602.28 & $-$2.19 & 0.17  & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3612.74 & $-$1.42 & 0.28 & 77.4 & 88.3 & \nodata & 99.3 & 81.1 & 
120.1 & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3619.39 & 0.02 & 0.42 & 107.4 & 124.5 & \nodata & \nodata & 118.1 & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3624.73 & $-$2.45 &  0.00 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3664.10 & $-$2.13 & 0.28  & 59.1 & 70.6 & \nodata & 84.8 & 65.7 & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3669.24 & $-$2.69 & 0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3670.43 & $-$2.40 & 0.17 & 54.8 & 65.6 & \nodata & 73.8 & 63.8 & 
99.0 & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3749.05 & $-$3.35 & 0.00 & \nodata & \nodata & \nodata & \nodata & \nodata & 
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 29 \\
 3775.57 & $-$1.41 &  0.42 &  77.8 &  90.4 &  \nodata&  94.7 &  86.3 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 29     \\
 3807.14 & $-$1.22 &  0.42 &  83.6 &  95.4 &  \nodata& 109.5 &  87.5 & 138.5 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 29     \\
 3831.69 & $-$2.27 &  0.42 &  54.4 &  69.1 &  \nodata&  86.9 &  64.8 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 29     \\
 3858.30 & $-$0.95 &  0.42 &  91.6 & 106.7 &  \nodata& 108.6 &  99.8 &  \nodata&  \nodata&  \nodata& 105.9 &  \nodata&  \nodata& 29     \\
 4331.65 & $-$2.10 &  1.68 &   5.0 &  11.2 &  \nodata&  17.7 &  10.1 &  43.3 &  \nodata&  21.3 &  \nodata&  41.5 &  49.8 & 28     \\
 4462.46 & $-$0.55 &  3.46 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  15.4 &  35.6 &  22.1 & 30     \\
 4470.48 & $-$0.31 &  3.40 &   4.5 &   8.4 &  \nodata&  12.1 &   8.4 &  26.0 &  \nodata&  18.6 &  \nodata&  29.7 &  21.0 & 30     \\
 4604.99 & $-$0.25 &  3.48 &   4.5 &   6.6 &  \nodata&  13.3 &   9.2 &  27.1 &  \nodata&  15.9 &  \nodata&  35.0 &  20.2 & 30     \\
 4648.65 & $-$0.10 &  3.42 &   6.4 &  11.0 &  \nodata&  18.7 &  13.4 &  37.1 &  \nodata&  26.6 &  \nodata&  39.8 &  28.3 & 30     \\
 4686.21 & $-$0.58 &  3.60 &   1.9 &  \nodata&  \nodata&   4.6 &  \nodata&  14.4 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 30     \\
 4715.76 & $-$0.32 &  3.54 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  13.5 &  \nodata&  31.2 &  \nodata& 30     \\
 4756.51 & $-$0.27 &  3.48 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  16.9 &  \nodata&  31.4 &  \nodata& 30     \\
 4866.27 & $-$0.21 &  3.54 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  20.1 &  \nodata&  14.2 &  \nodata&  33.0 &  \nodata& 30     \\
 4873.44 & $-$0.38 &  3.70 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  14.8 &  \nodata& 30     \\
 4925.56 & $-$0.77 &  3.65 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  14.5 &  \nodata& 30     \\
 4953.21 & $-$0.58 &  3.74 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  16.5 &  \nodata& 30     \\
 4976.35 & $-$3.10 &  1.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 28     \\
 4998.22 & $-$0.69 &  3.61 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  13.3 &  \nodata& 30     \\
 5003.75 & $-$2.80 &  1.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 28     \\
 5017.58 & $-$0.02 &  3.54 &  \nodata&   9.7 &  16.9 &  \nodata&  \nodata&  39.8 &  13.4 &  23.4 &  \nodata&  44.5 &  \nodata& 30     \\
 5035.36 &  0.29 &  3.63 &  \nodata&  21.2 &  20.0 &  \nodata&  21.3 &  40.6 &  18.0 &  30.5 &  24.0 &  49.5 &  \nodata& 30     \\
 5080.53 &  0.33 &  3.65 &  11.3 &  15.6 &  20.8 &  \nodata&  14.9 &  49.2 &  20.7 &  33.2 &  23.4 &  53.7 &  \nodata& 30     \\
 5099.32 & $-$0.44 &  3.65 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  20.9 &  \nodata& 30     \\
 5102.97 & $-$2.62 &  1.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  17.9 &  \nodata& 28     \\
 5137.08 & $-$1.99 &  1.68 &  \nodata&  \nodata&  23.9 &  \nodata&  20.9 &  70.4 &  \nodata&  39.2 &  22.8 &  59.5 &  \nodata& 28     \\
 5424.65 & $-$2.77 &  1.95 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  11.6 &  \nodata& 28     \\
 5435.87 & $-$2.59 &  1.99 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  15.6 &  \nodata&   7.0 &  \nodata&  15.9 &  \nodata& 28     \\
 5476.91 & $-$0.89 &  1.83 &  53.5 &  65.1 &  78.6 &  \nodata&  64.7 & 123.8 &  62.0 &  83.6 &  73.0 & 105.1 &  \nodata& 28     \\
 5578.72 & $-$2.64 &  1.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  25.4 &  \nodata&  \nodata&  \nodata&  23.2 &  \nodata& 28     \\
 5587.87 & $-$2.14 &  1.93 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  27.8 &  \nodata&   8.9 &  \nodata&  22.2 &  \nodata& 28     \\
 5592.28 & $-$2.57 &  1.95 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  25.5 &  \nodata&  \nodata&  \nodata&  27.0 &  \nodata& 28     \\
 5711.91 & $-$2.27 &  1.93 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  30.4 &  \nodata&  \nodata&  \nodata&  36.5 &  \nodata& 28     \\
 5754.68 & $-$2.33 &  1.93 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  40.9 &  \nodata&  15.0 &  \nodata&  34.4 &  \nodata& 28     \\
 5847.00 & $-$3.21 &  1.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 28     \\
 5892.88 & $-$2.35 &  1.99 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  30.6 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 28     \\
 6108.12 & $-$2.45 &  1.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  34.0 &  \nodata&  14.9 &  \nodata&  28.5 &  \nodata& 28     \\
 6128.99 & $-$3.33 &  1.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&   7.7 &  \nodata& 28     \\
 6176.81 & $-$0.26 &  4.09 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  15.8 &  \nodata& 30     \\
 6314.66 & $-$1.77 &  1.93 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  31.0 &  \nodata&  17.6 &  \nodata&  27.1 &  \nodata& 28     \\
 6327.60 & $-$3.15 &  1.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&   9.1 &  \nodata& 28     \\
 6482.80 & $-$2.63 &  1.93 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  28.3 &  \nodata&  \nodata&  \nodata &  14.9 &  \nodata& 28     \\
 6643.64 & $-$2.30 &  1.68 &  \nodata&  14.4 &  24.5 &  \nodata&  13.5 &  62.8 &  \nodata&  32.1 &  18.9 &  53.3 &  \nodata& 28     \\
 6767.77 & $-$2.17 &  1.83 &  \nodata&   8.3 &  19.4 &  \nodata&  14.9 &  59.3 &  \nodata&  28.1 &  16.6 &  46.0 &  \nodata& 28     \\
 7062.97 & $-$3.50 &  1.95 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 28     \\
\multicolumn{15}{c}{{ZnI}} \\
 4722.20 & $-$0.39 &  4.03 &   9.6 &  \nodata&  \nodata&  \nodata&  \nodata&  35.8 &  \nodata&  19.8 &  \nodata&  33.2 &  \nodata& 31     \\
 4810.55 & $-$0.17 &  4.08 &  14.0 &  14.3 &  28.8 &  \nodata&  16.3 &  42.0 &  18.4 &  28.1 &  22.4 &  40.2 &  \nodata& 31     \\
\multicolumn{15}{c}{{YII} } \\
 3549.01 & $-$0.28 & 0.13 & 8.0 & 23.5 & \nodata & 43.8 & 42.3 &
70.5 & \nodata & \nodata & \nodata & \nodata & \nodata & 32 \\
 3600.74 & 0.28 & 0.18 & 23.7 & 42.5 & \nodata & 64.4 & 51.3 &
94.7 & \nodata & \nodata & \nodata & \nodata & \nodata & 32 \\
 3611.04 & 0.01 & 0.13 & 15.6 & 31.3 & \nodata & 54.3 & 44.7 &
86.5 & \nodata & \nodata & \nodata & \nodata & \nodata & 32 \\
 3628.70 & $-$0.71 & 0.13 & \nodata & 13.6 & \nodata & 30.3 & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 32 \\
 3710.29 & 0.46 & 0.18 & \nodata & 62.0 & \nodata & 73.6 & 60.7 &
105.3 & \nodata & \nodata & \nodata & \nodata & \nodata & 32 \\
 3747.55 & $-$0.91 & 0.10 & \nodata & 8.9 & \nodata & 20.8 & 17.5 &
53.0 & \nodata & \nodata & \nodata & \nodata & 51.0  & 32 \\
 3774.34 &  0.21 &  0.13 &  25.3 &  51.3 &  \nodata&  63.0 &  60.7 & 105.4 &  \nodata&  \nodata&  \nodata&  \nodata& 101.1 & 32     \\
 3788.70 & $-$0.07 &  0.10 &  17.2 &  41.4 &  \nodata&  62.6 &  45.3 & 102.6 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 32     \\
 3950.36 & $-$0.49 &  0.10 &   8.7 &  23.0 &  \nodata&  41.5 &  35.6 &  79.9 &  \nodata&  47.5 &  68.0 &  \nodata &  84.0 & 32     \\
 4398.01 & $-$1.00 &  0.13 &  \nodata&  \nodata&  38.8 &  28.1 &  19.6 &  64.9 &  23.6 &  35.5 &  35.3 &  43.3 &  64.6 & 32     \\
 4854.87 & $-$0.38 &  0.99 &  \nodata&  \nodata&  23.3 &  \nodata&  \nodata&  43.2 &  \nodata&  18.4 &  \nodata&  36.8 &  \nodata& 32     \\
 4883.69 &  0.07 &  1.08 &  \nodata&  \nodata&  38.0 &  \nodata&  15.4 &  60.8 &  30.5 &  31.1 &  34.3 &  52.3 &  \nodata& 32     \\
 4900.11 & $-$0.09 &  1.03 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  30.7 &  45.2 &  56.3 &  \nodata& 32     \\
 5087.42 & $-$0.17 &  1.08 &  \nodata&  \nodata&  23.0 &  \nodata&  \nodata&  42.2 &  14.6 &  19.6 &  23.3 &  43.2 &  \nodata& 32     \\
5205.731 & $-$0.34 & 1.03 & \nodata & \nodata & \nodata & \nodata & \nodata &
45.1 & \nodata & \nodata & \nodata & \nodata & \nodata & 32 \\
\multicolumn{15}{c}{{ZrII}} \\
 3479.03 & $-$0.69 & 0.53 & \nodata & \nodata & \nodata & 19.6 & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 33 \\
 3479.39 & 0.17 & 0.71 & \nodata & \nodata & \nodata & 37.4 & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 33 \\
 3499.57 & $-$0.81 & 0.41 & \nodata & \nodata & \nodata & 14.1 & \nodata &
34.3 & \nodata & \nodata & \nodata & \nodata & \nodata & 33 \\
 3505.67 & $-$0.36 & 0.16 & 10.8 & 25.6 & \nodata & 46.4 & 36.5 &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 33 \\
 3551.96 & $-$0.31 & 0.09 & 9.2 & 34.1 & \nodata & 56.1 & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 33 \\
 3588.33 & $-$1.13 & 0.41 & \nodata & \nodata & \nodata & \nodata & 12.6 &
25.1 & \nodata & \nodata & \nodata & \nodata & \nodata & 33 \\
 3607.38 & $-$0.64 & 1.24 & \nodata & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 33 \\
 3714.79 & $-$0.93 & 0.53 & \nodata & \nodata & \nodata & 13.2 & \nodata &
50.2 & \nodata & \nodata & \nodata & \nodata & \nodata & 33 \\
 3836.77 & $-$0.06 &  0.56 &  \nodata &  22.9 &  \nodata&  \nodata&  31.2 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 33     \\
 4050.33 & $-$1.00 &  0.71 &  \nodata&  \nodata&  \nodata&   9.6 &  \nodata&  31.5 &  \nodata&  \nodata&  \nodata&  28.4 &  33.5 & 33     \\
 4208.98 & $-$0.46 &  0.71 &   2.6 &  11.4 &  35.8 &  27.8 &  19.5 &  65.0 &  26.7 &  31.3 &  40.0 &  50.3 &  65.2 & 33     \\
 4317.32 & $-$1.38 &  0.71 &  \nodata&  \nodata&  \nodata&   6.5 &  \nodata&  24.6 &  \nodata&  \nodata&  \nodata&  14.8 &  21.2 & 33     \\
 5112.28 & $-$0.59 &  1.66 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 33     \\
\multicolumn{15}{c}{{BaII}} \\
 4554.03 &  0.12 &  0.00 &  83.1 & 107.3 & 161.4 & 105.4 & 118.1 & 189.0 & 135.1 & 140.7 & 167.1 & 161.3 & 184.8 & 34     \\
 5853.69 & $-$1.02 &  0.60 &  \nodata&  13.6 &  62.5 &  \nodata&  21.0 &  79.7 &  32.2 &  45.2 &  63.6 &  65.2 &  \nodata& 34     \\
 6141.73 & $-$0.07 &  0.70 &  28.0 &  50.3 & 114.5 &  \nodata&  56.3 & 143.3 &  83.9 &  87.5 & 108.8 & 106.3 &  \nodata& 34     \\
 6496.91 & $-$0.37 &  0.60 &  33.2 &  60.5 & 111.6 &  \nodata&  49.0 & 136.0 &  77.4 &  83.1 & 107.6 & 114.0 &  \nodata& 34     \\
\multicolumn{15}{c}{{LaII}} \\
 3995.75 & $-$0.02 &  0.17 &  \nodata&  \nodata&  \nodata&  syn &  \nodata&  \nodata&  \nodata&  syn &  syn & syn & syn & 35     \\
 4086.71 & $-$0.16 &  0.00 & syn &  syn &  \nodata& syn & syn &  syn &  syn &
 syn &  syn &  syn &  syn & 35     \\
 4123.23 &  0.12 &  0.32 &  \nodata&  syn &  syn &  syn &  \nodata&  syn &  syn &  syn &  syn &  syn &  syn & 35     \\
 4333.76 & $-$0.16 &  0.17 &  \nodata&  syn &  syn &  \nodata&  \nodata&  syn 
&  \nodata&  syn &  \nodata&  syn &  syn & 35     \\
\multicolumn{15}{c}{{CeII}} \\
 4083.23 &  0.24 &  0.70 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  19.5 &  \nodata&  \nodata&  \nodata&  22.5 &  \nodata& 35   \\
 4120.84 & $-$0.24 &  0.32 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  10.8 &  \nodata&  \nodata&  \nodata&   7.5 &  \nodata& 35     \\
 4222.60 & $-$0.18 &  0.12 &  \nodata&  \nodata&  15.3 &  \nodata&  \nodata&  26.7 &  \nodata&  \nodata&  \nodata&  22.1 &  18.0 & 35     \\
 4562.37 &  0.33 &  0.48 &  \nodata&  \nodata&  13.7 &  \nodata&  \nodata&  32.3 &  \nodata&   9.9 &  19.5 &  23.6 &  18.4 & 35     \\
 4628.16 &  0.26 &  0.52 &  \nodata&  \nodata&  15.7 &  \nodata&  \nodata&  25.1 &  \nodata&   8.5 &  16.4 &  21.9 &  15.0 & 35     \\
\multicolumn{15}{c}{{PrII}} \\
 3964.81 &  0.09 &  0.05 &  \nodata&  syn &  \nodata&  syn &  syn &  syn 
&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 3965.26 & $-$0.13 &  0.20 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  syn &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
\multicolumn{15}{c}{{NdII}} \\
 3973.27 &  0.43 &  0.63 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  25.5 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 4021.34 & $-$0.17 &  0.32 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  24.8 &  \nodata&  \nodata&  13.4 &  26.8 &  15.5 & 35     \\
 4061.09 &  0.30 &  0.47 &  \nodata&   8.2 &  \nodata&   7.2 &  11.1 &  56.3 &  \nodata&  29.7 &  45.6 &  46.0 &  49.3 & 35     \\
 4069.27 & $-$0.40 &  0.06 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  26.4 &  \nodata&  \nodata&  15.2 &  \nodata&  \nodata& 35     \\
 4109.46 &  0.18 &  0.32 &  \nodata&  \nodata&  38.6 &   7.6 &  15.2 &  70.6 &  24.4 &  \nodata&  47.0 &  55.1 &  \nodata& 35     \\
 4232.38 & $-$0.35 &  0.06 &  \nodata&  \nodata&  12.6 &  \nodata&  \nodata&  33.1 &  \nodata&  \nodata&  14.7 &  19.5 &  24.1 & 35     \\
 4446.39 & $-$0.63 &  0.20 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  33.3 &  \nodata&   8.7 &  19.0 &  21.4 &  24.9 & 35     \\
 4462.99 & $-$0.07 &  0.56 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  35.3 &  \nodata&  12.8 &  17.8 &  24.5 &  24.9 & 35     \\
 5130.59 &  0.10 &  1.30 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  12.3 &  \nodata&  \nodata&  \nodata&  12.0 &  \nodata& 35     \\
 5212.35 & $-$0.70 &  0.20 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 5234.21 & $-$0.46 &  0.55 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 5249.60 &  0.08 &  0.98 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  11.5 &  \nodata& 35     \\
 5293.17 & $-$0.20 &  0.82 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  16.7 &  \nodata& 35     \\
 5311.48 & $-$0.56 &  0.99 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 5319.82 & $-$0.35 &  0.55 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  28.2 &  \nodata&  \nodata&  13.9 &  17.8 &  \nodata& 35     \\
 5361.51 & $-$0.40 &  0.68 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
\multicolumn{15}{c}{{SmII}} \\
 3896.97 & $-$0.58 & 0.04 & \nodata & \nodata & \nodata & \nodata & \nodata &
16.3 & \nodata & \nodata & \nodata & \nodata & \nodata & 36 \\
 3993.30 & $-$0.89 & 0.04 & \nodata & \nodata & \nodata & \nodata & \nodata &
16.3 & \nodata & \nodata & \nodata & \nodata & \nodata & 36 \\
 4035.10 & $-$0.45 &  0.33 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&   6.4 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 36     \\
 4244.70 & $-$0.73 & 0.28 & \nodata & \nodata & \nodata & \nodata & \nodata &
5.6 & \nodata & \nodata & \nodata & \nodata & \nodata & 36 \\
 4329.02 & $-$0.30 &  0.18 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  24.5 &  \nodata&  \nodata&  16.5 &  20.9 &  \nodata& 36     \\
 4452.71 & $-$0.43 &  0.28 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  22.4 &  \nodata&  \nodata&  \nodata&  17.8 &  20.1 & 36     \\
 4499.48 & $-$1.01 &  0.25 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&   8.6 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 36     \\
 4519.64 & $-$0.43 &  0.54 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  14.4 &  \nodata&  \nodata&  \nodata&  14.1 &  \nodata& 36     \\
 4523.91 & $-$0.58 &  0.43 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  16.7 &  \nodata&  \nodata&   9.5 &  12.3 &  10.5 & 36     \\
 4537.95 & $-$0.23 &  0.48 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  11.8 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 36     \\
 4577.69 & $-$0.77 &  0.25 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  13.7 &  \nodata&  \nodata&   8.9 &  \nodata&   8.1 & 36     \\
 4642.23 & $-$0.52 &  0.38 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  18.2 &  \nodata&  \nodata&  14.9 &  16.1 &  \nodata& 36     \\
\multicolumn{15}{c}{{EuII} } \\
 3724.95 &  $-$0.08 &  0.00  & \nodata & \nodata & \nodata & \nodata & 
syn  & syn  & \nodata & \nodata & syn & \nodata & syn  & 35 \\  
 4129.70 &  0.20 &  0.00 &  syn &  syn &  syn & syn & syn & syn & syn & syn 
& syn & syn & syn & 35     \\
 4205.05 &  0.12 &  0.00 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 4435.56 & $-$0.09 & 0.21 & \nodata & \nodata & \nodata & \nodata & \nodata & syn & \nodata
& \nodata & \nodata & \nodata & \nodata  & 35 \\
\multicolumn{15}{c}{{GdII} } \\
 3331.40 & $-$0.14 & 0.00  & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  37 \\
 3768.40 & $-$0.63 &  0.08 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  45.6 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 37     \\
 3796.39 &  0.07 &  0.03 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  46.9 & 37     \\
\multicolumn{15}{c}{{TbII}} \\
 3848.74 &  0.06 &  0.00 & syn &  syn &  \nodata&  syn    &  \nodata&  syn    &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 3874.17 &  0.28 &  0.00 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 4005.47 &  0.25 &  0.13 &  \nodata&  syn    & syn     & syn     & syn     & 
 \nodata&  syn    &  syn    &  syn    &  syn    &  \nodata& 35     \\
\multicolumn{15}{c}{{DyII}} \\
 3385.02 &  0.11  & 0.10 & \nodata & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 3434.37 & $-$0.43 & 0.00& \nodata & \nodata & \nodata & \nodata & \nodata &
31.1 & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 3454.32 & $-$0.13 & 0.10& \nodata & \nodata & \nodata & \nodata & \nodata &
58.8 & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 3531.71 &  0.79 & 0.00& 14.5 & 33.4 & \nodata & \nodata & 32.4 &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 3536.02 &  0.47 & 0.54& \nodata & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 3546.83 & $-$0.57 & 0.10& \nodata & \nodata & \nodata & \nodata & \nodata &
32.6 & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 3563.15 & $-$0.16 & 0.10& \nodata & \nodata & \nodata & \nodata & \nodata &
27.8 & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 3606.13 &  0.26 & 0.10& \nodata & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 3672.32 & $-$0.39 & 0.59& \nodata & \nodata & \nodata & \nodata & \nodata &
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 3694.82 &  0.00  & 0.10& \nodata & \nodata & \nodata & \nodata & \nodata &
57.9 & \nodata & \nodata & \nodata & \nodata & \nodata & 38 \\  
 4073.12 & $-$0.38 &  0.54 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  22.8 &  \nodata&  \nodata&  \nodata&  11.5 &  \nodata& 38     \\
 4103.31 & $-$0.39 &  0.10 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  47.3 &  \nodata&  \nodata&  33.2 &  35.9 &  \nodata& 38     \\
 4449.71 & $-$0.95 &  0.00 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  15.8 &  18.9 &  15.7 & 38     \\
\multicolumn{15}{c}{{HoII}} \\
 3810.74 &  0.14 &  0.00 &  \nodata&  syn    &  \nodata&  syn   &   \nodata&  
syn    &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 4045.47 & $-$0.18 &  0.00 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 4152.58 & $-$0.89 &  0.08 &  syn    &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
\multicolumn{15}{c}{{ErII} } \\
 3692.65 &   0.13 &   0.05  & syn     & syn & \nodata & syn & syn &
syn & \nodata & \nodata & \nodata & \nodata & syn & 35 \\ 
 3830.48 & $-$0.36 &  0.00 &  \nodata&  \nodata&  \nodata&  \nodata&  syn & 
 syn &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 3896.23 & $-$0.24 &  0.00 &  \nodata&  \nodata&  \nodata&  \nodata&  syn 
&  syn &  \nodata&  \nodata&  \nodata&  \nodata&  syn & 35    \\
\multicolumn{15}{c}{{TmII} } \\
 3700.26 &  -0.29 & 0.03 & \nodata & \nodata & \nodata & syn & 
\nodata
 & syn & \nodata & \nodata & \nodata & \nodata & \nodata & 35 \\ 
 3795.76 & $-$0.17 &  0.03 &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata&  syn &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
 3848.02 & $-$0.13 &  0.00 & syn & syn &  \nodata&  syn &  syn &  syn &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
\multicolumn{15}{c}{{YbII} } \\
 3694.19 &   $-$0.29 &  0.0 & syn  &  syn & \nodata & syn & syn & syn
& \nodata & \nodata & \nodata & \nodata & syn  & 39 \\
\multicolumn{15}{c}{{HfII} } \\
 3719.28 & $-$0.89 & 0.61 & \nodata & \nodata & \nodata & \nodata & \nodata &
syn & \nodata & \nodata & \nodata & \nodata & \nodata & 35 \\
 3793.38 & $-$0.95 &  0.38 &  syn &  \nodata&  \nodata&  \nodata&  syn &  
syn &  \nodata&  \nodata&  \nodata&  \nodata&  \nodata& 35     \\
\multicolumn{15}{c}{{OsI} } \\
 4261.85 & $-$1.44 &  0.00 &  syn&  syn&  syn&  syn&  syn&  syn&  syn&  syn&  syn&  syn&  \nodata& 35     \\
\enddata
\tablenotetext{a}{Line not used in abundance analysis}
\tablenotetext{b}{Line not used if EW $>$ 50.0}
\tablerefs{(1) Wiese \& Martin 1980; (2) Wiese, Smith \& Miles 1969; (3) J\"onsson 
et al. 1984;
(4) Fuhrmann, Axer, \& Gehren 1995; (5) Garz 1973; (6) Beveridge \& Sneden 1994; 
(7) Smith \& Raggett
1981; (8) Lawler \& Dakin 1989; (9) Blackwell et al.{} 1986; 
(10) Nitz et al.{} 1998; 
(11) Bizzarri et al.{} (1993); 
(12) Martin et al.{} 1988; (13) Doerr et al.{} 1985; (14) Bi\'emont
et al.{} 1989; (15) Blackwell et al.{} 1984b; (16) Tozzi et al.{} 1985; 
(17) Booth et al.{} (1983); (18) Blackwell \& Collins 1972; (19) 
Martinson et al.{}
1977; (20)Bard, Kock, \& Kock 1991; (21) O'Brian et al.{} (1991); (22) 
Blackwell et al.{} 1979a, 1979b, 1980, 1982a, 1982b, 1982c; (23) Heise
\& Kock 1990; (24) Moity 1983; (25) Kroll \& Kock 1987; (26) Bridges 1973;
(27) Hannaford et al.{} 1992; (28) Fuhr et al.{} (1988); (29) Blackwell et al.{}
 1989; (30) Wickliffe \& Lawler 1997; (31) Bi\'emont \& Godefroid 1980; 
(32) Hannaford et al.{} 1982; (33) Bi\'emont et al.{} 1981; (34) Kastberg et al. 1993; (35)
Sneden et al.{} (1996); (36) Bi\'emont et al.{} 1989; (37) Bergstr\"om et al.{}
1988; (38)Bi\'emont et al.{} 1993 (39) Pinnington et al.{} 1997b} 
\end{deluxetable}

